Secure Mobile Identities

The unique identities of every mobile user (phone number,IMSI) and device (IMEI) are far from secure and are increasingly vulnerable to a variety of network-level threats. The exceedingly high reliance on the weak SIM authentication layer does not present any notion of end-to-end security for mobile users. We propose the design and implementation of Secure Mobile Identities (SMI), a repetitive key-exchange protocol that uses this weak SIM authentication as a foundation to enable mobile users to establish stronger identity authenticity. The security guarantees of SMI are directly reliant on the mobility of users and are further enhanced by external trusted entities providing trusted location signatures (e.g. trusted GPS, NFC synchronization points). In this paper, we demonstrate the efficacy of our protocol using an implementation and analysis across standard mobility models.

==> Eurosys'16/.git/objects/0d/d43af0ac6524ea6e9f326e3a470234860f8ba8 <==
xRM›0í•ùVv›• M?T	)RمTHÙ$ÚÐvo°)Öa³Mÿ}BªpèedÏ<?Ï{3)ª"-ß/¿¼{Þí¢­÷°•.%¾?<…Ã]åyVˆìöþznÁnïÎð¹Sóö‡©'ÿG8Qào¢àe¢bÄà&xÙ{[?ðã´º½»ô3óÑé'?ƒ‡ÍîыÂݖš€ÑeL›¤âIÁ7InÜËǁU&¯'¥)§®©S®Öç)Ê»`aBŽeÿg
jM¯‰£ÖÌ6…1¢aöž«ßª"üÌlE¼'çt,›±ô¶ÖèÀl"©àâZUF¯LÓ
J>ª²NŒL%Jóg#Þ®–Χ‡©{.ËP$qó|BX*Ó+±ÓÈÉ,§ÓŽ]ÓÌt›–ÒЃ~4@°ntV½îVŒî£iÏÁš"ŒÖ¤ßK«
2gÑ«Œ»T%œ‰mØ­Îòñ«N9X_EV(ÆfâXÓ*	κt.Q¸×ðÙÞõyÒ3	¦òŒ–´7Ÿ7%³svïÐvP¤¡@÷NÒ)']Ä_QuQµ†¾÷Ÿ½u'(
·ßÝXÛ¥.ˆqÊ7]ÈFVnÊ┸8˜6Ï\ešº¿µˆ)@

==> Eurosys'16/.git/objects/6a/94acbaf21c98550d3040106d540f161b8db1a4 <==
x•ŽY
1DýÎ)úJ–éND¼J–0Î3žßè
ü*xÔ+*¯µ.¬Õ‡ÞD ?۔8"€"'Abï‰CðL\"£KÎÍbÕ›<;Ш f­sF,H'	ÑͦHñì¨dÖ©8÷~_¼c۟pο4t½Õ¸<Ny­0z䭃£ž´VƒŽo]þ³ÔÖꚖ¯¯=
õç/E@

==> Eurosys'16/.git/objects/72/8f6c295521a9223a53f099a2fbf78385b993a2 <==
x•ŽQn1ûSøEŽ"u	!®âØYX•°hÉr~P{'~=i¤Ñ<]{_寱µÙGãZ³ä`\Jå«ÍšrÁɈ§ÙgrÙÚ}@V5MɇP†"I)Q8c¥¨\‹†êd×uƒ—lûŽú»žÏ—.Ëí k?q*2øƈè>ôóm´ÿYî/±?LF3¸ÉÏóÚh¶Œ§{®éGƒ

==> Eurosys'16/.git/objects/bc/46284752979a2fa3f2386c0c9a964fa470859a <==
xuTÉnÛ0íÙ_A ðͲã¤iҞbÄ)` 	'¸Šª‡5–Xs¸81ý{Gr'š®sÅ7oæÍÆBš'MÏN.ßå¥áA¡ö\'s¿$z¶íÈ?ndPúwt¢Ê@¢Ác;ȃÃø*ŒR4.¨vÈjï›Ï"	÷ ÇÆV"f]Mv`b_YhjÁŸß`¼Â	uP£J#¯¤Ÿ^¹P¬DìFPN¯ÛÁ ×øäk4U¤Œ…jãuÿI‹6~ݙR=žD¥ ·ý'AJ\	-¼0ºóg
[`%t|­u'Ä/1.'"Zvg
!'-JjñёÅ0‡àkc…^™øH|Gõǒ=tÍaï/OmrJRÊ8Æï`ƒf×5è҂Ã5XУ–Å{|b?]³oZlÐ:á·£6²Mg>æ‰ù•Þ†1–¡eyÞIÑå`ø,b
l¦þ@9:êŽÍŠÀæ5¢s¼ÚÆÐŽyœ¹Z¢«Ù²«€\ÞhoC³eÍǝØ\Q]ºû17j_Ñ-¬]­"¦· A³e(,(Ђ>*°s*w¬+îÆI–-Ut+Xcß:;ôÜM…9Ma‰
ÍQ<ï:(t|¼_Î(œ·À»iÜ»f'mÊÀû'H°ÓìÁš'FiI't•2ϲ%ù{ºÞȖw"ún3Sè<{DÒÿ‡ú˜Ýl@†#ÈE¶P
i ê¾ Ã}ý—ÙͳGíhži è"›•e?é@:Rìӛñ¦'$RÒRf?hÓ¦Ól.®‹wnzš]ÍexÑÒo]CÏm–(¤0ý³±u~K;Ea7ä{‰»Ÿ­ñAëfMƒºÏ}ïé´·¤û¶çÑ

==> Eurosys'16/.git/objects/bc/8a42f6bec8463a318bfd23ecc16f9baa74ee31 <==
x=ÛjÃ0†wݧÐÌ#lcÐÁ`§²d]º0_"^ډˆM;øÀJÞ}JRê~IŸô['áîþáê¹ØU?ßo›Í{±ûà§/m³uèEÄëÐ)*çá	N‡"L…dZ@Ø^"G<¦ý,ä!±ZQG´p³ô鬈JX(o ¬ëdq–·Ú¶ŒäöS˜h¥øûEc`ëZø•BËÍ^6^SZ¡÷zÊq:º‡Ó։òêØ@遨ãb êhpºŸO¦wÂÖz—z菚av‰6êšZˆ>…¢FÕQå"Î/À'\9©ùÎÕÅüS·Y¶Wã?Ékv]

==> Eurosys'16/.git/objects/c0/a37c7963ce52d8e061f08e4a2efa38b071331a <==
xuTÉnÛ0íÙ_A ðͲã¤YšSŒ8$AwAQ÷0¢Æk.;¡ïHNPÓuN¢øæͼ٘K"³ñÙùɇþ¢0<(ԞKp.:QÖ47z™a°Æm]ÓKm~Iôm
5ځßndPúwKÍ@¢Á#''Ãø
JŒRÔ.¨¦Ï*ïëëш{ÐCcËQ½*G;0±/-ԕà/ï0Þà"ƒ:(áQ¥'—Ò€O¯\ȗ¢ö@#(§ÀWM¯·Ð¸ñ‹*RU"jâm÷IW‹&~ݙR=žD¥ ‰÷Ý'A
\
-¼0º‰Óg
›c)t|ëG+Ä/1Îf×lŽœ$³"‰lVPÇÈ	Rwzý_+ôÒÄgrâ¨	X°§¶CìãÕé¡Í'2•2öúñ;Ø Ùmº°àpô añ7짱+öM‹5Z'üvÐD¶n͇<1¿ÑÛ0Ä"4l±h¥è¢×ÿ±6Q uÇ&y`Ó
rÑ:^îCh	Ç<N\%ÑUl^U@.ï´·¡Þ²™æÃÖìn¨.íýµ¯èV®RBS'[РÙ<ähA	Ø:•;Ö
wÃ$ˆ*Ú[(Xa×!:;ôÜM…9b5
S<oÛ(t||œOg#ȝ·Àۑܻg3'mŠÀ»¹H°ÓìɚœæiNk't™2ϲ9ùÛ<€Nï?e45Dôíz¦ÐyöŒ¤þu'Ý­A†#Èe6S5i ê¾¢ý}ýWÙ݋Gíh¨i è2›E7î@:Rìó»ñÆ'$RÒ;Rd?hÓÆãl*®wn|šÝÍexÕÒ­^Mo­—È¥0ÝÛ±u~K‹yn×ä{‰»ŸíòAë&uº/]ïé´·©÷ä

==> Eurosys'16/NSDI/1-Introduction.tex <==
\section{Introduction}
\label{intro}

Existing authentication standards adopted by GSM cellular providers provide no notion of end-to-end trust. This is inherently due to the GSM authentication protocol, which is asymmetric in that it does not require the network to identify itself - exposing mobile devices to various network-level security vulnerabilities. Adversaries can launch different forms of Man-in-the-Middle (MitM) attacks \cite{securityVul} including message interception, modification, eavesdropping, spoofing and phishing. The recent proliferation in attacks on GSM security \cite{praattack,germany,comp128} has been exacerbated by the widespread availability of software-defined cellular platforms like OpenBTS \cite{openbts} powered by USRP nodes \cite{usrp}, sysmoBTS \cite{sysmobts}, Fairwaves \cite{fairwaves} and Opencell \cite{opencell}.  Application level security solutions typically rely on simple password based user authentication coupled with SSL/TLS \cite{ssltls}, both of which are fraught with significant problems. Surprisingly, many transactions in the mobile landscape are performed through applications written such that SSL is not always enabled \cite{schrittwieser2012guess}. A recent survey by FireEye on the $1000$ most downloaded free applications on the Google Play Store showed that of the $614$ applications that use SSL/TLS to communicate with a remote server, $448$ ($73\%$) do not check certificates \cite{fireeye}.

We aim to address the following question: {\em Can we build a secure key framework that enables mobile devices to establish an end-to-end trustworthy channel with other mobile devices, or a cloud service provider?} In this paper, we present the design and implementation of {\em Secure Mobile Identities (SMI)}, an identity authentication mechanism that enables mobile devices to convert their weak SIM identity to a stronger {\em self-certifying identity}. Establishing such a secure identity for every mobile device significantly enhances user and application security, especially for cloud-hosted applications that rely on the identity of the mobile device as an alternate trust channel (e.g. 2-factor authentication \cite{2fauth,schneier2005two}). 
%Most 2-factor authentication mechanisms transmit the verification code to the mobile device of a user in clear text providing relatively limited protection.

While there have been numerous efforts to enhance the security of mobile devices at different levels, none of these results focus on building a strong end-to-end trust model around the {\em unique identity} of mobile devices. Most existing solutions have predominantly focused on either the lower level to secure the wireless channel \cite{securepairing, bambos2000channel} or the higher level to protect user identities and applications \cite{lookout, otp, 2fauth}, while others have focused on protecting the mobile device itself \cite{cook2010method}. SMI is built upon the pragmatic assumption that the Mobile Network Operator (MNO) \footnote{Used interchangeably with Cellular Network Provider}is trustworthy, but the underlying cellular channel may not be. The SMI setup models for a local network-level adversary whose aim is to hijack this cellular channel and launch a variety of attacks. Using knowledge of this threat model, the basic building block to establish end-to-end trust between a pair of mobile devices is the {\em probabilistic one-way trust channel} abstraction offered by MNOs. More precisely: {\em At a given time $t$, if a mobile device with a unique identity $D_i$ is genuinely connected to its MNO $O$ and is weakly authenticated (using SIM authentication) by it; and if any arbitrary sender sends a control message $M$ addressed to $D_i$ which successfully reaches $O$'s network; then $M$ is correctly delivered to the device $D_i$ with high probability.} The delivery (and consequently security) guarantees are probabilistic in that successful delivery is dependent on the premise that the channel to $D_i$ is not subject to MitM threats at time $t$.

The SMI protocol involves repetitive key-exchanges using this probabilistic one-way trust channel. Devices can exchange their keys using a challenge-response protocol from a varied set of locations at different times, providing {\em spatio-temporal diversity}. SMI enables a mobile device (or cloud) to build sufficient trust in the key of another device using a reputation mechanism; higher the user mobility, larger the diversity and hence greater the trust on the corresponding (identity, key) pair. Additionally, we describe how a variant of SMI can quickly authenticate identities using third-party identity verification services for a pair of mobile devices, each of whom consider the other a stranger. 

In short, SMI is a mechanism for augmenting the existing SIM security in a cheap and convenient manner. Security guarantees of SMI can be
significantly enhanced through the use of {\em trusted} locations. With minimal infrastructural change, SMI can obtain such trusted location information from a variety of sources. Specific portions of the protocol can be implemented using alternative paths \footnote{Used interchangeably with channel} which include WiFi access points, data or other proximate physical synchronization points, increasing protocol scalability. We demonstrate the robustness of SMI based on proof of concept testing of secure applications on top of the SMI substrate and detailed analysis of its security properties. In summary, SMI provides a predominantly decentralized protocol to build a strong and secure mobile identity with strong end-to-end trust guarantees in the face of network-level security threats.




==> Eurosys'16/NSDI/10-Related-Work.tex <==
\section{Related work}

Despite the efforts of GSM to enhance their authentication security standards, many of the network security threats of cellular networks continue to remain. Toorani and Beheshti~\cite{toorani2008solutions} outline many of the weaknesses in the GSM authentication layer and propose simple fixes. The GSM specifications team~\cite{arkko2006extensible,haverinen2006extensible} proposed new cryptographic mechanisms to improve upon the early algorithmic vulnerabilities that plagued the original 2G authentication design. UMTS improved upon some of the security threats of the earlier GSM specifications to enhance integrity protection and authentication but even these extensions had several security problems~\cite{mobarhan2012evaluation}. The LTE authentication mechanism~\cite{bikos2013lte} builds upon the UMTS security model and introduces an key derivation hierarchy to enhance the security of the pre-shared keys; even these extensions suffered from several security problems~\cite{bikos2013lte, han2014security,tsay2012vulnerability}. Han and Choi~\cite{han2014security} demonstrate a threat against the LTE handover key management, involving a compromised base station. Tsay et al.~\cite{tsay2012vulnerability} find an attack on the UMTS and LTE AKA protocols using an automated protocol analyzer based on a computational model. Tang et al.~\cite{tang2013analysis} provide a detailed analysis of the security properties and vulnerabilities of different mobile authentication mechanisms.

Device pairing or key setup between two devices has been extensively studied
\cite{balfanz2002talking,castelluccia2005shake,bump,holmquist2001smart,lester2004you}. Specifically, relevant to SMI, we describe a few important secure encounter protocols. SDDR \cite{lentz2014sddr} provides secure encounters whilst enabling secure communication, providing selective linkability and silent revocation. SMILE \cite{smile} is a mobile “missed connections” application, that establishes trust between individuals who have shared a provable encounter. At the site of the encounter, MeetUp \cite{securesocial} proposes a visual authentication scheme using a trusted authority which attests a users public key to its picture. Groupthink \cite{groupthink} provides security primitives for users to count the number of participants and verify Short Authentic Strings (SAS). Secure Location Sharing (SLS) by Adams et al. \cite{clouds}, like SMI, uses multiple communication channels along with contextual question/answer protocols to prevent MitM attacks during device pairing. With the proliferation of WiFi gadgets and sensors that have susceptibility to different forms of MitM attacks, researchers have explored lower-layer signal abstractions to provide security over the wireless channel. Tamper-evident pairing (TEP) \cite{securepairing} is a protocol that provides simple, secure WiFi pairing and protects against MitM attacks without an out-of-band channel. SMI is only built for phones or for devices capable of sending a text message. SMI differs from these protocols in that it focuses establishing trust over the cellular channel building upon the weak authentication layer of GSM without heavy reliance on a PKI.

GAnGS \cite{gangs} exchanges the public keys of group members such that each member obtains the authentic public key of the other. However, continuous physical proximity is required. Moreover, the participant subgroup size can be constrained. SPATE \cite{spate} relies on visual channels and physical interactions. SPATE also requires a number of steps involving potentially inattentive end-users. SPATE was also designed for contact exchange in smaller groups (8 or fewer). Both GAnGS and SPATE enable bystanders to learn contact information, disclosing potentially sensitive private information. Our ephemeral key-pairs and counter-based encryption protect meta-data and ensure forward and backward secrecy. SafeSlinger \cite{safeslinger}, provides a system that leverages prior physical encounters to establish trust. The users communicate to determine a correct sequence that is common to all devices and select it to verify ephemeral keys, preventing users from simply proceeding. Incorporating mandatory verification may sacrifice asynchrony to ensure inattentive user resistance. Our system does not necessitate any pre-cursive encounter with other participants, and runs as a passive background process.

Keybase \cite{keybase} ensures safe retrieval of a particular public key using publicly readable social usernames. Each external service is used to post a signature proving that the account is bound to the named Keybase account. Onename \cite{onename} offers a verified "name" by registering a blockchain ID. Keybase and Onename can be viewed as independent third-party identity verifiers, which can co-exist with the SMI protocol.


==> Eurosys'16/NSDI/11-Discussion.tex <==
\section{Discussion}
\label{ref:disc}

Independent of the results shown in \S \ref{eval}, we stress that the protocol functions in the absence of trusted locations/verifiers. The presence of these entities makes the protocol converge faster due their intrinsic trustworthy nature. This presents an interesting trade-off to be resolved by the end-user: {\em Can we relax our minimal trust assumptions for quicker usability?} The answer is also subject to the application that requires the trusted identity; applications requiring immediate trust require quicker convergence, while those that do not can permit a relaxed rate of growth. We believe that the time required for convergence is acceptable; organizations such as Google and Blockauth require similar timeframes to authenticate identities. We would also like to stress on the fact that most cellular providers in the USA (and other countries) provide unlimited text-messaging feature. This ensures that the number of messages required is not a bottleneck. This protocol is suited to work against a computationally and economically constrained network-level adversary with local scope; an adversary with omniscient network knowledge can repeatedly thwart any attempt to successfully build reputation and will hinder the progress of the protocol. Mitigating such an adversary is not within the scope of this work. For additional details not summarized in the paper, refer to the full technical report \cite{tech}.

%In the interest of space, details pertatining to selection of threshold, key revocation, DDoS alleviation and implementational benchmarks are absent and can be found in the extended version of the paper. 


==> Eurosys'16/NSDI/12-Conclusions.tex <==
\section{Conclusions}

Establishing secure identities in a decentralized manner is a challenging research proposition. In the Internet context, several decentralized solutions have been proposed and yet few have actually been adopted. The key takeaway from this paper is that SMI can augment weaker SIM security, building upon the very same weak authentication layer of cellular networks. 
%To summarize, the SMI protocol provides a repetitive spatio-temporally diverse key-exchange protocol that can quickly establish a high reputation for a self-certifying key generated by a mobile device. 
If SMI is broadly adopted, we believe it has very important ramifications for building end-to-end secure applications for mobile devices. We demonstrate these benefits using sample applications and evaluation of the security properties using standard mobility models. 

%As future work, we plan to build to use the SMI substrate to envision a more secure mobile Internet void of network-level security threats.



==> Eurosys'16/NSDI/2-ProblemSetting.tex <==
\section{Setup and Threat Model}
\label{probsettings}

In this section, we define the problem we set out to solve, establish our assumptions and threat model. We begin by briefly reviewing current GSM authentication and how the SMI protocol augments it.

\subsection{Motivation}
\label{threats}

\noindent{\em Background:} Subscribers of any MNO initially procure a Subscriber Identity Module (SIM) which has a unique International Mobile Subscriber Identity (IMSI) and a shared key required for authentication. The Authentication Center (AuC) of the MNO gains knowledge of this key during SIM registration. The SIM and the AuC use an unidirectional challenge-response protocol to verify the shared key, and establishes a temporary session key for the subscriber.

\noindent{\em Threat Vectors:} However, this asymmetric cellular authentication layer is vulnerable to message interception, phishing, eavesdropping and spoofing, among other threats. One such threat is the use of fake base transceiver stations (fBTSs) to trick the device into connecting to an adversarial (henceforth termed fake) network. Such attacks are fairly easy to execute with the availability of software defined radio platforms that can emulate cellular base (transceiver) station functionality \cite{opencell, openbts, openbsc, usrp, sysmobts, fairwaves}. One possible attack involves the fBTSs exhibiting greater signal strength than the real base station to lure mobile subscribers during their first connection to the cellular network. Another possible attack is to selectively jam specific frequency bands in a local area to force mobile devices to search for alternative base stations, some of which could be fake. 

Forcing a mobile device to connect to a fake network exposes it to a myriad of network-level threats. Meyer et al. \cite{germany} show a MitM attack on Universal Mobile Telecommunications Systems (UMTS) by exploiting the lack of integrity protection in the base stations. Kostrzewa et al. \cite{thesis} exploit weaknesses of the A5/2 \cite{comp128} cipher to demonstrate another MitM attack. The A3 and A8 algorithms used by cellular networks, specifically COMP128 and COMP128-1, are known to have flawed implementations which make it easier for network adversaries to launch MitM attacks against \cite{toorani2008solutions}. Another attack is for the fBTS to use known ciphertext attacks \cite{kca} to recover the session keys without disrupting the original subscriber authentication process \cite{barkan2003instant}. Given physical access to a SIM card, there have been attacks that can recover the shared key embedded in the SIM through effective challenge-response mechanisms. Extensions of these attacks have facilitated over-the-air (OTA) cracking of shared keys \cite{nohl,mathur2008radio}. 
%Refer to Appendix \ref{netsec} for more threats.

\subsection{Problem Definition}
\label{definition}

SMI aims to establish an end-to-end secure channel between a pair of mobile devices in a decentralized manner. The problem can also be modified to build trust between a mobile device and a cloud service provider. Both problems require building upon the weak authentication mechanism provided by cellular networks. To elaborate further, consider mobile devices $U_1$ and $U_2$ with unique identities $D_1$ and $D_2$. $U_1$ and $U_2$ generate their own self-certifying \footnote{Complete certification is achieved as trust grows} public keys $PK_1$ and $PK_2$ and their corresponding private keys. Our goal is to achieve secure key exchange between $U_1$ and $U_2$ in the face of network adversaries who may try to disrupt this process. To state succinctly, $U_1$ has to learn the identity-key mapping $(U_2, PK_2)$ and likewise for $U_2$. With SMI, we aim to achieve two properties:

\textbf{Robustness of Key Establishment.} A combination of user and device IDs creates a certified identity as a consequence of repetitive spatio-temporally diverse interactions. This identity requires substantial (computational and economic) expenditure to forge.

\textbf{Scalable Key Exchange.} The protocol scales with the number of participating users. 

\subsection{Adversary Model}
\label{admodel}

Any user can be in the presence of a local network adversary at a particular location. The adversary can create an fBTS to monitor and alter any or all communication relayed through it \cite{stхhlberg2000radio}. With its devices, the adversary can overhear, intercept, and inject any wireless communication. The adversary can also jam specific signal frequencies. We assume that there is reasonable bootstrapping cost associated with setting up the equipment. Hence, we assume that the adversaries are not omnipresent with respect to the locations the user moves to. For practical considerations, we assume that the adversary will neither follow the user to more than $k$ locations, nor will follow any mobile user continuously. We also assume that the adversary is computationally bounded and would require reasonable amount of time (at least few hours \cite{dunkelman2010practical} to few days) to cryptographically break the weak authentication layer of GSM. Therefore, a new mobile subscriber who may immediately be subject to an attack by an adversary has sufficient time to establish and partially prove its self-certifying identity, unless it is subject to denial of service.



==> Eurosys'16/NSDI/3-StrawMan.tex <==
\section{Overview}
\label{smprot}

In this section, we present an overview of the SMI protocol. We begin by discussing the assumptions required to support our protocol, followed by explanation of the various components that constitute it. We base our discussion on the case where pairs of mobile devices authenticate their identities with respect to each other, but similar arguments can be made for a mobile device authenticating its identity to the cloud.
 
\subsection{Assumptions}
\label{powt}

The SMS channel operates over the same control channel used for authenticating mobile subscribers. Given the weak authentication mechanism currently in place, the SMS channel can be viewed as a {\em probabilistic one-way trust (POWT) channel} (as defined in \S \ref{intro}). This pragmatic assumption is critical to successful execution of the protocol. We also make the following assumptions, which naturally lead to the construction of the POWT channel assumption. First, we explicitly assume that the cellular service provider and mobile device is trusted. The SMI protocol primarily deals with network-level adversaries who aim to seize the cellular channel to launch MitM attacks. Second, we assume that the shared key present in the SIM issued by the cellular provider is not compromised at the time of issue. If adversaries have the capability to issue their own pre-authenticated SIM cards, then the POWT channel assumption does not hold. Third, we assume that SMS is delivered with high probability as the network layer inside a cellular network is not tapped or tampered internally, barring the last-hop where it is exposed. 

\subsection{Protocol Summary}
\label{basic}

The SMI protocol is a repetitive key-exchange that utilizes user mobility across different locations and time to incrementally establish trust over the POWT (SMS) channel. For the adversary to achieve success, it (in the form of an fBTS) has to be in the vicinity of the mobile device (or cloud provider) at all times. Assisted by this locality constraint placed on the adversary, successful spatio-temporally diverse key-exchanges stipulates an exponential decrease in the ability of an adversary to spoof an (identity, key) pair. Each mobile device participating in the SMI protocol computes a reputation score for every mobile device that it exchanges keys with, where the reputation grows with increased location diversity and number of exchanges. Similarly, the trusted cloud provider builds a reputation of participating devices based on the combination of their unique mobile footprint and device identities using the key-exchange protocol. The security guarantees of the SMI protocol strengthen with increase in the reputation score. 

\vspace{1mm}
\noindent{\bf Mobile To Mobile:} To explain in detail, one user termed the {\em initiator} calculates the reputation score of a participant across discretized time intervals called {\em epochs}. Successful key-exchanges, initiated both periodically and aperiodically across an epoch comprise of trading a signed digest (for verifying message integrity) and an encrypted tuple (ensuring information privacy). The tuple consists of spatial and temporal information coupled with user and device identities. The reputation score is increased when there is adequate diversity in location information and time. When the reputation score reaches a predefined threshold, the identity of the participant is authenticated with respect to the initiator. 

\vspace{1mm}
\noindent{\bf Cloud To Mobile:} This variant is an extension of the previous case. The cloud provider both periodically and aperiodically probes the mobile device for the information tuples, across multiple epochs. Succesful probing results in the growth of the reputation of the device in the eyes of the provider. The key differences with the earlier discussed variant stem from the fact that the cloud provider is trusted, and does not require to prove the mapping between its identity and the keys it uses. It is also important to note that providers are often static (or immobile), in safeguarded locations.

\vspace{1mm}
To maintain a healthy reputation score across each epoch, messages specially tagged for the SMI protocol are repeatedly exchanged in the background over the SMS channel. Running in the background reduces the amount of user intervention thereby increasing the usability of the system. 

\subsection{Spatial Diversity: Location Information}
\label{location}

Mobility ensures that the required geo-diversity is obtained for successful reputation growth. Mobility also enables a user to potentially move outside the range of an adversary. The other component required for spatial diversity, {\em location}, has two major components, namely:

\textbf{Untrusted Locations:} 
%As discussed earlier in \S \ref{smprot}, location plays a pivotal role in facilitating growth of reputation. 
This can be obtained from various sources such as location sensors on mobile devices, GPS, cell towers or other external sources (such as an access point) but these locations, by definition are non-certifying and are easy to forge \cite{tippenhauer2011requirements}. 
%This is further explained in detail in Appendix \ref{usage}.

\textbf{Trusted Locations:} Location information obtained from the sources listed above can be modified or forged. The security, and convergence time of the SMI protocol can substantially improve using time-certifying trusted locations. This certification by an accredited party increases credibility of the location and hence contributes greater towards the score calculation. The different ways of obtaining trusted location information are:
\vspace{-2mm}
\begin{itemize}
\itemsep-0.23em 
\item {\em Trusted GPS Sensors:} Phones could easily be embedded with trusted GPS sensors with pre-certifying keys that can provide time-certifying locations \cite{saroiu2010sensor}.

\item {\em Trusted Identity Verifier:} Recent proliferation of mobile payment systems such as Android Pay or Apple Pay can be used to provide a signed time, location contract. 

\item {\em Trusted BTS:} We envision that by imposing (minimal) hardware changes using trusted co-processors \cite{yee1995secure}, location information from BTS' can be used to verify the location, even during handoff.
\end{itemize}
\vspace{-2mm}

\subsection{Temporal Diversity: Epochs}
\label{time}

An epoch is a discrete, fixed-length time interval, usually in the order of hours. We select this specific duration of time as any adversary will require at least few hours to break the weak GSM authentication. We define an \textit{interaction} as user $U_1$ sending a message to user $U_2$ (or provider $P$), within an epoch. The duration of each interaction is finite and upper bounded. Thus, the number of interactions that can occur in an epoch is also finite. An interaction is \textit{successful} if it hasn't been interfered with by the adversary, through denial of channel or interception. This measurable nature of an interaction allows for revocation mechanisms in case of failure. In an epoch, the initiator begins interactions with other participants in both periodic and aperiodic manners. This aperiodicity or \textit{random probing} prevents an adversary from using knowledge of protocol periodicity for malicious intents. The reputation score is built by successful interactions across multiple epochs. If a user is inactive for more than half an epoch, successful interactions in that particular epoch do not contribute towards the calculation of the reputation score. Thus, an epoch can either complete successfully or abort, with no transient state in between.


\subsection{Reputation Score}
\label{score}

An important concept required for this score computation is that of a {\em zone}, which is defined to be a geographic region with a fixed boundary. A fundamental assumption is movement between zones entails much higher mobility than movement within a zone. The reputation score can be computed as a linear combination of scores from various components, including: (i) weights associated with both trusted and untrusted locations, (ii) third-party identity verifiers providing proofs of identities, (iii) temporal diversity in key-exchanges, and (iv) other meta-factors including node priority (defined in \S \ref{eval}). We believe that this formulation (discussed in detail in \S \ref{reputation}) necessitates user mobility which reduces the likelihood of an attack, and thereby increases the credibility of a user's identity. A threshold is chosen based on the user's mobility model, and frequency of adversarial interference. In essence, this threshold should ensure that the reputation of a user grows at a favorable rate independent of moderate adversarial interference, such that reaching the threshold implies that the user has reasonably mitigated threats from an adversary.

==> Eurosys'16/NSDI/4-SMIProtocol.tex <==
\section{Key-Exchange Protocol}
\label{scp}

In this section, we describe the key steps in the SMI key exchange protocol across epochs where pairs of mobile users sign spatio-temporally diverse tuples of information using self-generated, self-certifying key-pairs.

\vspace{1mm}
{\bf Three-Way Handshake:} The basic building block for SMI is a simple variant of the standard challenge-response mechanism used to establish a connection between two participating entities.  The initiator ($U_1$) and participant ($U_2$) with corresponding device identities $D_1$ and $D_2$ generate key-pairs ($PK_{1},QK_{1}$) and $(PK_{2},QK_{2})$ respectively. $U_1$ and $U_2$ exchange their public keys $PK_1$ and $PK_2$ with a challenge-nonce $c_1$ and a response-nonce $c_2$ and corresponding signatures $S_1(.)$ and $S_2(.)$. Each subsequent key-exchange is associated with a (location, time) pair. These subsequent three-way handshakes can be represented as:
\vspace{-2mm}
\begin{align*}
\textbf{1}.&& \quad U_1 \rightarrow U_2: & f_{PK_2}(L_{1},t_1,U_1,D_1,c_1) \\
\textbf{2}.&& \quad U_2 \rightarrow U_1: & S_2(c_1), f_{PK_1}(L_{2},t_{2},U_2,D_2,c_2,c_1) \\
\textbf{3}.&& \quad U_1 \rightarrow U_2: & S_1(c_2),f_{PK_2}(c_2)
\end{align*}

where $f_{PK_1}$ and $f_{PK_2}$ represent standard public key encryption function, and $S_1(.)$ is a standard signature. Additionally, $(L_1,t_1)$ and $(L_2,t_2)$ represent location time pairs. Issues raised by the rare event of message delivery failure can be resolved using standard retransmission techniques; delivery failure after certain number of retransmissions results in abort for the epoch.

\subsection{Using Untrusted Locations}
\label{dp}

In an epoch, a pair of devices {\em consistently} interact; at the start of an epoch, the users create and exchange seeds which inter-link subsequent interactions within the epoch. We label these seeds to be exchanged as {\em random parameters} and refer to this stage of the protocol as the {\em dialing phase}. This is followed by a {\em connection phase} where there is a repetitive exchange of keys with varied (location, time) pairs.

To elaborate, each epoch begins with users $U_1,U_2$ generating random parameters $a,b \in N$ respectively. These parameters assist in ensuring consistent interactions, defined to be a challenge-response mechanism with the Markov property i.e. the response at any time
$t_{m}$ depends only on the interaction at time $t_{m-1}$. Additionally, for any particular epoch, all further interactions between the users contain {\em incremental signatures} where every signature in an interaction $m$ builds upon the signature in interaction $m-1$. Random parameters $a$ and $b$ are repetitively used as challenge-response nonces for each such signature. %A tuple of information consists of a combination of location information, time information and user, device identities. 
After the dialing phase, both users are familiar with both $a$ and $b$. This is followed by $k$ two-way key exchanges, where at the $2i^{th}$ iteration, $U_1$ sends a signature $S_{2i}(a||S_{2i-1}(.), L_{2i},t_{2i})$ and $U_2$ responds with $S_{2i+1}(b||S_{2i}(.), L_{2i+1},t_{2i+1})$, where $||$ denotes concatenation. 
%Presence of the signature from the previous interaction enforces connectivity within an epoch. %In this context, $a||b||..$ denotes an concatenation based on the number of the iteration (i.e. $2i+1$ for $S_{2i+1}$). For example, if the number of the interaction is $3$, $a||b||..$ is $a||b||a$. The maximum length of the string $a||b||..$ is fixed to be some constant $l_{max}$ and this is maintained using a sliding window of the same size. The window begins to slide once the string length exceeds $l_{max}$, with each successful interaction. 
Hence all the signatures in an epoch are connected and an adversary who has to disrupt has to participate in an entire epoch, right from its inception. The exact key exchange steps in an epoch are outlined below. It is important to note that signatures are indexed by the interaction number. All odd numbered signatures in the dialing phase are generated by user $U_1$. However, in the connection phase, odd numbered signatures are generated by user $U_2$.
%\textbf{} & \quad U_2 \rightarrow U_1: f_{PK_1}(L_{2},t_{2},U_2,D_2,b,S_{init})\\
\vspace{-1mm}
\begin{align*}
\textbf{} & \quad ~\textbf{Dialing Phase:} \\
\textbf{1}.& \quad U_1 \rightarrow U_2: f_{PK_2}(L_{1},t_{1},U_1,D_1,a) \\
\textbf{2}.& \quad U_2 \rightarrow U_1: S_2(a),f_{PK_1}(L_2,t_2,U_2,D_2,b,a)) \\
\textbf{3}.& \quad U_1 \rightarrow U_2: S_3(b||a),f_{PK_2}(b) \\
\textbf{} & \quad ~\textbf{Connection Phase:} \\
\textbf{} & \quad ~\text{$For$ $steps$ $4,5$; $\forall$ $i: i = 2$ to $k+1$} \\
\textbf{4.1} & \quad U_1: S_{2i}(.)= S_{2i}(a||S_{2i-1}(.), L_{2i}, t_{2i}) \\
\textbf{4.2} & \quad U_1 \rightarrow U_2: S_{2i}(.),f_{PK_2}(L_{2i},t_{2i},U_1,D_1,S_{2i}) \\
\textbf{5.1} & \quad U_2: S_{2i+1}(.) =S_{2i+1}(b||S_{2i}(.), L_{2i+1}, t_{2i+1}) \\ 
\textbf{5.2} & \quad U_2 \rightarrow U_1: S_{2i+1}(.),f_{PK_1}(L_{2i+1},t_{2i+1},U_2,D_2,S_{2i+1})\\ 
\textbf{6}.& \quad ~\text{If all $k$ exchanges are successful} \\ 
\textbf{} & \quad U_1: IncreaseRep(D_2, PK_2)\\
\textbf{} & \quad U_2: IncreaseRep(D_1, PK_1)\\
\end{align*}
\vspace{-6mm}

%The dialing phase is a minor modification of the earlier explained three-way handshake to include the random parameters to be exchanged. 
During the connection phase, each interaction between $U_1$ and $U_2$ is initiated both periodically and aperiodically. The former is done to ensure devices have sufficient mobility; the latter to ensure randomness in an epoch exchange, reducing any advantage an adversary could have gained using the knowledge of periodicity. The adversary can forge the identity of the initiator and randomly start another epoch, taking undue advantage of this aperiodicity. We ensure that this is avoided by sending a special tag at the end of the ongoing epoch with consistent interactions. The inception of a new epoch will be approved by the participant only on receiving this tag. An adversary attempting to decrypt the secure and consistent interaction between the users at a time $t_i$ ($i \textgreater 0$) would have to possess knowledge of the random parameters which effectively serves as an increment counter. The probability that the adversary can correctly guess both parameters is very low ($\approx 1/|2^N|^2$) where $N$ is the number of bits in the key space, making it practically impossible to disrupt the epoch except forcing the mobile devices to abort the epoch. Spoofed messages sent by the adversary are \textit{inconsistent} with the ongoing interactions and this alerts the users of its presence in the communication channel. Upon successful completion, both parties enhance their reputation of the individual identities ($IncreaseRep(.)$) while an abort does not have a negative outcome.

\subsection{Using Trusted Locations} 
\label{tl}

The previous version of the protocol was specifically for untrusted locations. In \S \ref{location}, we discussed different types of third-party providers or physical interactions that can provide a notion of trusted locations with verifiable time-bound signatures. Consider one such provider $X$ who has an independent PKI rooted infrastructure \cite{herzberg2000access}. $X$ has a wide distribution of trusted device end-points where each device is embedded with (a) key-pair generated by the root $X$, and (b) corresponding trust certificate from the certificate root of $X$. In addition, each device has a trusted GPS sensor that provides the location $L$ of that particular device. Thus, this {\em donor} device is
equipped to provide a trusted signature $s(L,t)$ to any interacting device. This signature also encompasses the trust certificate of the donor from the root $X$. If one trusts the public key of the root of $X$, then the location signature $s(L,t)$ is a verifiable proof. Except the case of trusted GPS sensor within each mobile device, protocol participating devices obtain these trusted location through physical proximity-based interactions with the donor device. In SMI, we impose that the integrity of this signature persists over the time to live (TTL) window $\Delta_i$ from the moment it was exchanged (say $t_i$) i.e. exchange $i+1$ should be initiated at $t_{i+1}$ such that $t_{i+1} \leq t_i + \Delta_i$. Most mobile devices which connect to the genuine cellular network receive time updates from the network; hence an assumption about minimal time synchronization errors across participating devices and trusted location endpoints is pragmatic. Borrowing terminology from \S \ref{scp}, consider the following example of a three-way handshake (dialing phase) between user $U_1$ and trusted third-party $T$, where $\Rightarrow$ denotes communication using a close-proximity (eg. NFC) channel: 

%The basis of the trusted location key-exchange is that any location information $L_i$ (which is a part of the $i^{th}$ exchange) is associated with a verifiable proof of that location, $s(L_i, t_i)$. Except the case of trusted GPS sensor within each mobile device, protocol participating devices obtain these trusted location through physical proximity-based interactions with the donor device. Any trusted location signature is associated with a limited time value. To successfully utilize this signature in the reputation calculation, the next exchange should be within the TTL window of the signature i.e. exchange $i+1$ should be initiated at $t_{i+1}$ such that $t_{i+1} \leq t_i + \Delta_i$. Borrowing terminology from \S \ref{scp}, consider the following example of a three-way handshake (dialing phase) between user $U_1$ and trusted third-party $T$, where $\Rightarrow$ denotes communication using a close-proximity (eg. NFC) channel:
\vspace{-2mm}
\begin{align*}
\textbf{1}.& \quad T \Rightarrow U: f_{PK_U}(s(L_{T},t_{T}),U_T,D_T,c_1) \\
\textbf{2}.& \quad U \rightarrow T: S_U(c_1),f_{PK_T}(L_U,t_U,U_U,D_U,c_2,c_1)) \\
\textbf{3.1}.& \quad T \rightarrow U: S_T(c_2) \\
\textbf{3.2}.& \quad T \Rightarrow U: f_{PK_U}(c_2) \\
\end{align*}
\vspace{-6mm}

An alternative variant ensures that before providing a trusted location signature $s(L_T,t_T)$ in step $1$, the external location provider can perform an independent three-way handshake with the mobile device in physical proximity to it, where the external trusted location synchronization point uses the SMS channel to verify the authenticity of the device identity $D_U$. In other words, the trusted location provider can use an independent network interface to send the challenge over the SMS channel instead of Bluetooth or NFC channel. Thus, the trusted location provider verifies the interacting device identity $D_U$ subject to the POWT Channel assumption. An even stronger variant would be for the location provider to provide $s(D_T, L_T, t_i)$ where it provides a device specific time-bound location signature. 

\subsection{Using Multiple Channels}
\label{multi-path}

Another simple, but extremely useful variant of the key-exchange protocol is to leverage multiple communication channels during an epoch: SMS, data channel, WiFi, Bluetooth etc. Though the SMS channel is integral for the POWT Channel assumption to hold, it is severely inhibited by its 160 character limit. To partially alleviate load on the SMS channel, we can use alternative channels to offload non-critical data and use it to only send the challenge-response information. One cannot completely bypass the use of the SMS channel for challenge or response messages since that is the only channel that is directly connected to the identity of the mobile device participating in the protocol. This variant of the protocol can help in significantly reducing the number of SMS messages that we need to exchange to establish trust with other devices. 

\subsection{Validation With The Cloud} 
\label{cv}

This version of the protocol specifically discussed the issue of bootstrapping trust with a cloud service provider $P$. The key technical details, especially the random probing component, remain the same; minor variations arise due to the following reasons: (a) The cloud service provider has a fixed location i.e. $L_P$ never changes (as in \S \ref{tl}). This location is often not disclosed to the public to ensure secrecy, ergo providing better protection, (b)  The cloud service provider also has access to a cellular channel with much larger bandwidth than conventional cellular devices, partially mitigating any DoS attack attempts, and (c) The cloud service provider is trusted. It does not have to prove the authenticity of its (identity, key) mapping. It is pragmatic to assume that the cloud is equipped to quickly deal with any infrastructural failures, and proactively defend threats against it. Borrowing previously used terminology, the connection phase of the protocol can be summarized as follows: 

\vspace{-2mm}
\begin{align*}
\textbf{1}.& \quad P \longmapsto U: f_{PK_U}(.) = f_{PK_U}(s(L_{P},t_{P}),U_P,D_P) \\
\textbf{2}.& \quad U \rightarrow P: S_U(f_{PK_U}(.)),f_{PK_P}(L_U,t_U,U_U,D_U)) \\
\textbf{3}.& \quad P \longmapsto U: f_{PK_U}(.) = f_{PK_U}(s(L_{P},t_{P}),U_P,D_P) \\
\textbf{4}.& \quad U \rightarrow P: S_U(f_{PK_U}(.)),f_{PK_P}(L_U,t_U,U_U,D_U)) \\
\end{align*}
\vspace{-6mm}

where $\longmapsto$ denotes a random probe by the cloud server. This variant is particularly useful, when the cloud can host an identity verifier (explained in \S \ref{tpiv}). It is important to note that across all the variants discussed, the variable used to denote time, $t$, varies with each step. 


==> Eurosys'16/NSDI/5-Reputation.tex <==
\section{Reputation}
\label{reputation}

In this section, we further discuss the various components associated with the reputation score. We also discuss obtaining the threshold above which the identity is considered to be reputed, the security guarantees we provide and a quick mechanism to bootstrap reputation using a trusted third-party identity verifier. 

\subsection{Reputation Score Formulation}
\label{formulation}

To begin formalizing the reputation score in detail, let the duration of epoch $i$ be represented by $[t^i_{0},t^i_1]$ where $t^i_{0}$ is the time at inception of epoch $i$ and $t^i_1$ is time at its conclusion. The score for user $U$ at time $t \in [t^i_{0},t^i_1]$ is given by:

\vspace{1.5mm}
\framebox{\large {\centerline{\textbf{$R_U(t,i)$ = $\gamma.f_1(t,i)$ + $\delta.f_2(t)$}}}}

\vspace{1mm}
\begin{itemize}[leftmargin=-.01in]
\itemsep-0.23em 
\item $f_1(t,i)$=$\alpha.(m(t,i))$+$(1-\alpha) .f_1(t^{i-1}_1,i-1)$; smoothing factor $\alpha \in (0.5,1)$ and $i \ge 1$ such that

$m(t,i)$=$c_1.m_1(t,i)$+$c_2.m_2(t,i)$; $c_2 \textgreater c_1 \textgreater 1$, where (a) $m_1(t,i)$ denotes the number of \textit{successful} interactions in the time interval $[t^i_{0},t]$ due to untrusted locations, and (b) $m_2(t,i)$ denotes the number of \textit{successful} interactions with \textit{unique} trusted locations in the same interval. 

\item $f_2(t)$ is a cumulative score associated with the total number of proofs of identity from third-party identity verifiers in the time period $[t^1_{0},t]$ (explained in \S \ref{tpiv}). 

\end{itemize}
\vspace{-2mm}

We set $\alpha \in (0.5,1)$ to provide greater weightage to current transactions compared to historical transactions. We also set $c_2\textgreater c_1$ to provide greater credibility for trusted locations over untrusted locations. The notion of {\em unique} trusted locations provides verifiable proof of user mobility between these locations. Additionally, we view the reputation contribution due to third-party identity verifiers to be larger and hence, the contribution of function $f_2$ outweighs that of $f_1$. This is enforced by constants $\delta \textgreater \gamma$. 
The reputation score after $q$ epochs, $R=X_U + Y_U$ where:

\vspace{2mm}

{\large \centerline{\textbf{$X_U = \alpha.\gamma.\sum_{i=1}^q [(1-\alpha)^{q-i}].m(t^i_1,i)$}}}

\vspace{2mm}

{\large \centerline{\textbf{$Y_U = \delta.f_2(t^q_1)$}}}

\vspace{3mm}
%$X_U$ represents the total reputation gathered across epochs using untrusted locations and trusted locations excluding trusted third-party identity verifiers which is captured by $Y_U$.


\subsection{Management \& Scheduling}
\label{manager}

The number of messages that a mobile device can send is restricted because of cost factors and the network load. Each device leverages the multiple channels available at its disposal to reduce message overhead by transmitting non-critical information using alternative channels which are less constrained (in terms of content size) than the SMS channel. Every device has an inbuilt reputation manager that tracks the reputation of all the user identities in the address book. Additionally, SMI measures the frequency of interaction between users to determine the importance level (priority) of users in the contact list. Users can also pre-specify importance level of other users in their contact list. 

{\em Scheduling:} Based on the importance of a user, their reputation score, and threshold, SMI uses a simple optimization mechanism to determine an {\em active list} of recipients with which SMI will enter into a new epoch of key-exchanges. Given a limited message quota for a time period (characterized by costs), the schedule optimization mechanism orders messages based on the highest utility metric of user priority i.e. important users are to be bootstrapped faster. Once an initiator commences an epoch, it makes sure that it gives precedence for all message exchanges within the epoch even if it may slightly over-run the specified message quota. The reputation manager performs the important function of scheduling to achieve the dual goals of reducing message costs and maintaining the reputation levels of important mobile users in the address book. Apart from minimizing cost, this optimization provides an additional benefit of reducing cellular network load whilst producing the same guarantees with respect to security and score growth. 

\subsection{Security Guarantees}
\label{threshold}

An adversary is bound by the following constraints in the SMI protocol: First, any adversary that aims to hijack an identity has to generate its own key-pair for the identity. To be able to leverage the forged key-pair, the network adversary has to be in continuous proximity of the mobile device and completely prevent any communication between the device and the cellular network. This kind of adversarial behavior is severe and assumed to be infrequent. Second, if the adversary aims to hijack an identity before the device participates in the SMI protocol, then the device can generate a conflicting self-certifying key (discussed in \S \ref{extensions}) which forces the cellular network to abandon/reject the SIM used by that device. Third, an adversary aiming to hijack any epoch must obtain the random parameters exchanged at the beginning of the epoch, an event that occurs with very low probability. Outside of these options to hijack the channel, the easier strategy for the adversary is to jam specific exchanges in an epoch, enough to facilitate epoch abortion. This may at best, delay the establishment of a sufficient reputation score between an initiator, participant pair. All these factors clearly indicate the difficulties an adversary faces in disrupting the SMI protocol over every epoch. 

\vspace{1mm}
Consider a scenario where a network adversary disrupts a particular channel with a small probability $p$. Assuming no collusion between various adversaries, the probability that the user's communication is disrupted across $k$ locations (under the coverage of distinct cell towers) is $p^k$. The adversary controls a fraction of the the cell towers (locations) that the user frequents. We assume that even in the extreme case where the user frequents all cellular towers (of size $n$) within a region, the adversary can control upto half these towers i.e $k \leq n/2$. We also assume that the adversarial nodes are operating in the {\em always on} mode, to immediately detect and hinder any user activity. The value of $p^k << 1$ for larger values of $k$. Thus, with increased mobility, we are able to ensure that the adversarial interference is minimal with high probability (assuming the adversary does not actively follow the user). 

\vspace{1mm}
However, human mobility patterns can be predicted with high precision, and are often repetetive. The adversary can utilize this historical knowledge to strategically position his fBTS nodes to hinder user activity most effectively. For example, the adversary may utilize knowledge that the user is at work for nearly a quarter of his day (nearly $6$ hours), and place a node in the vicinity. As explained earlier, the adversary can combine a DoS attack and identity forgery to build reputation on behalf of the user. However, since the adversary is (economically) constrained to a few locations, the user is notified of its presence once he is not within adversarial proximity. To aleviate the degradation caused by the adversary, the user is presented two options: (a) Slowly build trust through alternate channels till he is out of the vicinity of the adversary, and (b) Visit trusted third-party verifiers (refer \S \ref{tpiv}) to quickly bootstrap trust. 

\vspace{1mm}
With each successful interaction in this period, the reputation score of the participating users grow, building confidence in their identities. To account for reputation decay and to maintain liveliness, nodes need to periodically perform key-exchanges to preserve their reputation above the threshold.

\subsection{Third-Party Identity Verifiers}
\label{tpiv}

A {\em third-party identity verifier} represents a specific variant of the SMI protocol where one of the end-points participating in the key-exchange protocol is not a mobile device but a cloud-based service (such as Keybase, Onename) that maintains reputation gained by a mobile device. A third-party identity verifier can be thought of as a simple datastore that maintains a history of all prior interactions of a device. Any external cloud-based entity can function as a third-party verifier and one can imagine an ecosystem with multiple such verifiers. As this third-party is trusted, a participating device can quickly build its reputation utilizing (historical) information contained. During key exchange, the verifier randomly probes the honest user at different time periods to ensure that the user does not behave erroneously under the influence of a network adversary. 

We envision the following trusted third-party providers to be used in the quick bootstrap process: (a) Cellular Providers like AT\&T, Sprint and Verizon; (b) Independent third-parties like Verisign, Keybase and Onename; (c) Trusted wallet providers like Google, Apple and Mastercard. There are several important use-cases for such third-party verifiers. First, each cellular network can run their own instance of the verifier. This enables the cellular network
to quickly learn the self-certifying key of its mobile users. With sufficient information, the cellular network has essentially established a decentralized PKI for all its mobile users. Consequently, this enables the cellular network to quickly detect SIM cards that may be subject to attacks by network-level adversaries as they present conflicting information. Second, third-party verifiers who are popular and potentially trustworthy can help a pair of mobile users to quickly bootstrap trust between themselves. Finally, trusted wallet providers can use the reputation score to create a reliable mapping between wallet identities, user identities and secure mobile identities of devices of users. 

%\subsubsection{Quick Reputation Bootstrap}
%\label{frb}
%
%Consider the case where two devices $U_1$ and $U_2$, as independent initiators, use the SMI protocol with a trusted third-party provider (eg. Keybase, Onename). After successful key-exchanges, both $U_1$ \& $U_2$ build a score, say $R_1$ and $R_2$, relative to this third-party
%and have authenticated their IDs to it. However, these devices have minimal reputation with respect to each other. 
%
%To quickly bootstrap their reputation of the other, two mutually distrusting devices can perform a three-way handshake to first exchange their keys and obtain a proof of interaction with a trusted-third-party (eg. Keybase, Onename) along with their established reputations certifying by the third-party with supporting proofs of historical key exchange interactions. Using this information, the two devices can quickly bootstrap their reputation of each other as a function of the reputation scores and how much the devices trust the third-party verifier. This quick bootstrap function can significantly reduce the number of message exchanges required to bootstrap and maintain reputation between a pair of devices.


==> Eurosys'16/NSDI/6-Evaluation.tex <==
\section{Reputation Score Evaluation}
\label{eval}

In this section, we discuss the various experiments performed, our results for the same and conclude with the key takeaways from our experiments. 
%\end{itemize}

\subsection{Emulation Setup}
\label{setup}

We evaluate the SMI protocol across different mobility models, testing with traces generated by standard mobility models \cite{smooth,citymob}, namely:

\vspace{1mm}
\noindent{\em Simple Traffic:} Models vertical and horizontal mobility patterns without direction changes.

\vspace{1mm}
\noindent{\em Random Walk:} Models unpredictable movement. It is also referred to as Brownian Motion \cite{hida1980brownian}.

\vspace{1mm}
\noindent{\em Probabilistic Random Walk:} This model introduces user-defined probabilistic direction changes.

\vspace{1mm}
\noindent{\em Manhattan Mobility Model:} Nodes move in horizontal or vertical direction on an urban map. It employs a probabilistic approach in the selection of movements. 

\vspace{1mm}
\noindent{\em Downtown Mobility Model:} Adds traffic density to the Manhattan model. Mobility is reduced in predefined downtown areas, where the user is 70\% of the time.

\vspace{1mm}
\noindent{\bf Test Ecosystem:} Our setup comprises of several initiators and participants, totalling $10^4$ nodes. The emulation is run across a $10^{10}$ sq. meter (3861 sq. mile) grid, roughly the size of Los Angeles County, California. In the context of our experimental setup, we define zones to be $10^8$ sq. meter (38.61 sq. mile) grids, totaling $10^2$ different zones. In this setup, each of the $10^2$ zones have a unique distribution of trusted locations. The mean speed chosen for mobility was 14 mph. This was the weighted average value of the speed whilst moving in a vehicle (25 mph) and whilst walking (3 mph), both amidst moderate traffic density. The algorithm chosen as part of the reputation manager is fixed-priority preemptive scheduling \cite{audsley1995fixed}. Any interaction can abort based on adversarial interception of the channel at the location the initiator/participant is at. We set an epoch to be $1$ day in all our experiments, with messages exchanged at an hourly frequency. Therefore, $3$ epochs or nearly $70$ exchanges increases the probability of successful protocol completion to $(1-p)^{70}$. We observe that the average reputation score increase per epoch is $1680$. This produces a corresponding threshold of $5000$ ($1680 \times 3$). Some of the other parameters required to compute the reputation score are explained below:

\vspace{1mm}
{\em Priority:} A manually entered value associated with each participant which indicates its relative importance on the initiator's contact list. Priority ranges from 1 which is the smallest value to 10 which is the largest. As per the scheduling algorithm chosen; in the vicinity of any trusted location, the reputation score of the highest priority nodes is increased.

\vspace{1mm}
{\em Batch:} A uniformly assigned value to each participant creating disjoint participant sets. This ensures that each disjoint set is entitled to score growth uniformly across the entire time interval independent of its priority, thereby preventing stunted score growth. The total number of batches is a function of the number of contacts on the initiator's device.
%\end{itemize}
\vspace{1mm}

\subsection{Composite Mobility Model}
\label{composite}

Due to the volume of data required for evaluation and the difficulty in obtaining anonymized mobility traces, we emulate our experiments using a composite mobility model. This model postulates that the mobility model of each node may change to one of two {\em foreign} models (Manhattan \& Downtown Manhattan) at every six hour interval during a day, but return to its {\em home} mobility model (Simple Traffic) at the start of each day i.e. between 00:00 hours and 06:00 hours, where the node is assumed to be stationary (or mobile in a restricted space). This composite mobility model draws insights from \cite{isaacman2012human,becker2013human,song2010limits,musolesi2007designing} and we believe that this draws some parallels with realistic mobility patterns as it attempts to emulate habitual human mobility. 


\subsection{Results}
\label{results}

%In this section, we discuss our results for the various experiments performed. 

\begin{table}[H]
\centering
\begin{tabular}{| l | l | l | l |}
\hline 
\textbf{Mobility} & \textbf{Low} & \textbf{Nil}& \textbf{High}\\ 
\textbf{Model} & \textbf{(p=0.28)} & \textbf{(p=0)}& \textbf{(p=0.54)}\\ 
\hline

 Simple Traffic & 191 & 150.6 & 229.2\\ 
 \hline
 Prob. Random Walk & 175 & 140 & 212.6\\ 
 \hline
 Random Walk & 100.2 & 79.1 & 122.6\\ 
 \hline
 Manhattan Traffic & 142 & 111.9 & 172.5\\ 
 \hline
 Downtown Manhattan & 119 & 92.5 & 141.3\\ 
 \hline
\end{tabular}
\caption {Average Number Of Exchanges Required}
\label{table:avg}
\end{table}

\noindent{\bf 1. Single Node Score Growth:} To provide visualization of the reputation score growth for a single node with the composite mobility model, we plot two cases: one in the absence and one in the presence of a severely active adversary. Using a scaled down version of the reputation manager (in terms of scoring), Figure \ref{fig:RSG} denotes the growth of the reputation for a node as a function of time, reaching a threshold of $1700$. The baseline case i.e. the absence of any adversarial interference or trusted locations converges in 70 hours. The second scenario where the node is in the presence of an adversary 43\% of the time i.e. the (increased) adversarial interference ($p$) is $0.43$. Thus, the node takes nearly double the time ($136$ hours) to reach the same threshold. In this extreme case where there is stunted growth of the reputation score, the protocol succeeds only because of score growth due to the trusted location distribution, where 1 of every 12 locations visited is trusted. 

\begin{figure}[!h]
  \begin{center}
      \includegraphics[width=.80\columnwidth]{images/foo5.pdf}
    \end{center}
\vspace{-0.1in}
  \caption{\small{Reputation Score Growth}}
  \label{fig:RSG}
 \vspace{-0.1in}
\end{figure}


\vspace{1mm}
\noindent{\bf 2. Number Of Exchanges:} Table \ref{table:avg} reports the average number of exchanges (NOE) required to reach a threshold of $3400$ for each of the mobility models across $10$ independent trials of the experiment and varied adversarial interference, where a subset (of size $100$) of participants are assigned the same priority. The Simple Traffic model has the largest NOE because participants move in a fixed direction, thereby reducing the chances of being in the vicinity of a trusted location frequently. On the other hand, the rate of mobility in the Downtown Manhattan model, while lower in some areas is higher in others. Thus, with increased mobility, the chances of being in the vicinity of a trusted location also increases, thereby lowering the NOE. 

\vspace{1mm}
\noindent{\bf 3. Protocol Convergence:} We emulated key-exchanges at an hourly frequency for a period of 30 days, for all $10^4$ nodes in our experimental setup. For all these experiments, the threshold is set to $5000$. We observe that the time taken to successfully reach the predefined threshold varies based on: 
%(a) mobility (b) adversarial interference (c) number of trusted locations encountered (d) priority and batch of participating nodes. We explain each of them below, with empirical results:

\vspace{1mm}
{\em i. User Mobility:} Figure \ref{fig:cdf} suggests that in the baseline case, a very small fraction of total participating nodes (the bottom 0.0063 percentile) are immobile. We vary the reputation threshold and observe that the percentage of immobile users remains nearly constant across all experiments. The mean convergence time however, varies with the reputation threshold and amount of adversarial interference. For visualization purposes, we represent protocol failure using a convergence time of $190$ hours. We observe that nearly $20$\% of participating nodes fail with the severity of interference.

\begin{figure*}
\centering
\subfigure{
\includegraphics[width=2.2in]{images/foo2.pdf}
\label{fig:cdf}
}
\subfigure{
\includegraphics[width=2.2in]{images/foo7.pdf}
\label{fig:trustedloc}
}
\subfigure{
\includegraphics[width=2.2in]{images/foo.pdf}
\label{fig:PrivsTime}
}

\caption{Aggregate Statistics}
\end{figure*}

\begin{table}[h]
\centering
\begin{tabular}{| l | l | l | l |}
\hline 
\textbf{} & \small{\textbf{Interference}} & \small{\textbf{Convergence}} & \small{\textbf{$\lambda$}}\\ 
\hline
 Baseline & 0 & 70 hrs & 0\\ 
 \hline
 Reduced & 0.11 & 79.37 hrs & 0\\ 
 \hline
 Increased & 0.39 & 89.05 hrs & 25\%\\ 
 \hline
\end{tabular}
\caption {Interference \& Convergence}
\label{table:adv}
\end{table}


\vspace{1mm}
{\em ii. Adversarial Interference:} We performed two sets of experiments, one with {\em reduced} adversarial interference with a maximum probability of 0.28 and another with {\em increased} adversarial interference of maximum probability 0.54. Note that even the maximum value of reduced interference is an overestimation of the actual value as an attack of such scale would require expansive economic resources. We sanction such (large) values to display the endurance of our protocol. We emulated $400$ trials of both experiments along with a baseline case for better comparison. As expected, increased interference affects a larger number of key-exchanges and thus increases the protocol convergence time, sometimes beyond $720$ hours. This increases the percentage of failure ($\lambda$) among participating nodes. On the other hand, reduced interference produces moderate delays towards convergence. Table \ref{table:adv} and Figure \ref{fig:convadv} reflect our claims.  

\vspace{1mm}
{\em iii. Number of Trusted Locations:} Across $400$ trials for a subset of users of size $10^2$ in the baseline case, we observed the impact of trusted locations towards protocol convergence. We achieved this by plotting the average convergence time against the number of trusted locations. Since the quick growth of reputation hinges on an increased number of such locations or cloud-based providers, we observe an expected direct correlation between the two parameters in Figure \ref{fig:trustedloc}. The small slope is due to the variation in trusted locations across zones; some have greater densities than others, and due to repeatedly visiting the same trusted location in a predefined window (of size 2 days in our experiments) disregarding the constraint for {\em unique trusted locations}.

\begin{figure}[h]
  \begin{center}
      \includegraphics[width=.80\columnwidth]{images/foo12.pdf}
    \end{center}
\vspace{-0.1in}
  \caption{\small{Convergence vs Adversarial Interference}}
  \label{fig:convadv}
 \vspace{-0.1in}
\end{figure}

\vspace{1mm}
{\em iv. Priority \& Batch of Participating Nodes:} The large scale emulation for $10^4$ nodes with reduced adversarial interference (p=0.28) was segregated and the convergence time was visualized as a function of the priority of the nodes. Since the reputation manager employs fixed priority scheduling, the protocol convergence time is inversely proportional to the priority of the participating nodes as in Figure \ref{fig:PrivsTime}. Outliers may exist in this plot because of two reasons, one being a cyclic-batch-wise score update module we have implemented as part of the reputation manager. This module ensures that no subset of nodes is starved for score updates due its reduced priority. The other reason is a module that reduces the maximum priority used as part of trusted-location based score increments. This reduction is done in a cyclic fashion in a periodic manner. However, these outliers have been normalized due to repeating this experiment $400$ times to account for sufficient randomness in batch, priority across nodes and adversarial interference, number of trusted locations across the emulation test-bed. By increasing the contribution due to trusted locations module, we can further increase the slope.  


\begin{figure}[h]
  \begin{center}
      \includegraphics[width=.80\columnwidth]{images/foo8.pdf}
    \end{center}
\vspace{-0.1in}
  \caption{\small{Quick Reputation Bootstrap}}
  \label{fig:qrb}
 \vspace{-0.1in}
\end{figure}


\vspace{1mm}
{\em v. Quick Reputation Bootstrap:} To emulate this phenomena (explained in \S \ref{tpiv}), we computed the reputation score with the trusted third-party and without (i.e. baseline case) but increased the key-exchange frequency to $40$ minutes. This frequency increase increases the baseline convergence because the average mobility (ratio of distance actually covered to the distance that can be covered) of nodes is lesser at a $0.67$ hour frequency when compared to an hourly frequency. From Figure \ref{fig:qrb}, we observe that the quick reputation bootstrap is faster by a factor of $80$, from $84$ hours to $1$ hour, highlighting its impact towards score growth. This decrease by nearly $1.9$ orders of magnitude is non-trivial, but comes with an implicit caveat. Staleness of the information at the third-party provider should be carefully measured.


%\subsection{Key Takeaways}
%
%\noindent{1.} Using Monte Carlo methods in our setup with $10^4$ nodes, only the bottom $0.0063$ percentile of users, on average, are immobile. 
%%A majority converge on time; only the top $20$ percentile experiencing abnormal delays.
%
%\noindent{2.} In an increased adversarial interference scenario, the protocol takes 27\% longer to converge. However, this extreme form of attack is highly unlikely. %In the reduced (yet overestimated) interference setup, the protocol always converges.
%
%\noindent{3.} As expected, the protocol converges faster with an increase in number of trusted locations and nodal priority. This is a consequence of our design decisions.
%% (\S \ref{setup}).
%
%\noindent{4.} The presence of quick reputation bootstrap reduces convergence time by nearly two orders of magnitude. This non-trivial improvement is very helpful in scenarios where users have limited time to establish trust.


==> Eurosys'16/NSDI/7-Implementation.tex <==
\section{Applications}
\label{impl}

Our implementation of the SMI protocol is on top of the Android platform. The devices used in our implementation were Samsung Galaxy Young (GT-S5360) phones with Android v2.3.6. Standard APIs such as Bouncy Castle Java cryptography were used for cryptographic operations, with a key length of 2048 bits. Our implementation emulates physical synchronization with a trusted location using Bluetooth. 

\vspace{1mm}
\noindent{\bf Secure Messaging:} We have implemented a version of secure messaging on Android. On building sufficient reputation, the user can send signed messages to (a selected subset of) its contacts. This application has a SMS receiver component, which filters messages having a SMI header. Based on experiments conducted, we observe that the average time taken to send messages over the Etisalat network is $12.88$ seconds per message especially since encrypted messages will be split across several messages due to the signature length. The actual cryptographic operations consumed less than $0.06$ seconds or 0.4\% of the total time on a mobile device.
%, indicating the simplicity from the efficacy of standard cryptographic techniques used.

\vspace{1mm}
\noindent{\bf Secure Image Transfer:} We first generate a shared AES key and then encrypt the image using it, and transfer the encrypted image over the data channel. Given that a direct data path between mobile devices may not exist, we use an online cloud server as a synchronization point and exchange the data through it. The encrypted version of the shared key and {\em proof} of the file is shared over the SMS channel. This proof is a simple one-way hash of the byte-array of the image generated using SHA-1. On receiving the message, the recipient fetches the encrypted image, decrypts the AES key and then the image, and verifies the one-way hash proof. Based on experiments, we observe that the average time taken for the image transfer application is $27.65$ seconds out of which an average time of $20.42$ seconds was taken to upload the image. This extended period of time for upload is due to asymmetry in bandwidth provided.

\vspace{1mm}
\noindent{\bf Secure Transactions:} We developed an encrypted marketplace where mobile users share their keys using SMI. Then, using an online server as a synchronization point for a marketplace server, participants could place encrypted buy/sell orders. In essence, the central server is unaware of the exact transactions but enables a group of users to execute peer-to-peer transactions securely. The participants obtain three guarantees using SMI: (a) SMI establishes authenticity of the keys of the individual participants; (b) Every order placed in the marketplace was signed by the corresponding buyer or seller which enabled transaction-level trust between participants; (c) Since all transactions were encrypted, the central server could not learn much information about the individual transactions but could learn statistical patterns on the number of requests from each identity.


==> Eurosys'16/NSDI/8-Extensions.tex <==
\section{Additional Considerations}
\label{extensions}

\noindent{\em Registering a new device:} Each cellular network can run their own key verification service where the device can generate its self-certifying key and initiate key-exchange with a {\em verifier} of the cellular network. This scheme of registering the user-generated public key on the cellular provider provides an expedited detection and mitigation strategy against network-level adversaries. In the extreme scenario where the adversary breaks the weak authentication, and spoofs the identity during first connect, it has to generate a different self-certifying key from the key generated by the device. Hence, the provider obtains two conflicting keys for the same identity and revokes access accordingly. 

\vspace{1mm}
\noindent{\em Key Revocation:} To provide better security with respect to the key itself, we ensure that the reputation of a user decays with time. A consequence of this is that participants of the protocol need to regularly participate in key-exchange to ensure liveness of the identity. On decay beneath a specific threshold, or on repeated blockage of interactions within an epoch, the previously generated (and used) self-certifying keys are revoked. A broadcast is sent to all associated users notifying them of this event. Thus, these ephemeral keys provide both forward and backward secrecy, as in the worst-case, a compromised key will provide no information about keys used prior, or to be used. 

\vspace{1mm}
\noindent{\em DDoS Alleviation:} SMI messages coupled with existing text message traffic can increase the network load on the cellular network. Enck et al. \cite{enck2005exploiting} suggest that to disturb cellular service, efficiently blanketing only a specific area with messages is sufficient so as to increase the probability of successful disturbance. Similar to the design of backoff protocols in wireless networks, SMI can use increasing delays in SMS messages and message losses as early signals to reduce the rate of messages from individual devices to reduce the network load. One additional strategy discussed earlier is to distribute the messages across the SMS and alternate channels to further reduce cellular network load.

%\vspace{2mm}
%\noindent{\em Global Network Adversary:} When faced with a computationally and economically unbounded adversary who can intercept a large fraction of cellular communications, key-exchanges can be severely hampered especially if the adversary can intercept all weak SIM authentication requests. The SMI protocol offers limited security guarantees in the face of such an all-powerful adversary. In the event where a global network adversary possesses limited access to intercepting communications within one cellular network, SMI users may be able to leverage device mobility across geographic locations to potentially discover the presence of conflicting key pairs for an identity in the event of a network level MitM attack from a global network adversary.



==> Eurosys'16/NSDI/abstract.tex <==
\begin{abstract} 

The {\em unique identities} of every mobile user (phone number, IMSI) and device (IMEI) are far from secure and are increasingly vulnerable to a variety of network-level threats. The exceedingly high reliance on the {\em weak SIM authentication} layer does not present any notion of end-to-end security for mobile users. We propose the design and implementation of Secure Mobile Identities (SMI), a repetitive key-exchange protocol that uses this weak SIM authentication as a foundation to enable mobile users to establish stronger identity authenticity. 
%The SMI protocol is a spatio-temporal, multi-path, repetitive challenge-response mechanism, enabling two mobile entities to tag every key exchange with a (location, time) pair. It leverages the diversity in this pair to build a reputation for every user-generated key. 
The security guarantees of SMI are directly reliant on the mobility of users and are further enhanced by external trusted entities providing trusted location signatures (e.g. trusted GPS, NFC synchronization points). In this paper, we demonstrate the efficacy of our protocol using an implementation and analysis across standard mobility models. We also demonstrate how the SMI abstraction can enable new forms of secure mobile applications, including messaging, multimedia transfer and a marketplace.

\end{abstract}


==> Eurosys'16/NSDI/dump/6-Security.tex <==
\section{Security Analysis}
\label{security}

In this section, we address the attacks and challenges discussed in \S \ref{probsettings}, specifically:



%\subsection{Addressing Threats}
%\begin{itemize}
\itemsep-0.23em 
{\bf Malicious Adversaries:} As discussed earlier, adversaries can create a fBTS. Once the honest device connects to it, the adversary negotiates to the lowest level of encryption supported by the device and relays inbound and outbound calls, as well as IP traffic sent on the data channel. In theory, these adversaries can be detected by the other BTS of the network provider, but there is no documented responses against such temporary rogue towers. This attack is heavily dependent on the probability $P$ of a user being in the vicinity of the fBTS. However, this attack is alleviated by moving outside the transmission zone of the fBTS. The probability that the user moves to $k$ locations and is in the vicinity of the fBTS in all of them is $P^k$, which is very small. Hence the probability of failure of the attack, or probability of protocol success is $1-P^k$. By ensuring mobility, the success of this attack decreases exponentially. If communication is carried out across multiple channels, the probability of protocol success across multiple channels is $\prod_{i=1}^{3} (1 - P^{k_i})$ ; $\sum_{i=1}^3 k_i \leq k$. This is a measure in the worst-case scenario as the event in which more than a single channel is compromised is very rare. Setting the predefined threshold large enough provides a degree of flexibility towards partially diligent users.  

{\bf Signal Jamming:} Another variant of the attack is where such an adversary jams communication of the device connected to the fBTS and attempts to join interactions in its place. However, the exchange of random parameters $a,b$ at the beginning of every epoch ensure that subsequent interactions in the epoch are consistent (as explained in \S4). On detecting an inconsistent interaction, a diligent participant aborts the protocol and restarts it at a different location. 

If an attacker spoofs the identity of a victim \textit{and} remains part of a consistent interaction by obtaining values $a,b$ at the beginning of an epoch, another improbable event, the other user will receive messages from two \textit{distinct} identities (as part of the PKI) once the victim is no longer in the vicinity of the fBTS. We wish to reiterate that as long as the users are mobile and diligent, these attacks fail. In the absence of mobility, there is a significant increase in probability of successful jamming and other failure events.



{\bf DoS:} As discussed in \S \ref{attacks}, adversarial DoS attacks are mitigated by moving out the range of the fBTS. Our honest MNO assumption invalidates any operator-based MitM and DoS attacks. Solutions such as MAC level disambigution of the message channel \cite{ghaderi2012connection} and content-based vertical handoff ensure that the cellular network is not overprovisioned due to scaling.

{\bf Low-Entropy Hash:} Modern smartphone processors run at clockspeeds upto 2 GHz, giving them fairly strong computational ability. By selecting an appropriately large key-length, we can ensure that the probability of a collision is significantly reduced. 

{\bf Key-pair generation:} The increasing processing capabilities of modern smartphones and the various entropy sources such as cameras and accelerometers \cite{voris2011accelerometers, marghescu2014cryptographic, yuzuguzel2015shakeme} available to it ensure that key-pairs can be frequently generated without substantial strain. The generated key-pair is stored safely as we assume that the user does not disclose any sensitive information.

%\end{itemize}


==> Eurosys'16/NSDI/dump/7-Additional.tex <==
\section{Discussion}
\label{discussion}

We now discuss the rationale behind our design.
\vspace{-2mm}
\subsection{Trusted Location Distrbution}
\label{tld}

309 retailers have an estimated 7623 stores in New York City \cite{survey}. With a size of 304.6 sq. miles, the average store density is 25 stores/sq. mile. The zip code 10003 (Greenwich Village) of size 0.58 sq. miles has 164 retail stores, resulting in value of 282 stores/sq.mile in this area. This is 11 times the city-wide average and is attributed to the high population density of Manhattan and it being a popular tourist destination. The recent proliferation of NFC based payment has resulted in a large number of stores adapting contact-less payment solutions. Based on analysis, close to 80\% of the chosen stores in New York have use such solutions and are hence are location verified \cite{mastercard}. 
%That is to say, 8 in 10 stores one would visit is a trusted location.

\vspace{-2mm}
\subsection{Smartphone Proliferation}
\label{proliferation}

Based on a Pew survey, 64 \% of all US adults now have smartphones. However, among the population of mobile phone owners (91 \% of US adults), the smartphone penetration number is now 61 \%. Apple iPhone sales alone exceeded 40 million in the US for the 2014 financial year. 19\% of Americans rely to some degree on a smartphone for accessing online services and information-either because they lack broadband at home, or because they have few options for online access other than their cell phone.
\vspace{-2mm}
\subsection{Economic Implications}
\label{economics}

Another Pew survey suggests cell owners between the ages of 18 and 24 exchange an average of 109.5 messages on a normal day which works out to more than 3,200 texts per month. The typical or median cell owner in this age group sends or receives 50 messages per day (or 1500 messages per month). However, over 100 service providers in the United States provide unlimited messaging as part of their monthly plans \cite{whistleout}. This greatly alleviates the cost associated with the large number of messages exchanged between users of SMI.
\vspace{-2mm}
\subsection{Human Mobility}
\label{mobility}

The average moderately active person take aound 7500 steps per day. Doing the math; the average person with the average stride walks 3.76 miles a day. To support this claim, New York was voted the most active state in the US, according to a recent study from Fitbit, where a resident takes an average of 10000 steps per day.
%\subsection{QoS In Cellular Networks}
%
%A variety of factors affect the time taken to successfully deliver a message. Delays are caused due to:
%\vspace{-2mm}
%\begin{itemize}[leftmargin=-.01in]
%\itemsep-0.23em
%\item Low quality cellular devices.
%\item Delay in allocation of adequate network infrastructure.
%\item Lack of fairness from service providers.
%\item Limited coverage and network capacity.
%\item Poor government monitoring on standards.
%\item Environmental materials and current location i.e. distance from the cellular towers.
%\end{itemize}
%\vspace{-2mm} 
%Any combination of the afforementioned reasons could result in a deviation from optimal delivery time of the messages required for the SMI protocol. For example, the difference in message delivery time between AT$\&$T in New York City and Etisalat at Abu Dhabi may arise due differences in city demographics, geographics and infrastructure. This could cause advancements or delays towards the time required to build sufficient reputation. 










==> Eurosys'16/Old Draft/Acknowledgements.tex <==
\section{Acknowledgments}
This material is based on the work partially supported by
 funding from the Center of 
Technology and Economic Development (CTED), NYU Abu Dhabi. We thank CTED and NYUAD for their support.

==> Eurosys'16/Old Draft/Applications.tex <==
\section{Applications}

There can be various applications that can be built on top of Secure Mobile
Identities protocol. DSMI promises security and reliability along with usability.
DSMI does not involve any user involvement and the simplicity of DSMI makes
it favorable to be adapted in existing as well as new applications.
We present here some of the ideas of the applications which we think can be built
on top of DSMI protocol seamlessly. 

\subsection{Secure Messaging Application}
We have implemented secure SMS for Android. Secure information; text or pictures or
documents; can be encrypted using shared public key using DSMI and the information
exchanged is authenticated by DSMI as well. Popular applications like Whatsapp\cite{whatsapp}, 
Viber\cite{viber}, 
and BBM\cite{bbm} etc can be extended to include another security layer(DSMI) without changing
their signature interface.

Photo sharing is popular these days (snapchat~\cite{snapchat}, instagram~\cite{instagram}), 
the users needs privacy for the pictures pictures they
share. Building an application that sends private pictures to a closed set of audience with
no intrusion is possible using DSMI.


\subsection{Secure Cash}
We can leverage DSMI to build an app that requires the most security. We can build a virtual
cash system on top of DSMI which can be used as the security layer. The bank is a trusted 
party whose secure cash app would allow its customers to perform secure digital transactions.
The secure cash is the implementation of the process of sending and receiving a bank transaction 
through an app, removing the requirements of a cash register. 
Electronic transactions can be done with or without the presence of a designated point of sale.
Alice wants to buy a dress, from a store which is registered with her bank and has a trusted 
location device, using her secure cash app. She opens the application and scans/takes a picture 
of the bar-code of the dress and sends it to her bank using the pre-installed trusted location device 
in the shop. Alice's phone performs the three-way handshake using the trusted location device at the
shop with the bank. The bank authenticates the location and evaluates the trust level of Alice and 
sends a receipt to the shop indicating that the transaction has been taken place.

Another important scenario using secure cash can be the cash receipt system and it can be useful in places
where banks/ATM/credit card transactions are not widely accessible. Alice who wants to transfer money to
Bob's account; uses the secure cash application to do so; signs a cheque and sends it to Bob after 
completing a secure key exchange handshake. Bob on receiving the cheque goes to the bank where it gets
scanned and receives the money.

\subsection{Safe and Secure Virtual Identity}
Documents like passport, SSN, driver's license, property documents etc are very sensitive and need to be
kept at a safe location at all times. Applications can be built on top of DSMI that can encrypt these files
and send them to the trusted intended party or user without physically sending the documents. Using DSMI 
would help the sending and the receiving party be sure that the document is actually received from the
actual owner and is received by the intended user.

\begin{comment}
\subsection{Secure SMS}

We have implemented secure SMS for Android as discussed in the Implementation section.
The two users exchange their keys using one of the paths: SMS, bluetooth or IP.
Alice and Bob wants to share some secret information with one another so they decided
to use the DSMI text message app. Alice enters the contact number of Bob and the app
performs the 3-way key exchange handshake in the background after Alice choose one of
the three methods she wants the key exchange to take place through. Then she types the
top secret information in plain text and hit send. The app encrypts the message in plain
text and sends it to Bob. The DSMI application decrypts the message and shows the message
to Bob in plain text. This can be done for instant messaging applications
as well. Existing applications for example WhatsApp \cite{whatsapp},
Viber \cite{viber} and Line \cite{line} can make use of DSMI to perform the same functionality and their signature
interface but they can add additional security without having to change their popular
application.

\subsection{Secure Photo exchange}

Sharing pictures online is the new trend. Every user who has a phone with a camera not
only takes a picture of every single moment of his/her life, they want to share these pictures within
their social circle. As photo sharing became popular, it became apparent that the user
needs privacy for those personal pictures as well. One such popular application: Snapchat \cite{snapchat} enables
its users to share their picture with their friends for a set amount of time and then the picture
is removed. While this allows a certain degree of security this isn't completely devoid of any kind
of intruder attacks. Instagram \cite{instagram} is also one of the leading photo sharing application these days. Both 
these applications can use DSMI protocol to make their system reliable and secure. Similarly, one can develop
an application that can encrypt the photos only the user wants them to encrypt-doing so we can reduce the overhead of
an application for encryption and decryption.

\subsection{Secure cash}

We can leverage DSMI to build an app that requires the most security. We can create 
a cash receipt system using DSMI. The system would require a bank account that would 
allow transactions. We can create an application for a user to sign the bank approvals
and authorize another user to cash those approvals. The application can make use of
DSMI as a security layer. The security layer is a much needed feature in this application.
Nobody wants an intruder to eavesdrop in transactions as critical and sensitive as this.
After completing a secure key exchange handshake, Alice who wants to authorize Bob
to get cash from a bank; digitally allows Bob to do so by signing a cheque using secure
cash. The bank is a trusted party whose secure cash app would allow its customers to perform
secure digitally transactions.

\subsection{Secure File exchange}

In the present era of technology, it seems redundant to have a physical copy of
all the important and sensitive documents. One needs to securely place them and in hour
of need take those documents out of the secure area and send them securely to the
trusted intended recipient. Documents like a user's passport, social security number,
property documents etc. Applications can be built on DSMI and can encrypt the files
and send them to the trusted intended party or user. Using DSMI would help the sending 
and the receiving party be sure that the document is actually received from the
actual owner and is received by the intended user.
\end{comment}

==> Eurosys'16/Old Draft/Conclusion.tex <==
\section{Conclusion}

People share information all the time using their cell phones. Phone carriers claim
that their system is protected and all the data sent and received by a user is
encrypted. However, this is not the case. A lot of times users fall a victim of
various attacks such as snooping, eavesdropping, jamming, stealing the identity etc.
To fill in this gap of security we designed Secure Mobile Identities, a protocol that
uses various locations and multiple paths to develop a notion of trust. The
user uses DSMI repeatedly through various locations and through different paths to
earn trust score. The trust score is directly proportional to the user's authentication.

We have implemented and evaluated DSMI on an android platform. It is an easy-to-use app
and is similar to that of a native SMS android app to enhance usability of DSMI.
DSMI can be extended to share pictures, documents and it can be used for bank transactions
as well. Using DSMI can help users communicate securely and with a confidence that no
other person in the middle and they are communicating to the person they intend to communicate with.


==> Eurosys'16/Old Draft/Evaluation.tex <==
\section{Evaluation}

To evaluate the usability of Secure Mobile Identities usability
we conducted trial runs and tests to gather stats. In this section
we will explain the procedure and the results and observations on
the basis of the tests conducted.

\subsection{Procedure}
We wanted to test how long it takes for a user to complete the key
exchange handshake as it involves exchanging multiple text messaging.
The results depends on the network used for sure. Our tests were
conducted in Abu Dhabi, UAE using Etisalat \cite{etisalat} as our 
telecommunications services provider. 
We used java's function for time calculation to get time in nanoseconds.
We recorded the current time in nanoseconds. We used two ways to get the time: the phone
is linked with a PC via bluetooth and both phones signals the PC to record the
time (to get time of one machine) and for more accuracy we used the phones
to record their times themselves (to account for any delays caused while
transmitting the messages via bluetooth).
Time 1a is the time required to start the transaction by phone A and when phone
B replies back with its own data. Time 1b is the time recorded from the moment
phone B sends back its own data until it receives the challenge reply by A.
Both these times: Time 1a and Time 2a are taken by the PC connected via
bluetooth to both phones.
Time 1b and 2b is the same time as Time 1a and 2a, the difference is the
way the time is recorded. 1b and 2b are recorded on phone A and phone B
themselves.
Time a is the time required by phone A to send data to phone B. It is calculated
by getting the time in nanoseconds when user using phone A clicks send; phone
A sends an alert to PC to record the current time via bluetooth. Phone B when
receives the message sends an alert to PC to record the current time.
\\Time b is the time recorded when phone B sends its own data to A and the time
A receives it. Time c is the time required when A sends the challenge reply to
phone B and B receives it.

\subsection{Observations and Results}

We used a PC for recording the time when the phone sends a signal using bluetooth. 
We also used phones themselves to record the time. Using another device, in our case
the PC, for recording time can cause delays and by using two different devices for
recording time can create the difference in time. Figure \ref{timeDif} shows the difference
in times. Time 1 is the time taken by phone A to send meta-data to phone B 
and phone B replies back with encrypted challenge reply and its own metadata to phone A.
Time 2 is the time taken by phone B to send the encrypted challenge reply and its 
own metadata to phone A and phone A replies with the challenge reply. This figure shows that
the difference between the two is not very significant and we can use the average number to 
add into the results for an approximate time calculation.


\begin{figure}[htb]
    \centering
		\subfigure[{\smallTime difference for time 1: time taken by phone A to send meta-data to phone B and gets back a response}]
		{
				\includegraphics[width=0.45\columnwidth]
				{C:/Users/fa45/Dropbox/secmobid/tex/analysis/DiffTime1.jpg}
    }
		\subfigure[{\small Time difference for time 2: time taken by phone B to send the encrypted challenge reply and its 
own metadata to phone A and gets back a response}]
		{
				\includegraphics[width=0.45\columnwidth]
				{C:/Users/fa45/Dropbox/secmobid/tex/analysis/DiffTime2.jpg}
        
		}
		\caption{The time difference recorded}
		\label{timeDif}
\end{figure}


\\We measure the total amount of time needed to complete the 3-way key exchange
handshake by all paths.
ToDo: include data and bluetooth as well
\\Figure \ref{ttime} shows the timing analysis. According to this figure, for the
SMS the maximum time taken in all the tests was approximately 120seconds and the
minimum time taken was approximately 70seconds. The average is approximately 95seconds.
This means on average a user has to wait for up to 95seconds to start the exchanging
the messages with the intended user.

\begin{figure}[htb]
    \center{\includegraphics[width=2in]
        {C:/Users/fa45/Dropbox/secmobid/tex/analysis/totalTimeTaken.jpg}}
    \caption{\label{ttime} Total time taken for 3-way key exchange}
\end{figure}

\\Figure \ref{timeabc} shows which part of the 3-way protocol takes the most time.
Time a is the time required by phone A to send data to phone B. Time b is the time recorded when phone B sends its own data to A and the time
A receives it. Time c is the time required when A sends the challenge reply to
phone B and B receives it. The figure clearly shows that time C requires the least
amount of time whereas time a requires the most.


\begin{figure}[htb]
    \center{\includegraphics[width=2in]
        {C:/Users/fa45/Dropbox/secmobid/tex/analysis/TIMEabc.jpg}}
    \caption{\label{timeabc} Time a, Time b and Time c}
\end{figure}















==> Eurosys'16/Old Draft/SMI.tex <==
\section{DSMI protocol overview}

The main idea of Secure Mobile Identities is to enable users to exchange keys for
a secure one-to-one session. We want to implement a highly secure protocol
over highly insecure channels. DSMI uses various paths for building trust amongst 
the users. The application uses the cell towers and the GPS coordinates to 
gather the location data. It also uses various forms of trusted location services.
DSMI is a repetitive, spatiotemporal protocol that uses time, location and paths to
develop digital trust. 

\subsection{Overall design} 

Secure Mobile Identities uses the solo SMS path/single path, the IP-SMS path 
and the Bluetooth-SMS path. So there are 3 ways in which
a user can communicate: via SMS, via Bluetooth and via IP.
All these paths receive the verification of the
key exchange handshake via SMS. Hence it is our assumption that the SMS will 
always be delivered to the user. The single path relies only on the SMS. 

\\The user opens the application and enter the number of the intended user. This is all
what a user has to do in order to initiate the key-exchange process. 
Secure Mobile Identities uses a 3-way key exchange handshake, like most of the 
network security protocols. In single path all these 3 messages are transmitted via
SMS. In multi-path; the data is exchanged using IP or Bluetooth but the verification
which is the challenge reply is always done via SMS. We have modified the 3-way handshake
for the multi-path.

\\For a 3-way handshake,(1) user A sends A's public key, A's location, time, A's phone number
and a challenge to the user B. User B on receiving this message sends back (2) B's public
key, B's location, time, B's phone number, challenge and the reply to A's challenge.
User A verifies the challenge reply sent by the user B and if correct sends (3) the final
challenge reply to B. 

\\For a muti-path modified 3-way handshake,(1) user A sends A's public key, A's location, time, A's phone number
and a challenge to the user B via Bluetooth or IP channel. User B on receiving this message
sends back (2) B's public key, B's location, time, B's phone number and B's challenge to A via 
Bluetooth or IP channel "and" User B then sends  the reply to A's challenge via SMS path.
User A verifies the challenge reply sent by the user B and if correct sends (3) the final
challenge reply to B via SMS. 


\\DSMI maintains a table of the digital trust; as mentioned in section \ref{score}; using the 
user's location data, the time of exchanging keys and the path used. Location
plays a very vital role in DSMI. Location of the user is captured by a number of
ways which includes using cell towers and the GPS coordinates. For more reliable 
and trust worthy location data, DSMI uses various forms of getting trusted and
certifying location along with a time stamp. The location data gathered via
trusted location provider is considered the most authentic and trustworthy location
data. 

\\Each user performs the key exchange multiple times and each time the location and time of
user is recorded along with the path used to exchange the keys. Doing so, DSMI determines the
pattern the user is using for the interaction. 
Once the 3-way handshake is completed, the
score is increased on the basis if the location information obtained. If the location data 
obtained is from a trusted/authentic location provider such as trusted location provider; as discussed in section 
\ref{location} and \ref{score}; the score is increased more. As DSMI is the repetitive key exchange protocol; the user
exchanges keys multiple times along with the location and time. This information is stored and
on the basis of this information; the score is calculated. The score is maintained by DSMI to develop different
levels of trust. If an attacker has hacked the user's information, it is a very less probability
that the attacker is at the same location as the user. The user builds more trust i.e. more score
by following some kind of a pattern. Therefore, if the same set of keys are exchanged
from a location that does not follow the pattern; the level of trust and hence the score is
decreased. DSMI has established a certain threshold which when is achieved by the user; the keys
are assumed to be genuine. The score is calculated on the basis of the location pattern, it is
also set on the basis of different paths used by the user. A user sharing the same set of keys
from a set pattern of location across different paths of DSMI is also a variable that is set for calculating
the trust score. The variety of paths used and the set pattern followed by the user helps achieving
a high trust score.


\subsection{Spatiotemporal single and multi paths}

The single path in DSMI relies only on the SMS. It is a one-way probabilistically trusted
path. The assumption is that the user's phone is connected to the network which is
trusted. If the network that the phone is connected to is trusted then we can also assume
that there are no main-in-the-middle attacks in that path and our final assumption is that
there is no loss in the SMS i.e. SMS will always be delivered to the intended user. In a 
nutshell it can be said that SMS is the most secure, one-way, trusted path. By saying so
we believe that SMS once sent-will be delivered but we are not making any assumptions
that the user who is sending the SMS is the intended user; the user who's sending the
SMS can be an attacker.
DSMI uses multiple channels to exchange keys in a secure manner. Having multiple
channels for authentication allows the DSMI protocol to have added security. The assumption is that the attacker can compromise one channel
only-the probability to compromise both paths is extremely low. DSMI uses two such paths:
IP-SMS channel and Bluetooth-SMS channel. SMS channel in both cases is used for verification
or for the challenge reply in the key exchange handshake as discussed in section \ref{location}
. It should also
be noted that it is assumed that the verification SMS will always reach the intended user.
Users using different channels across different times and locations increase the trust level.


\subsection{Trusted or untrusted location}\label{location}

In DSMI, location plays a pivot role. Location data is gathered in a number of ways. Location data
is the key variable in evaluating reputation score. The user can have trusted location and the
user can have untrusted location. Users performing the key exchange using trusted location scores
more than the users performing the key exchange using untrusted location. A trusted location is
a certifying location signed by a trusted 3rd party. We describe the different ways of gathering data
as follows: 

\begin{itemize}

\item {\em GPS coordinates and cell towers}. The most
common way is through cellular tower and GPS coordinates. This is an unreliable and untrustworthy 
way to acquire the location information as any attacker can modify the GPS coordinates easily. Cell
towers maintains the location and this location information can be easily fetched.  

\item {\em Trusted 3rd party service} As the location gathered by GPS coordinates and cell towers
is not secure as it can easily be modified; we propose a secure, certifying location service. A 3rd
party service such as Google wallet \cite{googlewallet} can be used to fetch a signed location 
contract along with the timestamp. This service is not limited to Google wallet; a 3rd party can
deploy their own location tracking system which can enable a user to quickly sync the phone via
bluetooth to get the certifying and signed location. The location, timestamp can be used by any user
using a global public key. 

\item {\em Trusted IP} Another way of gathering location information is through the user's IP address.
IP address of every device is unique and it is theoretically possible, to determine the 
physical location of IP addresses. This is called Geolocation. Geolocation systems attempt to map IP 
addresses to geographic locations using large computer databases. As it is possible that the attacker
can hide behind a proxy, thus we need a trusted 3rd party wifi hotspot which works in essentially the
same way as described above but instead of using coordinates gives away a certifying IP address.

\end{itemize}

\\DSMI requires the users to perform this key exchange handshake a number of times for score
generation as discussed below. Performing this exchange across different locations at different
time would help increase the level of trust for that user.
 
\subsection{Repetitive key exchange and Reputation score}\label{score}

DSMI maintains a table of user information data including user's phone number,
user's public key, all the various locations the user performed the handshake and
the date and time of the handshake. DSMI requires the users to 
perform this key exchange handshake a number of times for score
generation. On the basis of this table; DSMI evaluates the digital
trust score against each user. Retaining these scores creates various levels of trust.
Each time a user use the same key from different or same location across various timings
and via a variety of paths used, the score of the user is increased. Getting a variety of
location information helps DSMI determine a pattern. If the location information deviates from
the set pattern, the score is affected accordingle. Some factors like
trusted location add more score than the usual, insecure location gathering techniques.
The score is deducted if the data gathered and stored in the table shows anomaly. If
a user's score reach a certain threshold, the key of that user is considered genuine. 
To reach that level of trust requires repetitive key exchange across different locations,
time and path.



==> Eurosys'16/Old Draft/SMI_with_trusted_location.tex <==
\section{DSMI with trusted location}

In this section we will discuss the DSMI protocol in detail using trusted location data gathered
through 3rd party services. We first explain the details of trusted location data.

\subsection{Trusted location based key exchange}

The location data gathered through GPS and cell tower is not trusted as explained the above section.
We need a secure and trusted location gathering mechanism. By a trusted location we mean a location that
can not be changed by an attacker and is signed by a trusted 3rd party. The location data gathered through
these trusted points of location gathering devices is considered the most authentic and a user having a trusted
location gains more score points. There can be a number of ways to achieve this. We present a few of those
techniques in this paper.

\\A trusted 3rd party installs some of these certifying location gathering devices in a few places for a user to sync
their device and gets a certifying location along with a time stamp. The location data is actually the location
of that device and as the user is in close proximity of that device; the location of the user is the same as that
of the device. Syncing can be done via bluetooth or any other technology. This is something very trivial to do
as Google already has deployed its Google wallet points at various location. A user can sync up with the
Google wallet point and get a certifying location.

\\Another way of gathering location data is through IP. As the public IP address of every device is unique and IP
addresses are assigned in the form of a tier system based on the geographical location. It is possible to gather
the location information through IP. Mapping IP addresses to a geographical location is known as Geolocation and is
described in \cite{taylor2012bringing}  and \cite{kovacs2002geolocation}. The idea is to have a trusted 3rd party
hotspot deployed at various location so that a user can sync the mobile to get a certifying IP location. The IP
location can further be processed as discussed above to break it down to geographical location. 


\subsubsection{Trusted location data}

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1,c1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2,c2)S_2,c1 \\
 \textbf{3}.& \quad U_1 \rightarrow U_2: & & (c2)S_1 \\
\end{align*}

In this protocol, the location data ($L_1,L_2,t)$ is from a trusted
source. The GPS chip within the mobile devices $W_1,W_2$ are trusted
and the cell tower information obtained is also trusted. Hence the
protocol boils down to the three-way handshake protocol. 


\subsubsection{Trusted point of sale device}

\subsubsection*{Assumptions}
\begin{itemize}
\item Point of sale devices are trusted. 
\item Point of sale devices have the ability to sign a message and
  transmit the message securely to the device $W_1$ of the user $U_1$.
\end{itemize}

\subsubsection*{Protocol}

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow G: & & P_1,L_1,t,U_1,D_1  \\
 \textbf{2}.& \quad G \rightarrow U_1: & & G_P, (P_1,L_1,t,U_1,D_1)G_S \\
 \textbf{3}.& \quad U_1 \rightarrow C: & & P_1, (G_P,(P_1,L_1,t,U_1,D_1)G_S)S_1 \\
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] $U_1$ sends the message $P_1,L_1,t,U_1,D_1$ to a
  point of sale device $G$. 

\item[\textbf{2.}] A point of sale device can be a NFC
  device or other device which is capable to signing a message. The
  point of sale device $G$ signs the message $(P_1,L_1,t,U_1,D_1)G_S$
  and along with $G_P$ (public key) sends it back to $U_1$.

\item[\textbf{3.}] Now $U_1$ signs the message it received from $G$,

  ($P_1$,$L_1$,$t$,$U_1$,$D_1$)$G_S$)$S_1$ and sends it to the central
  authority $C$ along with $P_1$. Since $G$ is trusted (has trusted
  credentials), $C$ is certain that the message is signed by $G$ and
  that $U_1$ was indeed present at the point of sale location. The
  point of sale device could also have a fingerprint reader (or any
  biometric device) to authenticate user's identity and the biometric
  data can also be part of the signed message from $G$ to $U_1$. 
\end{enumerate}



\subsection{SINGLE PATH SPATIO-TEMPORAL REPETITIVE KEY EXCHANGE}

It is the same as the described in the previous section except for the
addition of trusted location. We will now describe the same protocol
with added security.

\subsection*{Preliminaries}
\begin{itemize}
\item  Every mobile device is allocated a unique identity $D_1$
(either a phone number or IMSI number)
\item User $U_1$ registers with provider a $X_1$ using a device $W_1$
  with a unique identity $D_1$ 
\item If $W_1$ is directly connected to an authorized base station of
  provider $X_1$, then anyone who sends a message to identity $D_1$ is
  routed to $W_1$ and is received by user $U_1$.
\item The 3rd party location gathering device $W_2$ is trusted and the location
	data $D_2$ is genuine. 
%\item The routing layer within the cellular network is trusted
\end{itemize}


The step by step protocol is described as follows.

\begin{align*}

	\textbf{1}.& \quad W_2 \rightarrow U_1: & & (L_1)S_G  \\
	\textbf{2}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1,c1)S_1  \\
	\textbf{3}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2,c2)S_2,c1 \\
	\textbf{4}.& \quad U_1 \rightarrow U_2: & & (c2)S_1 \\
	\textbf{5}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
								times} \\
 \textbf{6}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}

\begin{enumerate}

\item[\textbf{1.}] User $U_1$ syncs with a trusted location device $W_2$ which gives
	$U_1$ a certifying location $L_1$. $W_2$ sends the signed message $(L_1)S_G$ to $U_1$.

\item[\textbf{2.}] User $U_1$ generates a self certifying key $P_1$ and
  signs the message consisting of location data $L_1$, time $t$,
  username $U_1$, user identity $D_1$ and challenge nonce $c1$. Here
  $L_1$ is location data obtained using 3rd party in step 1. $U_1$ sends the signed
  message $(L_1,t,U_1,D_1,c1)S_1$ and $P_1$ to $U_2$.

\item[\textbf{3.}] User $U_2$ generates a self certifying key $P_2$ and
  decrypts the message using the key $P_1$ sent in the message. $U_2$
  then signs the message consisting his location data $L_2$, time $t$,
  username $U_2$, user identity $D_2$ and reverse challenge nonce $c2$. User
  $U_2$ sends key $P_2$, challenge nonce $c1$ and signed message
  $(L_2,t,U_2,D_2,c2)S_2$ to $U_1$.

\item[\textbf{4.}] User $U_1$ decrypts message and sends the signed
  reverse challenge nonce $c2$ back to $U_2$. This completes the
  three-way handshake protocol.

\item[\textbf{5.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. We have to repeat the protocol $n$ times because
  the location information is untrusted. The rationale here is, an
  attacker might try to spoof the identity of $U_2$ once or twice, but
  repeatedly ($n$ times) masquerading the identity of $U_2$ is
  hard. So by repeating the protocol $n$ times, preferably from
  different locations, increases the chances of the user being $U_2$. 

\item[\textbf{6.}] If after $n$ times $(D_2, P_2)$ corresponds to
  $(L_1,L_2,t)$ then with high probability $U_1$ has established a
  secure connection with $U_2$.
\end{enumerate}



\subsection{Multi-Path spatio-temporal repetitive key exchange}

In the previous section we looked at single path key exchange protocol, where
just one channel (SMS) was used to exchange keys between two users with trusted location.
In this section we discuss the multi-path key exchange protocol, where
multiple communication channels are used to exchange keys in a secure
manner using trusted location data. 

\subsubsection{IP and SMS}
The key exchange handshake is the same as described in the previous section, we present here
the key exchange handshake with trusted location data.

\begin{align*}
 \textbf{1}.& \quad W_2 \rightarrow U_1: & & (L_1)S_G  \\
 \textbf{2}.& \quad U_1 \rightarrow IP: & & P_1,t_1,IP_1  \\
           .& \quad U_2 \rightarrow IP: & & P_2,t_2,IP_2  \\
 \textbf{3}.& \quad U_1 \rightarrow U_2: & & (L_1,t,U_1,D_1,c1)S_2 \\
 \textbf{4}.& \quad U_2 \rightarrow U_1: & & (L_2,t,U_2,D_2,c2,c1)S_1,\\
 \textbf{5}.& \quad U_1 \rightarrow U_2: & & (c1,c2)S_1 \\
 \textbf{6}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
 times} \\
 \textbf{7}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] User $U_1$ syncs with a trusted location device $W_2$ which gives
	$U_1$ a certifying location $L_1$. $W_2$ sends the signed message $(L_1)S_G$ to $U_1$.

\item[\textbf{2.}] $U_1$ and $U_2$ exposure their public keys $P_1$
  and $P_2$ respectively though an IP channel. The keys get deleted
  after a certain time period ($t_1$ and $t_2$). $IP_1$ and $IP_2$ are
  IP addresses where $P_1$ and $P_2$ were stored respectively. 

\item[\textbf{3.}] $U_1$ signs the message $(L_1,t,U_1,D_1,c1)$ where
  the message consists of 
  location data $L_1$, time $t$, username $U_1$, user identity $D_1$
  and challenge nonce $c1$. with 
  the public key $S_2$ and sends it to $U_2$ using SMS. $L_1$ is the
  location data obtained in step 1.

\item[\textbf{4.}] $U_2$ decrypts the message and gets the challenge
  nonce $c_1$. $U_2$ signs the message $(L_2,t,U_2,D_2,c2,c1)$ and
  sends it back to $U_1$ using SMS. $L_2$ is the location data of the
  $U_2$ which might be one of, or a combination of i) Trusted location, 
	ii) cell tower information, and iii) GPS information, as
  mentioned on the previous step. 

\item[\textbf{5.}] $U_2$ sends the signed nonces $c1$ and $c2$ to
  $U_2$. This completes the three-way handshake protocol. 


\item[\textbf{6.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. We have to repeat the protocol $n$ times because
  the location information is untrusted. $U_2$ also follows the same
  approach and verifies whether $(D_1, P_1)$ corresponds to
  $(L_1,L_2)$. 

\item[\textbf{7.}] By repeating the protocol $n$ times, the reputation
  score (as described in the previous section) either increases or
  decreases. Once the reputation score crosses a certain threshold,
   then with high probability $U_1$ has established a
  secure connection with $U_2$.

\end{enumerate}


\subsubsection{Bluetooth and SMS}

Following is the detailed version of the Bluetooth protocol using trusted location:

\begin{align*}
 \textbf{1}.& \quad W_2 \rightarrow U_1: & & (L_1)S_G  \\
 \textbf{2}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1)S_1  \\
 \textbf{3}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2)S_2 \\
 \textbf{4}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
            times} \\
 \textbf{5}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}


\begin{enumerate}
\item[\textbf{1.}] User $U_1$ syncs with a trusted location device $W_2$ which gives
	$U_1$ a certifying location $L_1$. $W_2$ sends the signed message $(L_1)S_G$ to $U_1$.
	
\item[\textbf{2.}] $U_1$ sends the location information $L_1$ obtained above, time
  $t$, username $U_1$, user identity $D_1$ to $U_2$ using Bluetooth. 

\item[\textbf{3.}] $U_2$ sends the location information $L_2$, time
  $t$, username $U_2$, user identity $D_2$ to $U_1$ using Bluetooth. 

\item[\textbf{4.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. 

\item[\textbf{5.}] If after $n$ times $(D_2, P_2)$ corresponds to
  $(L_1,L_2,t)$ then with high probability $U_1$ has established a
  secure connection with $U_2$.

\end{enumerate}

==> Eurosys'16/Old Draft/SMI_with_untrusted_location.tex <==
\section{DSMI with untrusted location}

In this section we will discuss the DSMI protocol in detail using untrusted location data gathered
through GPS and cell tower.

\subsection{SINGLE PATH SPATIO-TEMPORAL REPETITIVE KEY EXCHANGE}\label{singlepath}

In this protocol, only SMS is used to exchange keys between the
users. It is a one-way probabilistically trusted
path under the assumption that the SMS that is sent to a user is
always delivered to that user and that the network is trusted such that
there are no man-in-the-middle attacks possible.
The location information is not trusted, hence the protocol has
a repetitive procedure. Initially keys are exchanged using a simple
3-way handshake protocol where each user generates a self certifying
key. Once the initial 3-way protocol is completed, a reputation score
is maintained by each user. This score is increased based on the
location information obtained from the cell 
towers and the GPS. The assumption here is
the attacker will not follow the user at all times. So if the
adversary was impersonating the user a few times, his location will be
very different from the actual user's location. As the keys are
repetitively exchanged at different intervals of time the location
information is updated. As the user location behavior follows a
specific pattern repeatedly, the reputation score is increased. Same
set of keys are exchanged at different intervals and from different 
locations, where the locations follow a pattern. If the same set of
keys are exchanged from a location that does not follow the
established pattern, then the reputation score is reduced. Else it is
increased. When the reputation score reached a certain threshold the
keys are assumed to be genuine. 

\subsection*{Preliminaries}
\begin{itemize}
\item  Every mobile device is allocated a unique identity $D_1$
(either a phone number or IMSI number)
\item User $U_1$ registers with provider a $X_1$ using a device $W_1$
  with a unique identity $D_1$ 
\item If $W_1$ is directly connected to an authorized base station of
  provider $X_1$, then anyone who sends a message to identity $D_1$ is
  routed to $W_1$ and is received by user $U_1$.
%\item The routing layer within the cellular network is trusted
\end{itemize}


The step by step protocol is described as follows.

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1,c1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2,c2)S_2,c1 \\
 \textbf{3}.& \quad U_1 \rightarrow U_2: & & (c2)S_1 \\
 \textbf{4}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
 times} \\
 \textbf{5}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] User $U_1$ generates a self certifying key $P_1$ and
  signs the message consisting of location data $L_1$, time $t$,
  username $U_1$, user identity $D_1$ and challenge nonce $c1$. Here
  $L_1$ is the location data which might be the location of the cell
  tower combined with the GPS coordinates. $U_1$ sends the signed
  message $(L_1,t,U_1,D_1,c1)S_1$ and $P_1$ to $U_2$.

\item[\textbf{2.}] User $U_2$ generates a self certifying key $P_2$ and
  decrypts the message using the key $P_1$ sent in the message. $U_2$
  then signs the message consisting his location data $L_2$, time $t$,
  username $U_2$, user identity $D_2$ and reverse challenge nonce $c2$. User
  $U_2$ sends key $P_2$, challenge nonce $c1$ and signed message
  $(L_2,t,U_2,D_2,c2)S_2$ to $U_1$.

\item[\textbf{3.}] User $U_1$ decrypts message and sends the signed
  reverse challenge nonce $c2$ back to $U_2$. This completes the
  three-way handshake protocol.

\item[\textbf{4.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. We have to repeat the protocol $n$ times because
  the location information is untrusted. The rationale here is, an
  attacker might try to spoof the identity of $U_2$ once or twice, but
  repeatedly ($n$ times) masquerading the identity of $U_2$ is
  hard. So by repeating the protocol $n$ times, preferably from
  different locations, increases the chances of the user being $U_2$. 

\item[\textbf{5.}] If after $n$ times $(D_2, P_2)$ corresponds to
  $(L_1,L_2,t)$ then with high probability $U_1$ has established a
  secure connection with $U_2$.
\end{enumerate}

\subsubsection{Security Analysis}

In Step 1, $U_1$ generates a self certifying key $P_1$, signs the
message which contains the location data $L_1$, time $t$,
  username $U_1$, user identity $D_1$ and challenge nonce $c1$, and
  sends the message and $P_1$ to the other user $U_2$. As we discussed
  in the previous Section, the cellular network is one-way
  probabilistically secure. An adversary can spoof the cellphone
  number of $U_1$ and hijack the message. But if $U_2$ is present in
  the cellular network $U_2$ would also receive the message, since the
  message is being routed to $U_2$'s number. The adversary could
  create a fake base station within $U_2$'s vicinity and hijack the
  message. In this case $U_2$ would never receive the message. The
  adversary could continue the entire protocol with $U_1$. But this is
  a highly unlikely event due to the following reasons. i) the
  adversary has to be in the vicinity of $U_2$ at the exact moment
  when the message is sent to by $U_1$ to $U_2$. ii) during the entire
  course of the protocol the $U_2$'s cellphone has be switched off, so
  that $U_2$ can't join the network. If $U_2$ joins the network during
  the course of the protocol, $U_2$ would get an encrypted message
  from $U_1$ with no key to decrypt. This would alert $U_2$ about the
  MITM attack and $U_2$ could send a message to $U_1$ to abort the
  protocol. $U_1$ would receive messages from two different locations
  and because of this $U_1$ would abort the protocol. Another scenario
  is $U_2$ would switch on the phone during the repetitive location
  exchange step. This would again give $U_1$ different or
  inconsistent location information and $U_1$ would abort the protocol. 

In Step 2, $U_2$ first checks if the message sent by $U_1$ is
consistent. If not, it aborts the protocol. If the message is
consistent, $U_2$ generates its self
certifying keys and signs the message containing its location data
$L_2$, time $t$, username $U_2$, user identity $D_2$ and reverse
challenge nonce $c2$.  An adversary could spoof $U_1$'s message. So
$U_2$ does not have any guarantee that the message was indeed sent by
$U_1$. Only in step 5 of the protocol when the reputation score goes
above a certain threshold, $U_2$ would have established a secure key
exchange with $U_1$.

In Step 3, $U_1$ checks if the message sent by $U_2$ is consistent. If
not, $U_1$ aborts the protocol. Else, $U_1$ will sign a reverse
challenge response $c_2$ and send it to $U_2$.

{\em Reputation score:} In Step 4, $U_1$ stores $(D_2, P_2)$ and its
corresponding location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. Similarly, $U_2$ stores the $(D_1, P_1)$ and its
  corresponding location information and time $(L_1, L_2)$. In this
  step, the keys are exchanged $n$ times. Each time if the location
  and time information are consistent then the reputation score is
  increased by 1. If the time to send or receive the message is
  greater than a certain time $T$, then the reputation score is reset
  to zero and Step 4 is started again. An adversary could spoof the
  location and time message by performing a MITM attack, but since the
  step is performed $n$ at different locations and time periods, the
  adversary would not be able to modify the message such that either
  $U_1$ or $U_2$ would always get consistent location and time
  information. Also, if the message is inconsistent $k$ times, then
  the protocol is aborted. When the reputation score
  passes $n$, then $U_1$ and $U_2$ have exchanged keys with high
  probability. 

\subsection{Multi-Path spatio-temporal repetitive key exchange}

In section \ref{singlepath} we looked at single path key exchange protocol, where
just one channel (SMS) was used to exchange keys between two users. In
the section we discuss the multi-path key exchange protocol, where
multiple communication channels are used to exchange keys in a secure
manner. We introduce two such paths: IP-SMS and Bluetooth-SMS; both of
which are discussed in detail below. The assumption is that the attacker can compromise a single path
and the probability of attacking another path is very low. Thus, having more
than one path adds to the security. 

\subsubsection{IP and SMS}
The first protocol in the multi-path key exchange is a protocol that
uses an IP path and SMS to exchange keys. The user initiates the key exchange
handshake using IP channel. User A sends its data (A's number, A's location,
A's challenge, current time, A's public key) to a centralized server. Once A's
data is uploaded on the server successfully, A send the nonce to B via SMS. User
B when receives the SMS, uploads its own data on the server and sends the reply 
to A's challenge via SMS. User A receives the response, verifies it, stores B's
information in its table and fetches B's information from the server. A then replies
back to B with the challenge response which B receives and stores it in its table
after verifying it. It should be noted that the messages on the server are removed
as soon as the user fetches the data from the server.


The step by step protocol is described as follows.

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow IP: & & P_1,t_1,IP_1  \\
           .& \quad U_2 \rightarrow IP: & & P_2,t_2,IP_2  \\
 \textbf{2}.& \quad U_1 \rightarrow U_2: & & (L_1,t,U_1,D_1,c1)S_2 \\
 \textbf{3}.& \quad U_2 \rightarrow U_1: & & (L_2,t,U_2,D_2,c2,c1)S_1,\\
 \textbf{4}.& \quad U_1 \rightarrow U_2: & & (c1,c2)S_1 \\
 \textbf{5}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
 times} \\
 \textbf{6}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] $U_1$ and $U_2$ exposure their public keys $P_1$
  and $P_2$ respectively though an IP channel. The keys get deleted
  after a certain time period ($t_1$ and $t_2$). $IP_1$ and $IP_2$ are
  IP addresses where $P_1$ and $P_2$ were stored respectively. 

\item[\textbf{2.}] $U_1$ signs the message $(L_1,t,U_1,D_1,c1)$ where
  the message consists of 
  location data $L_1$, time $t$, username $U_1$, user identity $D_1$
  and challenge nonce $c1$. with 
  the public key $S_2$ and sends it to $U_2$ using SMS. $L_1$ is the
  location data which might be a one of, or a combination three types of
  location information, i) IP-geographic location, ii) cell tower
  information, and iii) GPS information.

\item[\textbf{3.}] $U_2$ decrypts the message and gets the challenge
  nonce $c_1$. $U_2$ signs the message $(L_2,t,U_2,D_2,c2,c1)$ and
  sends it back to $U_1$ using SMS. $L_2$ is the location data of the
  $U_2$ which might be one of, or a combination of i) IP-geographic
  location, ii) cell tower information, and iii) GPS information, as
  mentioned on the previous step. 

\item[\textbf{4.}] $U_2$ sends the signed nonces $c1$ and $c2$ to
  $U_2$. This completes the three-way handshake protocol. 


\item[\textbf{5.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. We have to repeat the protocol $n$ times because
  the location information is untrusted. $U_2$ also follows the same
  approach and verifies whether $(D_1, P_1)$ corresponds to
  $(L_1,L_2)$. 

\item[\textbf{6.}] By repeating the protocol $n$ times, the reputation
  score (as described in the previous section) either increases or
  decreases. Once the reputation score crosses a certain threshold,
   then with high probability $U_1$ has established a
  secure connection with $U_2$.

\end{enumerate}


\paragraph{Security Analysis}

In Step 1, $U_1$ and $U_2$ use publicly recognized IP to send or store
their respective public keys. Since each IP address can be
geographically mapped, the location information of both $U_1$ and
$U_2$ can be determined. Since we are assuming that the IP is public,
the adversary cannot spoof the location information. This initial location
information of $U_1$ and $U_2$ plays a significant role in the later
steps when the reputation score is computed.

In Step 2, $U_1$ signs the message with $U_2$ key and sends it to
$U_2$ using SMS. Note that this is a different channel than Step 1. In
Step 1, the IP-channel was used to get the key and location
information. In Step 2, since the channel used is SMS, the encrypted
message has to be go through the cellular route. As discussed earlier,
the cellular channel is one-way probabilistically secure. Therefore if
in Step 1 the adversary spoofed the user, then in Step 2, when the
message is sent using the cellular network it reaches the genuine user
with high probability. Once the message is sent if there is no
response within a certain period of time or if the response from $U_2$
is negative, this means that there is a MITM attack and the protocol
is aborted. 

In Step 3, if the message sent by $U_1$ reaches $U_2$, then $U_2$
sends back the response with a signed message with its location data
$L_2$, time $t$, username $U_2$, user identity $D_2$ and reverse 
challenge nonce $c2$.  An adversary could spoof $U_1$'s message. So
$U_2$ does not have any guarantee that the message was indeed sent by
$U_1$. Only in step 5 of the protocol when the reputation score goes
above a certain threshold, $U_2$ would have established a secure key
exchange with $U_1$.

In Step 4, $U_1$ checks if the message sent by $U_2$ is consistent. If
not, $U_1$ aborts the protocol. Else, $U_1$ will sign a reverse
challenge response $c_2$ and send it to $U_2$.

In Step 5 and 6, the protocol is repeated $n$ times to check for
consistency in the (key,location) pair. $U_1$ stores $(D_2, P_2)$ and its
corresponding location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. Similarly, $U_2$ stores the $(D_1, P_1)$ and its
  corresponding location information and time $(L_1, L_2)$. The
  reputation score is computed in the same manner as described in the
  single path key exchange protocol. The difference in the multi-path
  protocol is that initial exchange of keys using a different channel
  or path. The number of rounds of key and location information
  exchanges might be reduced, if Step 1 to Step 4 are consistent. This
  means the keys that were exchanged in Step 1 are being used in
  subsequent steps (in the cellular network) so there is a high
  probability that the users are genuine. 

\subsubsection{Bluetooth and SMS}
In this protocol, the users are in close proximity and Bluetooth is
used to exchange keys between them. Once the keys and the messages are
exchanged the users can communicate securely using SMS or other channels.
Bluetooth is an unreliable way of communication as described in \cite{bluetooth1}
and \cite{bluetooth2}. For added security, when user A opts Bluetooth as a mean
of key exchange the system asks for a password which both users: A and B; should
decide before starting the key exchange. Once they both enter the same password-
the key exchange process starts. User A sends its data (A's number, A's location,
A's challenge, current time, A's public key) to B via bluetooth. User
B when receives the SMS, sends its own data to A via Bluetooth and sends the reply 
to A's challenge via SMS. User A receives the SMS response, verifies it, stores B's
information in its table and when it receives B's data; replies
back to B with the challenge response via SMS which B receives and stores it in its table
after verifying it. 


\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2)S_2 \\
 \textbf{3}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
 times} \\
 \textbf{4}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}


\begin{enumerate}
\item[\textbf{1.}] $U_1$ sends the location information $L_1$, time
  $t$, username $U_1$, user identity $D_1$ to $U_2$ using Bluetooth. 

\item[\textbf{2.}] $U_2$ sends the location information $L_2$, time
  $t$, username $U_2$, user identity $D_2$ to $U_1$ using Bluetooth. 

\item[\textbf{4.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. 

\item[\textbf{5.}] If after $n$ times $(D_2, P_2)$ corresponds to
  $(L_1,L_2,t)$ then with high probability $U_1$ has established a
  secure connection with $U_2$.

\end{enumerate}

\paragraph{Security Analysis}

In Step 1 and 2, $U_1$ and $U_2$ exchange keys using Bluetooth which
means they are in close proximity to each other. But there is a
possibility that the $U_1$ has not met $U_2$ before and does not have
any information on $U_2$'s identity and vice-versa. Hence just the key
exchange using Bluetooth is not sufficient. The repetitive key
exchange protocol is necessary to ensure that the users are talking to
each other instead of the adversary. In Step 3 and 4, reputation score
is computed just as in earlier protocols. In the first step the
messages were exchanged using Bluetooth and in the subsequent steps
the messages were exchanged using SMS. If the messages are consistent
from Step 1 to Step 4 and the repetitive key exchange is performed as
described in the earlier protocols, then there is no MITM attack and
the users can communicate with each in a secure manner. 




==> Eurosys'16/Old Draft/SMIprotocol.tex <==
\section{The Secure Mobile Identities Protocol Details}

In this section we will discuss the DSMI protocol in detail using untrusted and trusted
location data gathered through GPS and cell tower and 3rd party services.

\subsection{Single Path Spatio-Temporal Repetitive Key Exchange}\label{singlepath}

In this protocol, only SMS is used to exchange keys between the
users. It is a one-way probabilistically trusted
path under the assumption that the SMS that is sent to a user is
always delivered to that user and that the network is trusted such that
there are no man-in-the-middle attacks possible.
The location information is not trusted, hence the protocol has
a repetitive procedure. Initially keys are exchanged using a simple
3-way handshake protocol where each user generates a self certifying
key. Once the initial 3-way protocol is completed, a reputation score
is maintained by each user. This score is increased based on the
location information obtained from the cell 
towers and the GPS. The assumption here is
the attacker will not follow the user at all times. So if the
adversary was impersonating the user a few times, his location will be
very different from the actual user's location. As the keys are
repetitively exchanged at different intervals of time the location
information is updated. As the user location behavior follows a
specific pattern repeatedly, the reputation score is increased. Same
set of keys are exchanged at different intervals and from different 
locations, where the locations follow a pattern. If the same set of
keys are exchanged from a location that does not follow the
established pattern, then the reputation score is reduced. Else it is
increased. When the reputation score reached a certain threshold the
keys are assumed to be genuine. 

\subsection*{Preliminaries}
\begin{itemize}
\item  Every mobile device is allocated a unique identity $D_1$
(either a phone number or IMSI number)
\item User $U_1$ registers with provider a $X_1$ using a device $W_1$
  with a unique identity $D_1$ 
\item If $W_1$ is directly connected to an authorized base station of
  provider $X_1$, then anyone who sends a message to identity $D_1$ is
  routed to $W_1$ and is received by user $U_1$.
%\item The routing layer within the cellular network is trusted
\end{itemize}


The step by step protocol is described as follows.

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1,c1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2,c2)S_2,c1 \\
 \textbf{3}.& \quad U_1 \rightarrow U_2: & & (c2)S_1 \\
 \textbf{4}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
 times} \\
 \textbf{5}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] User $U_1$ generates a self certifying key $P_1$ and
  signs the message consisting of location data $L_1$, time $t$,
  username $U_1$, user identity $D_1$ and challenge nonce $c1$. Here
  $L_1$ is the location data which might be the location of the cell
  tower combined with the GPS coordinates. $U_1$ sends the signed
  message $(L_1,t,U_1,D_1,c1)S_1$ and $P_1$ to $U_2$.

\item[\textbf{2.}] User $U_2$ generates a self certifying key $P_2$ and
  decrypts the message using the key $P_1$ sent in the message. $U_2$
  then signs the message consisting his location data $L_2$, time $t$,
  username $U_2$, user identity $D_2$ and reverse challenge nonce $c2$. User
  $U_2$ sends key $P_2$, challenge nonce $c1$ and signed message
  $(L_2,t,U_2,D_2,c2)S_2$ to $U_1$.

\item[\textbf{3.}] User $U_1$ decrypts message and sends the signed
  reverse challenge nonce $c2$ back to $U_2$. This completes the
  three-way handshake protocol.

\item[\textbf{4.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. We have to repeat the protocol $n$ times because
  the location information is untrusted. The rationale here is, an
  attacker might try to spoof the identity of $U_2$ once or twice, but
  repeatedly ($n$ times) masquerading the identity of $U_2$ is
  hard. So by repeating the protocol $n$ times, preferably from
  different locations, increases the chances of the user being $U_2$. 

\item[\textbf{5.}] If after $n$ times $(D_2, P_2)$ corresponds to
  $(L_1,L_2,t)$ then with high probability $U_1$ has established a
  secure connection with $U_2$.
\end{enumerate}

\subsubsection{Security Analysis}

In Step 1, $U_1$ generates a self certifying key $P_1$, signs the
message which contains the location data $L_1$, time $t$,
  username $U_1$, user identity $D_1$ and challenge nonce $c1$, and
  sends the message and $P_1$ to the other user $U_2$. As we discussed
  in the previous Section, the cellular network is one-way
  probabilistically secure. An adversary can spoof the cellphone
  number of $U_1$ and hijack the message. But if $U_2$ is present in
  the cellular network $U_2$ would also receive the message, since the
  message is being routed to $U_2$'s number. The adversary could
  create a fake base station within $U_2$'s vicinity and hijack the
  message. In this case $U_2$ would never receive the message. The
  adversary could continue the entire protocol with $U_1$. But this is
  a highly unlikely event due to the following reasons. i) the
  adversary has to be in the vicinity of $U_2$ at the exact moment
  when the message is sent to by $U_1$ to $U_2$. ii) during the entire
  course of the protocol the $U_2$'s cellphone has be switched off, so
  that $U_2$ can't join the network. If $U_2$ joins the network during
  the course of the protocol, $U_2$ would get an encrypted message
  from $U_1$ with no key to decrypt. This would alert $U_2$ about the
  MITM attack and $U_2$ could send a message to $U_1$ to abort the
  protocol. $U_1$ would receive messages from two different locations
  and because of this $U_1$ would abort the protocol. Another scenario
  is $U_2$ would switch on the phone during the repetitive location
  exchange step. This would again give $U_1$ different or
  inconsistent location information and $U_1$ would abort the protocol. 

In Step 2, $U_2$ first checks if the message sent by $U_1$ is
consistent. If not, it aborts the protocol. If the message is
consistent, $U_2$ generates its self
certifying keys and signs the message containing its location data
$L_2$, time $t$, username $U_2$, user identity $D_2$ and reverse
challenge nonce $c2$.  An adversary could spoof $U_1$'s message. So
$U_2$ does not have any guarantee that the message was indeed sent by
$U_1$. Only in step 5 of the protocol when the reputation score goes
above a certain threshold, $U_2$ would have established a secure key
exchange with $U_1$.

In Step 3, $U_1$ checks if the message sent by $U_2$ is consistent. If
not, $U_1$ aborts the protocol. Else, $U_1$ will sign a reverse
challenge response $c_2$ and send it to $U_2$.

{\em Reputation score:} In Step 4, $U_1$ stores $(D_2, P_2)$ and its
corresponding location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. Similarly, $U_2$ stores the $(D_1, P_1)$ and its
  corresponding location information and time $(L_1, L_2)$. In this
  step, the keys are exchanged $n$ times. Each time if the location
  and time information are consistent then the reputation score is
  increased by 1. If the time to send or receive the message is
  greater than a certain time $T$, then the reputation score is reset
  to zero and Step 4 is started again. An adversary could spoof the
  location and time message by performing a MITM attack, but since the
  step is performed $n$ at different locations and time periods, the
  adversary would not be able to modify the message such that either
  $U_1$ or $U_2$ would always get consistent location and time
  information. Also, if the message is inconsistent $k$ times, then
  the protocol is aborted. When the reputation score
  passes $n$, then $U_1$ and $U_2$ have exchanged keys with high
  probability. 

\subsection{Multi-Path spatio-temporal repetitive key exchange}\label{multi-path}

In section \ref{singlepath} we looked at single path key exchange protocol, where
just one channel (SMS) was used to exchange keys between two users. In
the section we discuss the multi-path key exchange protocol, where
multiple communication channels are used to exchange keys in a secure
manner. We introduce two such paths: IP-SMS and Bluetooth-SMS; both of
which are discussed in detail below. The assumption is that the attacker can compromise a single path
and the probability of attacking another path is very low. Thus, having more
than one path adds to the security. 

\subsubsection{IP and SMS}
The first protocol in the multi-path key exchange is a protocol that
uses an IP path and SMS to exchange keys. The user initiates the key exchange
handshake using IP channel. User A sends its data (A's number, A's location,
A's challenge, current time, A's public key) to a centralized server. Once A's
data is uploaded on the server successfully, A send the nonce to B via SMS. User
B when receives the SMS, uploads its own data on the server and sends the reply 
to A's challenge via SMS. User A receives the response, verifies it, stores B's
information in its table and fetches B's information from the server. A then replies
back to B with the challenge response which B receives and stores it in its table
after verifying it. It should be noted that the messages on the server are removed
as soon as the user fetches the data from the server.


The step by step protocol is described as follows.

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow IP: & & P_1,t_1,IP_1  \\
           .& \quad U_2 \rightarrow IP: & & P_2,t_2,IP_2  \\
 \textbf{2}.& \quad U_1 \rightarrow U_2: & & (L_1,t,U_1,D_1,c1)S_2 \\
 \textbf{3}.& \quad U_2 \rightarrow U_1: & & (L_2,t,U_2,D_2,c2,c1)S_1,\\
 \textbf{4}.& \quad U_1 \rightarrow U_2: & & (c1,c2)S_1 \\
 \textbf{5}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
 times} \\
 \textbf{6}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] $U_1$ and $U_2$ exposure their public keys $P_1$
  and $P_2$ respectively though an IP channel. The keys get deleted
  after a certain time period ($t_1$ and $t_2$). $IP_1$ and $IP_2$ are
  IP addresses where $P_1$ and $P_2$ were stored respectively. 

\item[\textbf{2.}] $U_1$ signs the message $(L_1,t,U_1,D_1,c1)$ where
  the message consists of 
  location data $L_1$, time $t$, username $U_1$, user identity $D_1$
  and challenge nonce $c1$. with 
  the public key $S_2$ and sends it to $U_2$ using SMS. $L_1$ is the
  location data which might be a one of, or a combination three types of
  location information, i) IP-geographic location, ii) cell tower
  information, and iii) GPS information.

\item[\textbf{3.}] $U_2$ decrypts the message and gets the challenge
  nonce $c_1$. $U_2$ signs the message $(L_2,t,U_2,D_2,c2,c1)$ and
  sends it back to $U_1$ using SMS. $L_2$ is the location data of the
  $U_2$ which might be one of, or a combination of i) IP-geographic
  location, ii) cell tower information, and iii) GPS information, as
  mentioned on the previous step. 

\item[\textbf{4.}] $U_2$ sends the signed nonces $c1$ and $c2$ to
  $U_2$. This completes the three-way handshake protocol. 


\item[\textbf{5.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. We have to repeat the protocol $n$ times because
  the location information is untrusted. $U_2$ also follows the same
  approach and verifies whether $(D_1, P_1)$ corresponds to
  $(L_1,L_2)$. 

\item[\textbf{6.}] By repeating the protocol $n$ times, the reputation
  score (as described in the previous section) either increases or
  decreases. Once the reputation score crosses a certain threshold,
   then with high probability $U_1$ has established a
  secure connection with $U_2$.

\end{enumerate}


\paragraph{Security Analysis}

In Step 1, $U_1$ and $U_2$ use publicly recognized IP to send or store
their respective public keys. Since each IP address can be
geographically mapped, the location information of both $U_1$ and
$U_2$ can be determined. Since we are assuming that the IP is public,
the adversary cannot spoof the location information. This initial location
information of $U_1$ and $U_2$ plays a significant role in the later
steps when the reputation score is computed.

In Step 2, $U_1$ signs the message with $U_2$ key and sends it to
$U_2$ using SMS. Note that this is a different channel than Step 1. In
Step 1, the IP-channel was used to get the key and location
information. In Step 2, since the channel used is SMS, the encrypted
message has to be go through the cellular route. As discussed earlier,
the cellular channel is one-way probabilistically secure. Therefore if
in Step 1 the adversary spoofed the user, then in Step 2, when the
message is sent using the cellular network it reaches the genuine user
with high probability. Once the message is sent if there is no
response within a certain period of time or if the response from $U_2$
is negative, this means that there is a MITM attack and the protocol
is aborted. 

In Step 3, if the message sent by $U_1$ reaches $U_2$, then $U_2$
sends back the response with a signed message with its location data
$L_2$, time $t$, username $U_2$, user identity $D_2$ and reverse 
challenge nonce $c2$.  An adversary could spoof $U_1$'s message. So
$U_2$ does not have any guarantee that the message was indeed sent by
$U_1$. Only in step 5 of the protocol when the reputation score goes
above a certain threshold, $U_2$ would have established a secure key
exchange with $U_1$.

In Step 4, $U_1$ checks if the message sent by $U_2$ is consistent. If
not, $U_1$ aborts the protocol. Else, $U_1$ will sign a reverse
challenge response $c_2$ and send it to $U_2$.

In Step 5 and 6, the protocol is repeated $n$ times to check for
consistency in the (key,location) pair. $U_1$ stores $(D_2, P_2)$ and its
corresponding location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. Similarly, $U_2$ stores the $(D_1, P_1)$ and its
  corresponding location information and time $(L_1, L_2)$. The
  reputation score is computed in the same manner as described in the
  single path key exchange protocol. The difference in the multi-path
  protocol is that initial exchange of keys using a different channel
  or path. The number of rounds of key and location information
  exchanges might be reduced, if Step 1 to Step 4 are consistent. This
  means the keys that were exchanged in Step 1 are being used in
  subsequent steps (in the cellular network) so there is a high
  probability that the users are genuine. 

\subsubsection{Bluetooth and SMS}
In this protocol, the users are in close proximity and Bluetooth is
used to exchange keys between them. Once the keys and the messages are
exchanged the users can communicate securely using SMS or other channels.
Bluetooth is an unreliable way of communication as described in \cite{bluetooth1}
and \cite{bluetooth2}. For added security, when user A opts Bluetooth as a mean
of key exchange the system asks for a password which both users: A and B; should
decide before starting the key exchange. Once they both enter the same password-
the key exchange process starts. User A sends its data (A's number, A's location,
A's challenge, current time, A's public key) to B via bluetooth. User
B when receives the SMS, sends its own data to A via Bluetooth and sends the reply 
to A's challenge via SMS. User A receives the SMS response, verifies it, stores B's
information in its table and when it receives B's data; replies
back to B with the challenge response via SMS which B receives and stores it in its table
after verifying it. 


\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2)S_2 \\
 \textbf{3}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
 times} \\
 \textbf{4}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}


\begin{enumerate}
\item[\textbf{1.}] $U_1$ sends the location information $L_1$, time
  $t$, username $U_1$, user identity $D_1$ to $U_2$ using Bluetooth. 

\item[\textbf{2.}] $U_2$ sends the location information $L_2$, time
  $t$, username $U_2$, user identity $D_2$ to $U_1$ using Bluetooth. 

\item[\textbf{4.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. 

\item[\textbf{5.}] If after $n$ times $(D_2, P_2)$ corresponds to
  $(L_1,L_2,t)$ then with high probability $U_1$ has established a
  secure connection with $U_2$.

\end{enumerate}

\paragraph{Security Analysis}

In Step 1 and 2, $U_1$ and $U_2$ exchange keys using Bluetooth which
means they are in close proximity to each other. But there is a
possibility that the $U_1$ has not met $U_2$ before and does not have
any information on $U_2$'s identity and vice-versa. Hence just the key
exchange using Bluetooth is not sufficient. The repetitive key
exchange protocol is necessary to ensure that the users are talking to
each other instead of the adversary. In Step 3 and 4, reputation score
is computed just as in earlier protocols. In the first step the
messages were exchanged using Bluetooth and in the subsequent steps
the messages were exchanged using SMS. If the messages are consistent
from Step 1 to Step 4 and the repetitive key exchange is performed as
described in the earlier protocols, then there is no MITM attack and
the users can communicate with each in a secure manner. 

\subsection{Trusted location based key exchange}

The location data gathered through GPS and cell tower is not trusted and can easily be manipulated.
We need a secure and trusted location gathering mechanism. By a trusted location we mean a location that
can not be changed by an attacker and is signed by a trusted 3rd party. The location data gathered through
these trusted points of location gathering devices is considered the most authentic and a user having a trusted
location gains more score points. There can be a number of ways to achieve this. We present a few of those
techniques in this paper. Instead of gathering location through GPS, this is an added security step that 
can be included in the DSMI protocol as explained in section \ref{singlepath} and \ref{multi-path}.

\subsubsection{Third-party trusted location devices}

A trusted 3rd party installs some of these certifying location gathering devices in a few places for a user to sync
their device and gets a certifying location along with a time stamp. The location data is actually the location
of that device and as the user is in close proximity of that device; the location of the user is the same as that
of the device. Syncing can be done via bluetooth or any other technology. This is something very trivial to do
as Google already has deployed its Google wallet points at various location. A user can sync up with the
Google wallet point and get a certifying location. 

\subsubsection{Geolocation}

Another way of gathering location data is through IP. As the public IP address of every device is unique and IP
addresses are assigned in the form of a tier system based on the geographical location. It is possible to gather
the location information through IP. Mapping IP addresses to a geographical location is known as Geolocation and is
described in \cite{taylor2012bringing}  and \cite{kovacs2002geolocation}. The idea is to have a trusted 3rd party
hotspot deployed at various location so that a user can sync the mobile to get a certifying IP location. The IP
location can further be processed as discussed above to break it down to geographical location. 


\subsubsection{Trusted location data}
\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1,c1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2,c2)S_2,c1 \\
 \textbf{3}.& \quad U_1 \rightarrow U_2: & & (c2)S_1 \\
\end{align*}
In this protocol, the location data ($L_1,L_2,t)$ is from a trusted
source. The GPS chip within the mobile devices $W_1,W_2$ are trusted
and the cell tower information obtained is also trusted. Hence the
protocol boils down to the three-way handshake protocol. 


\subsubsection{Trusted point of sale device}

\subsubsection*{Assumptions}
\begin{itemize}
\item Point of sale devices are trusted. 
\item Point of sale devices have the ability to sign a message and
  transmit the message securely to the device $W_1$ of the user $U_1$.
\end{itemize}

\subsubsection*{Protocol}

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow G: & & P_1,L_1,t,U_1,D_1  \\
 \textbf{2}.& \quad G \rightarrow U_1: & & G_P, (P_1,L_1,t,U_1,D_1)G_S \\
 \textbf{3}.& \quad U_1 \rightarrow C: & & P_1, (G_P,(P_1,L_1,t,U_1,D_1)G_S)S_1 \\
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] $U_1$ sends the message $P_1,L_1,t,U_1,D_1$ to a
  point of sale device $G$. 

\item[\textbf{2.}] A point of sale device can be a NFC
  device or other device which is capable to signing a message. The
  point of sale device $G$ signs the message $(P_1,L_1,t,U_1,D_1)G_S$
  and along with $G_P$ (public key) sends it back to $U_1$.

\item[\textbf{3.}] Now $U_1$ signs the message it received from $G$,

  ($P_1$,$L_1$,$t$,$U_1$,$D_1$)$G_S$)$S_1$ and sends it to the central
  authority $C$ along with $P_1$. Since $G$ is trusted (has trusted
  credentials), $C$ is certain that the message is signed by $G$ and
  that $U_1$ was indeed present at the point of sale location. The
  point of sale device could also have a fingerprint reader (or any
  biometric device) to authenticate user's identity and the biometric
  data can also be part of the signed message from $G$ to $U_1$. 
\end{enumerate}



==> Eurosys'16/Old Draft/abstract-new.tex <==
\begin{abstract}

%motivation%
The proliferation of cell phones has brought out issues in security
as they are becoming more and more vulnerable as targets 
for attack \cite{cyberThreats} like man-in-the-middle (MITM) attacks and 
phishing attacks where an attacker may trick the user by masquerading 
as a trustworthy entity. 
%related work 2-3%
Methods like SSL/TLS-a third party service,
apps which use one-time PIN and passwords, protocols that require the users to be there
physically are some of the examples of the efforts made to solve this issue.
%DSMI 3-4%
In this paper we propose the design
and implementation of Secure Mobile Identities (DSMI), a protocol that promises a 
secure and reliable communication by exchanging and authenticating keys.
The key idea of DSMI is to provide a spatio-temporal, multi-path, repetitive 
challenge-response key exchange protocol to enable two mobile entities to 
builds up reputation across multiple levels of trust.
%Applications 1-2%
Many new and existing applications can be built on top of DSMI which require sensitive data handling
such as apps that involve money transactions or apps that involve sensitive data transaction. 
%evaluation results%
In this paper we show the protocol 
implementation and evaluation across variety of channels. 



\begin{comment}
%motivation%
The proliferation of cell phones has brought out issues in security
which is causing a major problem worldwide. 
Mobile phones are becoming more and more vulnerable as targets 
for attack \cite{cyberThreats}. Some major security threats that a 
common user is facing are man-in-the-middle (MITM) attacks and 
phishing attacks where an attacker may trick the user by masquerading 
as a trustworthy entity. 

%related work 2-3%
Methods like SSL/TLS-a third party service,
apps which use one-time PIN and passwords, protocols that require the users to be there
physically are some of the examples of the efforts made to solve this issue.

%DSMI 3-4%

In this paper we propose the design
and implementation of Secure Mobile Identities (DSMI), a protocol that promises a 
secure and reliable communication by exchanging and authenticating keys.
The key idea of DSMI is to provide a spatio-temporal, multi-path, repetitive 
challenge-response key exchange protocol to enable two mobile entities to 
builds up reputation across multiple levels of trust. DSMI tags keys with 
location and time and populates the table for 
the same traditional (identity, key) pair.

%Applications 1-2%
\\Many new applications can be built on top of DSMI which require sensitive data handling
such as apps that involve money transactions or apps that involve sensitive data transaction. 

%evaluation results%
\\In this paper we show the protocol 
implementation and evaluation across variety of channels. 
\end{comment}
\end{abstract}

==> Eurosys'16/Old Draft/abstract.tex <==
\begin{abstract}
Mobile devices are increasingly becoming vulnerable to a variety of
network-level security threats including different types of
man-in-the-middle (MITM) attacks such as message interceptions and
modifications, eavesdropping on calls and text messages, message
spoofing and phishing attacks. In this paper, we propose the design
and implementation of Secure Mobile Identities (DSMI), a secure
key-exchange protocol that enables a mobile user to establish a secure
and trustworthy communication channel with other mobile users in the
face of external adversaries.  The design of DSMI places initial
bootstrap trust on the cellular providers and builds upon the basic
assumption that cellular networks offer a unique ``partially
trustworthy one-way'' channel to connected mobile devices; unlike
Internet routes which can be hijacked, the cellular network routing
layer is closed thereby forcing the MITM attacker to attack only the
last-hop wireless channel between the tower and the device. Building
on this assumption, DSMI provides a spatio-temporal, multi-path,
repetitive challenge-response key exchange protocol to enable two
mobile entities to tag every key exchange with a (location, time,
path) triplet and leverage diversity across paths to build a trust
reputation for every key. The security of DSMI can be further enhanced
with the use of external trusted entities providing non-forgeable
trusted location signatures (e.g. trusted GPS, trusted cell towers,
physical synchronization points). In this paper, we demonstrate the
effectiveness of our protocol using a prototype implementation and
demonstrate ease of use across a variety of real-world channels. We
also show how the DSMI abstraction can enable new forms of secure
mobile applications including secure cash transfer, secure physical
identities and secure file exchange.

\end{abstract}



==> Eurosys'16/Old Draft/abstract_mod.tex <==
\begin{abstract}
The proliferation of cellphones has brought out issues in security
which is causing major problems worldwide. 
Recent reports suggests that due to vulnerabilities in the network, 
security loopholes exist which puts the users at risk to
attackers\cite{cyberThreats}. Man-in-the-middle (MITM)
attacks such as snooping, eavesdropping on phone calls and text
messages, to jamming the channel to block access to secure session
,phishing attacks where an attacker may trick
the user by masquerading as a trustworthy entity, have been
increasing. In this paper we present the design and implementation of
Secure Mobile Identities (DSMI), a key exchange protocol that helps the
users to communicate in a secure manner. 
The key idea of DSMI is to provide a spatio-temporal, multi-path, repetitive 
challenge-response key exchange protocol to enable two mobile entities
to develop trust in order to communicate securely. Assuming the
cellular network is a trusted one way probabilistic path, we use self
certifying keys, location of the devices and communication
channels in different ways to increase the trust in the mobile
identity of each person. 
We develop a real world implementation and evaluate the protocol
across a variety of communication channels. 

\end{abstract}


==> Eurosys'16/Old Draft/appANDeval.tex <==
\section{Applications and Evaluation}

There can be various applications that can be built on top of Secure Mobile
Identities protocol. DSMI promises security and reliability along with usability.
DSMI does not involve any user involvement and the simplicity of DSMI makes
it favorable to be adapted in existing as well as new applications.
To evaluate the usability of Secure Mobile Identities usability
we conducted trial runs and tests to gather stats.

\subsection{Applications}

We present here some of the ideas of the applications which we think can be built
on top of DSMI protocol seamlessly. 

\subsubsection{Secure Cash}
We can leverage DSMI to build an app that requires the most security. We can build a virtual
cash system on top of DSMI which can be used as the security layer. The bank is a trusted 
party whose secure cash app would allow its customers to perform secure digital transactions.
The secure cash is the implementation of the process of sending and receiving a bank transaction 
through an app, removing the requirements of a cash register. 
Electronic transactions can be done with or without the presence of a designated point of sale.
Alice wants to buy a dress, from a store which is registered with her bank and has a trusted 
location device, using her secure cash app. She opens the application and scans/takes a picture 
of the bar-code of the dress and sends it to her bank using the pre-installed trusted location device 
in the shop. Alice's phone performs the three-way handshake using the trusted location device at the
shop with the bank. The bank authenticates the location and evaluates the trust level of Alice and 
sends a receipt to the shop indicating that the transaction has been taken place.

Another important scenario using secure cash can be the cash receipt system and it can be useful in places
where banks/ATM/credit card transactions are not widely accessible. Alice who wants to transfer money to
Bob's account; uses the secure cash application to do so; signs a cheque and sends it to Bob after 
completing a secure key exchange handshake. Bob on receiving the cheque goes to the bank where it gets
scanned and receives the money.

\subsubsection{Safe and Secure Virtual Identity}
Documents like passport, SSN, driver's license, property documents etc are very sensitive and need to be
kept at a safe location at all times. Applications can be built on top of DSMI that can encrypt these files
and send them to the trusted intended party or user without physically sending the documents. Using DSMI 
would help the sending and the receiving party be sure that the document is actually received from the
actual owner and is received by the intended user.


\subsection{Evaluation}

We wanted to test how long it takes for a user to complete the key
exchange handshake as it involves exchanging multiple text messaging.
The results depends on the network used for sure. Our tests were
conducted in Abu Dhabi, UAE using Etisalat \cite{etisalat} as our 
telecommunications services provider. 
We used java's function for time calculation to get time in nanoseconds.
We recorded the current time in nanoseconds. We used two ways to get the time: the phone
is linked with a PC via bluetooth and both phones signals the PC to record the
time (to get time of one machine) and for more accuracy we used the phones
to record their times themselves (to account for any delays caused while
transmitting the messages via bluetooth).
Time 1a is the time required to start the transaction by phone A and when phone
B replies back with its own data. Time 1b is the time recorded from the moment
phone B sends back its own data until it receives the challenge reply by A.
Both these times: Time 1a and Time 2a are taken by the PC connected via
bluetooth to both phones.
Time 1b and 2b is the same time as Time 1a and 2a, the difference is the
way the time is recorded. 1b and 2b are recorded on phone A and phone B
themselves.
Time a is the time required by phone A to send data to phone B. It is calculated
by getting the time in nanoseconds when user using phone A clicks send; phone
A sends an alert to PC to record the current time via bluetooth. Phone B when
receives the message sends an alert to PC to record the current time.
\\Time b is the time recorded when phone B sends its own data to A and the time
A receives it. Time c is the time required when A sends the challenge reply to
phone B and B receives it.

\subsubsection{Observations and Results}

We used a PC for recording the time when the phone sends a signal using bluetooth. 
We also used phones themselves to record the time. Using another device, in our case
the PC, for recording time can cause delays and by using two different devices for
recording time can create the difference in time. Figure \ref{timeDif} shows the difference
in times. Time 1 is the time taken by phone A to send meta-data to phone B 
and phone B replies back with encrypted challenge reply and its own metadata to phone A.
Time 2 is the time taken by phone B to send the encrypted challenge reply and its 
own metadata to phone A and phone A replies with the challenge reply. This figure shows that
the difference between the two is not very significant and we can use the average number to 
add into the results for an approximate time calculation.


\begin{figure}[htb]
    \centering
		\subfigure[{\smallTime difference for time 1: time taken by phone A to send meta-data to phone B and gets back a response}]
		{
				\includegraphics[width=0.45\columnwidth]
				{C:/Users/fa45/Dropbox/secmobid/tex/analysis/DiffTime1.jpg}
    }
		\subfigure[{\small Time difference for time 2: time taken by phone B to send the encrypted challenge reply and its 
own metadata to phone A and gets back a response}]
		{
				\includegraphics[width=0.45\columnwidth]
				{C:/Users/fa45/Dropbox/secmobid/tex/analysis/DiffTime2.jpg}
        
		}
		\caption{The time difference recorded}
		\label{timeDif}
\end{figure}


We measure the total amount of time needed to complete the 3-way key exchange
handshake by all paths.
Figure \ref{ttime} shows the timing analysis. According to this figure, for the
SMS the maximum time taken in all the tests was approximately 120seconds and the
minimum time taken was approximately 70seconds. The average is approximately 95seconds.
This means on average a user has to wait for up to 95seconds to start the exchanging
the messages with the intended user.

\begin{comment}

\begin{figure}[htb]
    \center{\includegraphics[width=2in]
        {C:/Users/fa45/Dropbox/secmobid/tex/analysis/totalTimeTaken.jpg}}
    \caption{\label{ttime} Total time taken for 3-way key exchange}
\end{figure}


\begin{figure}[htb]
    \center{\includegraphics[width=2in]
        {C:/Users/fa45/Dropbox/secmobid/tex/analysis/TIMEabc.jpg}}
    \caption{\label{timeabc} Time a-SMS path, Time b-data/SMS path and Time c-bluetooth/SMS path}
\end{figure}


\begin{figure}[htb]
    \centering
		\subfigure[{\small Total time taken for 3-way key exchange}]
		{
				\includegraphics[width=0.45\columnwidth]
				{C:/Users/fa45/Dropbox/secmobid/tex/analysis/totalTimeTaken.jpg}
    }\label{ttime}
		\subfigure[{\small Time a-SMS path, Time b-data/SMS path and Time c-bluetooth/SMS path}]
		{
				\includegraphics[width=0.45\columnwidth]
				{C:/Users/fa45/Dropbox/secmobid/tex/analysis/TIMEabc.jpg}
        
		}\label{timeabc}
\end{figure}
\end{comment}

Figure \ref{timeabc} shows time taken by all path. Time taken by data/SMS path is the most and depends on the
upload and download speed as well the time taken by the cellular service provider for receiving
and sending an SMS.


\begin{figure}[ht]
	\begin{minipage}[b]{0.45\linewidth}
		\centering
			\includegraphics[width=\textwidth]{C:/Users/fa45/Dropbox/secmobid/tex/analysis/totalTimeTaken.jpg}
			\caption{{\small Total time taken for 3-way key exchange}}
			\label{ttime}
	\end{minipage}
	\hspace{0.5cm}
	\begin{minipage}[b]{0.45\linewidth}
		\centering
			\includegraphics[width=\textwidth]{C:/Users/fa45/Dropbox/secmobid/tex/analysis/TIMEabc.jpg}
			\caption{{\small Time a-SMS path, Time b-data/SMS path and Time c-bluetooth/SMS path}}
			\label{timeabc}
	\end{minipage}
\end{figure}





==> Eurosys'16/Old Draft/flow.tex <==
1, Introduction

No good solution for mobile security
Too much trust on the cellular base station
Attacks are for real

Secure Mobile Identities problem
Key Contributions
Key Ideas

Implementation and Eval results



2. Threat Model and Security Overview

Assumptions
Phone is trusted
The Real Cellular Network is not an adversary

Threat
Fake base stations
Man in the Middle Attackers
Channel eavesdropping and jammers


3. Related Work


4. One-way Probabilistic Secure Cellular Channels

Cellular Voice and SMS channel
Under what assumptions does it give the One-way probabilistic secure channel
abstraction.



5. Single Path Spatiotemporal Repetitive Key Exchange Protocol

3-way handshake over SMS channel alone

How to measure reputations after repetitive exchange?

Security guarantees of the protocol under the probabilistic security guarantee?

Detecting an attacker? - adding a repetitive checking protocol (did you actually exchange keys with me?)



6. Multi-Path Spatiotemporal Repetitive Key Exchange

The IP path (Scenario 1b)

The Bluetooth path (Scenario 3 - physical handshake)

Reputation computation

Security guarantees




7. Trusted Locations

Trusted Cell towers 

Trusted GPS 

Google Wallet Model

The Trusted IP model?

Security guarantees in the face of non-forgeable locations




8. Trusted Fingerprints

User fingerprint based exchange?

Device Fingerprint based exchange?


9. Implementation


10. Evaluation



11. Conclusions


==> Eurosys'16/Old Draft/implementation.tex <==
\section{Implementation}

Android was selected as our target operating system primarily because of the availability and cost of the android phones. We used the android 
SDK for Eclipse as our development environment which we downloaded from the official android website. For implementation we used two Samsung 
Galaxy Young (GT-S5360) phones having Android version 2.3.6 installed on them. For implementing the Bluetooth part we downloaded the BlueCove
 Java library from the BlueCove website.
\\Android crypto library was used for RSA encryption. The RSA keys used are 2048-bit long; we chose this key size for security purposes. 
A 2048-bit long RSA key can encrypt 215-bytes of data; which is roughly the size of data we want to encrypt. We generate a random, 128-bytes 
long nonce in our implementation for maximum security purposes. The phone stores the RSA keys generated for itself in the 
Android's shared preferences for the app. Shared Preferences in Android are stored as a file within the application's 
data directory with file permissions set that allow only that application to access it. For the rest of data that we 
want to store goes into a SQLite database for storing public keys of other phones and messages. Metadata used in all the 
interactions is the phone number location and the current time of the phone that is generating the metadata. The time includes 
the seconds, hours, date, month and year. 
\\All the messages, we receive and through whatever channel we are sending it through, have a specific header that helps the application 
in determining what to do with it. In our application we have a SMS receiver class that checks whether the SMS is supposed to be 
processed by our application; our protocol SMS; or is it just a regular SMS. If it is the SMS that our application needs to process then we do not let the SMS go to the Android phone's default application for receiving SMS; thus making sure that the SMS used for our application remains private. If it 
is a regular SMS then the application discards it and sends to the Android phone's default SMS application. SMS in our 
application are used for the following purposes: sending metadata, location and key; sending challenges and sending signed challenge replies.
Bluetooth channel works in pretty much the same way as the SMS channel but it has an added security feature 
of providing a password before starting key-exchange. The signed verification is not sent through the Bluetooth channel instead it is 
sent through SMS.
\\The signed verification in our data path is also sent through SMS. The phones connect to our server 
to send and receive messages. One phone uploads the message with a randomly generated, 128-byte long nonce on the server and 
sends the nonce to the other phone via SMS.


\begin{comment}
\\ Figure \ref{sms} shows how SMS are being exchanged between two phones A and B. A generates metadata and nonce and stores them in 
its database for verification later. It then sends them and its public key to B via SMS. B when receives the text message 
containing this information stores the public key of A in its database. It signs the metadata and nonce of A using its 
private key and generates its own metadata and nonce and sends it to A including its public key. 

\begin{figure}[htb]
    \center{\includegraphics[width=3in]
        {C:/Users/fa45/Dropbox/secmobid/tex/SMS.jpg}}
    \caption{\label{sms} SMS exchange between two phones: A and B}
\end{figure}
			
			
When A receives this reply, it fetches the metadata and nonce it generated before sending the message to B from the database, 
decrypts the challenge using B's public key and compares the two. If they are equal it stores B's public key, B's location and 
the path it used to send i.e. SMS in its database. It then signs the metadata and nonce sent by B using its private key and then 
sends this to B. B fetches: the public key of A to decrypt the challenge, the metadata and nonce it generated before sending them 
to A and compares the two. If the two are the same it stores them in its database. 

\begin{figure}[htb]
    \center{\includegraphics[width=3in]
        {C:/Users/fa45/Dropbox/secmobid/tex/Bluetooth.jpg}}
    \caption{\label{bluetooth} Message exchange between two phones: A and B; using Bluetooth (in blue) and SMS (in orange)}
\end{figure}

\\ Figure \ref{bluetooth} shows the exchange of messages using an alternate path: Bluetooth. When A wants to send a message to B using Bluetooth 
it enters a password which should also be known to B. If both passwords match then the following happens. A generates and stores metadata
 and nonce and sends it via Bluetooth to B. B receives it, generates and stores its own metadata and nonce and save it along with the public
 key of A. B sends metadata and nonce it generated to A via Bluetooth and it signs metadata and nonce of A and sends it using SMS channel.
 A gets the metadata and nonce and the message containing and verifies it. If the match it sends an SMS to B containing signed metadata 
and nonce of B.

\begin{figure}[htb]
    \center{\includegraphics[width=3in]
        {C:/Users/fa45/Dropbox/secmobid/tex/Data.jpg}}
    \caption{\label{data} Message exchange between two phones: A and B; using data}
\end{figure}
	

\\ Figure \ref{data} shows how we are sending messages from A to B. The basic protocol is the same. A generates and stores the metadata and the 
nonce. It creates another nonce and stores the message with a reference to the new nonce and sends an SMS to B to fetch the message using 
the new nonce. B fetches the messages from the server and the server deletes the message. Then B signs the metadata and nonce sent by A 
and sends it using SMS. Then B generates its own metadata and nonce and sends it to A in the same way.
The metadata includes the location of the phone. In order to get a certifying location the phone connects to one of 
the certifying Bluetooth device and gets a certifying location in return. The phone and the certifying Bluetooth device 
know a key. The certifying Bluetooth device sends its own public key, location and time to live signed with the known key to the device.
\end{comment}


==> Eurosys'16/Old Draft/intro-new.tex <==
\section{Introduction}

Security loopholes exists due to vulnerabilities in the network which puts 
the users at risk to attackers~\cite{securityVul}\cite{securityVul2}. A recent advancement 
in attacks on Global System for Mobile Communications (GSM) security has shown that
anybody with some skill can use the techniques and hardware 
to eavesdrop or record GSM cell phone calls~\cite{PerezAttack}.
Security issues range from man-in-the-middle (MITM)
attacks such as snooping, eavesdropping on phone calls and text
messages, to jamming the channel to block access to secure session
thereby causing disruption in the service. 
While SSL/TLS~\cite{oppliger2008ssl} is used in secure web transactions, most of the
transactions in the mobile world is through apps. Researchers have
noted that SSL is not always enabled in apps and there is no easy way to
check whether the traffic between the mobile app and the server is
encrypted~\cite{SSL/TLSVul}. Due to these issues it is
hard to conduct reliable secure transactions between users.

There have been efforts to enhance the security of mobile
devices. Apps such as Lookout Security \cite{lookoutSecurity} and others use PINs and
passwords to conduct transactions. But their security models and
processes do not depend on the identity of the person involved in the
transaction. If the password or PIN is stolen then the so called
secure wallet is exposed to the attackers. There have been efforts by
few companies to provide one-time PIN authentication which gives the
user the ability to input a one-time PIN before opening the
application or conducting a transaction~\cite{haller1995s};
and two-factor authentication~\cite{financial2007two}\cite{lakshmiraghavan2013two},
which allows users to authenticate using the debit cards and the pin. 
But since the PIN is a one
time solution and there is no guarantee that the PIN reached the user
or not, the security of this model can be compromised. 

%The design of DSMI places initial
%bootstrap trust on the cellular providers and builds upon the basic
%assumption that cellular networks offer a unique ``partially
%trustworthy one-way'' channel to connected mobile devices; unlike
%Internet routes which can be hijacked, the cellular network routing
%layer is closed thereby forcing the MITM attacker to attack only the
%last-hop wireless channel between the tower and the device.

In this paper we introduce a new protocol; Secure Mobile Identities (DSMI); 
to provide reliable identities
of the user thereby enabling secure transactions. DSMI guarantees that the user is
communicating only with the intended users.
DSMI is built over the trusted security layer provided by the cellular network. We assume that it is a
`partial trustworthy' channel as a user gets authenticated by the cell tower and once the user
is on the network, he/she will always get messages sent to them.
In our solution, we generate a secure mobile identity of a user and share it
to other users via different paths. Third party solutions like 
SSL/TLS~\cite{oppliger2008ssl}, used in secure web transactions requires all
web services to go through the certification authority to validate the credentials.
The identity assigned to each device and its
authentication is done using a decentralized approach in our protocol.

DSMI uses multiple paths for exchanging keys and
verification. The idea behind this is that if a certain path is compromised, 
the verification is always done via SMS based on our trust assumption. The probability of both channels being 
compromised is very low. DSMI maintains a list of users with their keys along
with their location and time. It creates different levels of trust depending
on how reliable the location information is and from how many different paths
the user has tried to contact the intended user. Using multiple paths has been
proposed to be a better authentication scheme
\cite{bauckman2013multi}\cite{abdurrahman2013new}\cite{dispensa2007multi}\cite{weber2010multi}.

DSMI is a repetitive spatio-temporal key exchange method. The users exchange
their keys across various location at different times. By repetitively exchanging keys
over different locations-the users develop trust or a strong identity. DSMI maintains a {\textit{trust score}}
against each user. The higher the score is the stronger the identity is.
Since location can be tapered in a variety of ways~\cite{GPSTemper}\cite{bland2008gps} and that would weaken our protocol; DSMI
introduces other methods for secure location. One idea is using a trusted location sync interface like
Google wallet~\cite{googleWallet} or using geolocation~\cite{katz2006towards}. By syncing with the Google wallet device, the mobile can get a certifying location of 
the wallet or the user can map his/her IP addresses to the geographical location and that would earn more trust score for the user.

Many applications can be developed on top of DSMI and many existing applications can extend DSMI
using it as the security layer. Applications
as data sensitive as mobile banking can be built leveraging DSMI. It can particularly be useful in
places where access to banks is not easy. Other applications
involving private photo exchange and file exchange can be built using DSMI.

We implemented the android version of DSMI. It is a very user friendly in a way
that only requires the user to enter the number of the intended user, rest of
the work is done in the background without any user involvement, which
makes this application very trivial to use. Secure
Mobile Identities is not platform specific which makes it even more diverse and scalable.


\begin{comment}
DSMI does not require third party solutions and it is built on minimum trust assumptions.
SSL/TLS~\cite{oppliger2008ssl}, used in secure web transactions requires all
web services to go through the certification authority to validate the credentials.
The identity assigned to each device and its
authentication is done using a decentralized approach in our protocol.
DSMI is built over the trusted layer provided by the cellular network. We assume that it is an
almost reliable delivery path in a way that the text messages are always delivered to the
intended recipient and the cellular network is trusted.


Users regularly face a problem of mobile security which is why they suffer of 
crisis of confidence. Recent reports suggests that due to vulnerabilities in the network, 
security loopholes exist which puts the users at risk to
attackers~\cite{securityVul}\cite{securityVul2}. The users doubt whether the message is actually sent by
the claimed person or if their conversation is being eavesdropped. A recent advancement 
in attacks on Global System for Mobile Communications (GSM) security has shown that it 
is now trivial to intercept or record GSM cell phone calls. Anybody with some skill can 
use the techniques and hardware described by Chris Paget~\cite{PerezAttack} to eavesdrop or 
record GSM cell phone calls.
\end{comment}

==> Eurosys'16/Old Draft/intro.tex <==
\section{Introduction}

Users regularly face a problem of mobile security which is why they suffer of 
crisis of confidence. Recent reports suggests that due to vulnerabilities in the network, 
security loopholes exist which puts the users at risk to
attackers. The users doubt whether the message is actually sent by
the claimed person or if their conversation is being eavesdropped. A recent advancement 
in attacks on Global System for Mobile Communications (GSM) security has shown that it 
is now trivial to intercept or record GSM cell phone calls. Anybody with some skill can 
use the techniques and hardware described by Chris Paget \cite{PerezAttack} to eavesdrop or 
record GSM cell phone calls.

\\Security issues range from man-in-the-middle (MITM)
attacks such as snooping, eavesdropping on phone calls and text
messages, to jamming the channel to block access to secure session
thereby causing disruption in the service. 
While SSL/TLS is used in secure web transactions, most of the
transactions in the mobile world is through apps. Researchers have
noted that SSL is not always enabled in apps and there is no easy way to
check whether the traffic between your mobile app and the server is
encrypted. Due to these issues it is
hard to conduct reliable secure transactions between users. Since the
communication channel is insecure, there is no good solution which a
service (or service provider) could use in which the identity of the
user is guaranteed. This mobile 
security issue is a major problem and because of this there hasn't
been any reliable way to conduct secure transactions where the mobile
device and user's identity is guaranteed to be genuine. 


\\In this paper we introduce new protocols to provide reliable identity
of the user thereby enabling secure transactions. We provide protocols
that enable two or more parties to transaction in a secure manner,
where with high probability each party is guaranteed that it is
communicating with other genuine parties. A number of applications can be built on
top of these protocols that enable secure transfer of messages, secure
transfer of funds. mobile payments etc.  

There have been efforts to increase the security of mobile
devices. Apps such as Lookout Security \cite{lookoutSecurity} and others use PINs and
passwords to conduct transactions. But their security models and
processes does not depend on the identity of the person involved in the
transaction. If the password or PIN is stolen then the so called
secure wallet is exposed to the attackers. There have been efforts by
few companies to provide two-factor authentication, which gives the
user the ability to input a one-time PIN before opening the
application or conducting a transaction. But since the PIN is a one
time solution and there is no guarantee that the PIN reached the user
or not, the security of this model can be compromised. 

\\In our solution we use self certifying keys which are exchanged by the
users in addition to their location and identity information in a
specific manner providing a much stronger security guarantee than the
earlier efforts in the area. DSMI uses multiple paths for exchanging keys and
verification. The idea behind this is that if a certain path is compromised, 
the verification is always done via SMS. The probability of both channels being 
compromised is very low. DSMI maintains a list of users with their keys along
with their location and time. It creates different levels of trust depending
on how reliable the location information is and from how many different paths
the user has tried to contact the intended user.

\\We implemented the android version of DSMI. It is a very user friendly in a way
that only requires the user to enter the number of the intended user, rest of
the work is done in the background without any user involvement, which
makes this application very trivial to use. Closely related work includes
SafeSlinger \cite{safeslinger} which requires the users to be present; physically
or virtually; with each other at the same time as the keys are being exchanged. Secure
Mobile Identity is not platform specific which makes it even more diverse and scalable.

\\The organization of this paper is as follows: In section 2 we will describe the problem
definition and threat model. In section 3 we discuss some of the closely related work and
how DSMI is different that them. We give the overall general setup in section 4. ...






==> Eurosys'16/Old Draft/location.tex <==
\section{Identifying location}

In this section, we try to answer the following question: can we
correctly identify the physical location of a cellphone? Either using
the location information from the cell towers or GPS information
present on the phone, nearby Wifi signals etc. 

Nowadays, Android and other mobile operating systems use various
techniques for pin pointing the location of the cellphone. 


\section{Techniques}


==> Eurosys'16/Old Draft/protocol.tex <==
\section{Protocol}

\begin{itemize}
\item GSM security is broken. Therefore, we need end-to-end security
mechanism to make sure that mobile banking and other security
applications implemented on top of GSM are always secure.
\item We plan to develop a protocol that satisfies certain security
  guarantees.
\item The central question is: how do you establish a secure
  communication channel between two mobile devices?
\end{itemize}

\subsection{Outline}
The device is associated with a username, a cellphone number, a set of
keys, a GPS location, cellular base station connection information,
set of self-certifying signatures and challenge-response signatures.
Let,  U - username, N - Mobile number, L - Location, P - Self
certifying key, c - challenge-response signature. 
Let $U_A,N_A,L_A,P_A, c_A$ be the properties of mobile device A and $U_B,
N_B, L_B, P_B, c_B$ are the properties of mobile device B.

The outline of the 3-way handshake protocol is as follows. 

\begin{align*}
 \textbf{1}.& \quad  D_A\rightarrow D_B: & & sign(M_A) \\
           .& \quad : & & \text{where}, M_A = (U_A, N_A, L_A, P_A, c_A)\\
 \textbf{2}.& \quad D_B \rightarrow D_A: & & sign(M_B), sign(c_A) \\
	   .& \quad : & & \text{where}, M_B = (U_B, N_B, L_B, P_B,
           c_B)\\
\textbf{3}.& \quad D_A \rightarrow D_B: & & sign(c_B)
\end{align*}

\textbf{1.} Device $D_A$ encrypts or signs message $M_A$ which
consists of $U_A, N_B, L_B, P_B, c_A$, using its key and sends it to
device $D_B$. 

\textbf{2.} Device $D_B$ signs $M_B$ which consists of $U_B, N_B, L_B,
P_B, c_B$, signs $c_A$ and sends it to $D_A$.

\textbf{3.} Device $D_A$ signs $c_B$ and sends it to $D_B$.

Repeat the 3-way handshake protocol across different $L_i$ (locations), at
different points in time. If $P_A$, $P_B$ are consistent after
repetitions, then both $D_A$ and $D_B$ have higher confidence that
they are talking to each other. This type of asynchronous method of
device pairing would help in thwarting some of the security flaws in
the underlying GSM channel.


\cite{Lin09spate}

==> Eurosys'16/Old Draft/protocols.tex <==
\section{Single path spatio-temporal key exchange}

In this protocol, only SMS is used to exchange keys between the
users. The location information is not trusted, hence the protocol has
a repetitive procedure. Initially keys are exchanged using a simple
3-way handshake protocol where each user generates a self certifying
key. Once the initial 3-way protocol is completed, a reputation score
is maintained by each user. This score is increased based on the
location information obtained from the cell 
towers and the GPS. The assumption here is
the attacker will not follow the user at all times. So if the
adversary was impersonating the user a few times, his location will be
very different from the actual user's location. As the keys are
repetitively exchanged at different intervals of time the location
information is updated. As the user location behavior follows a
specific pattern repeatedly, the reputation score is increased. Same
set of keys are exchanged at different intervals and from different 
locations, where the locations follow a pattern. If the same set of
keys are exchanged from a location that does not follow the
established pattern, then the reputation score is reduced. Else it is
increased. When the reputation score reached a certain threshold the
keys are assumed to be genuine. 

\subsection*{Preliminaries}
\begin{itemize}
\item  Every mobile device is allocated a unique identity $D_1$
(either a phone number or IMSI number)
\item User $U_1$ registers with provider a $X_1$ using a device $W_1$
  with a unique identity $D_1$ 
\item If $W_1$ is directly connected to an authorized base station of
  provider $X_1$, then anyone who sends a message to identity $D_1$ is
  routed to $W_1$ and is received by user $U_1$.
%\item The routing layer within the cellular network is trusted
\end{itemize}




The step by step protocol is described as follows.

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1,c1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2,c2)S_2,c1 \\
 \textbf{3}.& \quad U_1 \rightarrow U_2: & & (c2)S_1 \\
 \textbf{4}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
 times} \\
 \textbf{5}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] User $U_1$ generates a self certifying key $P_1$ and
  signs the message consisting of location data $L_1$, time $t$,
  username $U_1$, user identity $D_1$ and challenge nonce $c1$. Here
  $L_1$ is the location data which might be the location of the cell
  tower combined with the GPS coordinates. $U_1$ sends the signed
  message $(L_1,t,U_1,D_1,c1)S_1$ and $P_1$ to $U_2$.

\item[\textbf{2.}] User $U_2$ generates a self certifying key $P_2$ and
  decrypts the message using the key $P_1$ sent in the message. $U_2$
  then signs the message consisting his location data $L_2$, time $t$,
  username $U_2$, user identity $D_2$ and reverse challenge nonce $c2$. User
  $U_2$ sends key $P_2$, challenge nonce $c1$ and signed message
  $(L_2,t,U_2,D_2,c2)S_2$ to $U_1$.

\item[\textbf{3.}] User $U_1$ decrypts message and sends the signed
  reverse challenge nonce $c2$ back to $U_2$. This completes the
  three-way handshake protocol.

\item[\textbf{4.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. We have to repeat the protocol $n$ times because
  the location information is untrusted. The rationale here is, an
  attacker might try to spoof the identity of $U_2$ once or twice, but
  repeatedly ($n$ times) masquerading the identity of $U_2$ is
  hard. So by repeating the protocol $n$ times, preferably from
  different locations, increases the chances of the user being $U_2$. 

\item[\textbf{5.}] If after $n$ times $(D_2, P_2)$ corresponds to
  $(L_1,L_2,t)$ then with high probability $U_1$ has established a
  secure connection with $U_2$.
\end{enumerate}


\subsubsection{Security Analysis}

In Step 1, $U_1$ generates a self certifying key $P_1$, signs the
message which contains the location data $L_1$, time $t$,
  username $U_1$, user identity $D_1$ and challenge nonce $c1$, and
  sends the message and $P_1$ to the other user $U_2$. As we discussed
  in the previous Section, the cellular network is one-way
  probabilistically secure. An adversary can spoof the cellphone
  number of $U_1$ and hijack the message. But if $U_2$ is present in
  the cellular network $U_2$ would also receive the message, since the
  message is being routed to $U_2$'s number. The adversary could
  create a fake base station within $U_2$'s vicinity and hijack the
  message. In this case $U_2$ would never receive the message. The
  adversary could continue the entire protocol with $U_1$. But this is
  a highly unlikely event due to the following reasons. i) the
  adversary has to be in the vicinity of $U_2$ at the exact moment
  when the message is sent to by $U_1$ to $U_2$. ii) during the entire
  course of the protocol the $U_2$'s cellphone has be switched off, so
  that $U_2$ can't join the network. If $U_2$ joins the network during
  the course of the protocol, $U_2$ would get an encrypted message
  from $U_1$ with no key to decrypt. This would alert $U_2$ about the
  MITM attack and $U_2$ could send a message to $U_1$ to abort the
  protocol. $U_1$ would receive messages from two different locations
  and because of this $U_1$ would abort the protocol. Another scenario
  is $U_2$ would switch on the phone during the repetitive location
  exchange step. This would again give $U_1$ different or
  inconsistent location information and $U_1$ would abort the protocol. 

In Step 2, $U_2$ first checks if the message sent by $U_1$ is
consistent. If not, it aborts the protocol. If the message is
consistent, $U_2$ generates its self
certifying keys and signs the message containing its location data
$L_2$, time $t$, username $U_2$, user identity $D_2$ and reverse
challenge nonce $c2$.  An adversary could spoof $U_1$'s message. So
$U_2$ does not have any guarantee that the message was indeed sent by
$U_1$. Only in step 5 of the protocol when the reputation score goes
above a certain threshold, $U_2$ would have established a secure key
exchange with $U_1$.

In Step 3, $U_1$ checks if the message sent by $U_2$ is consistent. If
not, $U_1$ aborts the protocol. Else, $U_1$ will sign a reverse
challenge response $c_2$ and send it to $U_2$.

{\em Reputation score:} In Step 4, $U_1$ stores $(D_2, P_2)$ and its
corresponding location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. Similarly, $U_2$ stores the $(D_1, P_1)$ and its
  corresponding location information and time $(L_1, L_2)$. In this
  step, the keys are exchanged $n$ times. Each time if the location
  and time information are consistent then the reputation score is
  increased by 1. If the time to send or receive the message is
  greater than a certain time $T$, then the reputation score is reset
  to zero and Step 4 is started again. An adversary could spoof the
  location and time message by performing a MITM attack, but since the
  step is performed $n$ at different locations and time periods, the
  adversary would not be able to modify the message such that either
  $U_1$ or $U_2$ would always get consistent location and time
  information. Also, if the message is inconsistent $k$ times, then
  the protocol is aborted. When the reputation score
  passes $n$, then $U_1$ and $U_2$ have exchanged keys with high
  probability. 


\subsection{Two: Trusted location data}

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1,c1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2,c2)S_2,c1 \\
 \textbf{3}.& \quad U_1 \rightarrow U_2: & & (c2)S_1 \\
\end{align*}

In this protocol, the location data ($L_1,L_2,t)$ is from a trusted
source. The GPS chip within the mobile devices $W_1,W_2$ are trusted
and the cell tower information obtained is also trusted. Hence the
protocol boils down to the three-way handshake protocol. 


\subsection{Three: Trusted point of sale device}

\subsection*{Assumptions}
\begin{itemize}
\item Point of sale devices are trusted. 
\item Point of sale devices have the ability to sign a message and
  transmit the message securely to the device $W_1$ of the user $U_1$.
\end{itemize}

\subsubsection{Protocol}

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow G: & & P_1,L_1,t,U_1,D_1  \\
 \textbf{2}.& \quad G \rightarrow U_1: & & G_P, (P_1,L_1,t,U_1,D_1)G_S \\
 \textbf{3}.& \quad U_1 \rightarrow C: & & P_1, (G_P,(P_1,L_1,t,U_1,D_1)G_S)S_1 \\
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] $U_1$ sends the message $P_1,L_1,t,U_1,D_1$ to a
  point of sale device $G$. 

\item[\textbf{2.}] A point of sale device can be a NFC
  device or other device which is capable to signing a message. The
  point of sale device $G$ signs the message $(P_1,L_1,t,U_1,D_1)G_S$
  and along with $G_P$ (public key) sends it back to $U_1$.

\item[\textbf{3.}] Now $U_1$ signs the message it received from $G$,

  ($P_1$,$L_1$,$t$,$U_1$,$D_1$)$G_S$)$S_1$ and sends it to the central
  authority $C$ along with $P_1$. Since $G$ is trusted (has trusted
  credentials), $C$ is certain that the message is signed by $G$ and
  that $U_1$ was indeed present at the point of sale location. The
  point of sale device could also have a fingerprint reader (or any
  biometric device) to authenticate user's identity and the biometric
  data can also be part of the signed message from $G$ to $U_1$. 
\end{enumerate}



==> Eurosys'16/Old Draft/relatedWork.tex <==
\section{Related work}

% physical encounter,
% Short Authentic Strings (SAS)
% count no of participants

Closely related work by Farb, Lin, Kim, McCune and Perrig \cite{safeslinger}, provides a system, 
named SafeSlinger, that leverages physical encounter to establish digital trust that is exchange 
keys with one another. Our system on the other hand does not require any kind of physical encounter 
with the person the user wants to exchange information to. However, SafeSlinger does allow establishing
digital trust by having a common acquaintance to facilitate a mutual introduction. 
In addition to this SafeSlinger \cite{safeslinger} asks the users to compare a 3-word phrase(encoded 24-bit hash value)
for verification and to minimize attacks. Groupthink \cite{groupthink} like SafeSlinger \cite{safeslinger} requires 
users to count the number of participants and requires users to verify Short Authentic Strings (SAS)
Secure mobile identities, like Safeslinger \cite{safeslinger}, does all the cryptographic steps in the background; but in DSMI, 
the user only enters the number of the user similar to what they do while sending a traditional SMS or MMS. Secure mobile identities
protocol requires physical proximity only in case of bluetooth exchange of messages and/or trusted location.

%multi-path

Secure location sharing system(SLS) by Adams and Lee \cite{sls}, uses similar approach as DSMI in a way
that they use multi-path approach for exchanging keys. Unlike Secure mobile identities, SLS requires the users have previously communicated
via some other channel and that channel will be used for verification. For further verification(someone other than the intended user
is using the channel) the user generates a secret question which has to be answered correctly by the intended user.

%server + visual encounter

DSMILE \cite{DSMILE} establishes trust between individuals who shared an encounter and they must provide a proof of that encounter.
The user broadcasts the encounter key to other devices within its communication range and then uploads a cryptographically secure hash
of they key along with a message encrypted by the encounter key to a server. The intended users claim the encounter by looking up
the hash of the key at the server.
Meetup \cite{meetup} similar to DSMILE \cite{DSMILE}, requires a visual authentication scheme which is a digital certificate signed by a 
trusted authority but they have to be at the encounter site. DSMI does not require a server and a visual authentication.

% public authentication

PGP Key signing parties \cite{keySigningParty} use people to verify that the public key is authentic. The larger the number of verification,
the more authentic the key is which is similar to our scoring mechanism except that DSMI uses location and path for scoring while PGP Key signing 
parties uses manual user authentication.

% a hub to pass info

GAnGS \cite{GANGS} exchanges group members' public keys such that each group member obtains the authentic public key of every member. 
It involves three phases: collection, distribution and identification. GAnGS need an untrusted projector or a phone as a hub to pass
information. This is too cumbersome to use because of so many operations to perform by a user.
SPATE \cite{SPATE} relies on visual channels and physical interactions. Like GAnGS \cite{GANGS}, SPATE requires a number of steps, 
visual hash function verification, leader selection, giving away personal information to bystanders. 

There is a proliferation of WiFi gadgets and sensors that do not have to protect against MITM attacks as the key exchange messages are 
not authenticated in any wayas it require devices to support an out-of-band communication channel. \cite{gollakota2011secure} presents 
tamper-evident pairing (TEP), a protocol that provides simple, secure WiFi pairing and protects against MITM attacks without an out-of-band
channel. DSMI is only built for phones or for devices capable of sending an SMS.


==> Eurosys'16/Old Draft/threat.tex <==
\section{Problem definition and threat model}

In this section we give the problem definition and threat model of the system and also
present an overview of the security properties. 

\subsection{Problem definition}

The current
state of security in the mobile ecosystem is either broken or have
severe vulnerabilities. We want to have a very secure and reliable communicating channel. 
We want to be absolutely certain that we are communicating only with the desired person and not to an intruder and that the conversation is not being intercepted by an imposter. This security and reliability is absolutely vital when 
two users or a user and the system wants to reveal their secret and/or sensitive information such as 
PIN codes or credit card numbers etc; without which data like this can fall in wrong hands and can be misused. In this age of technology; where people are always looking for ways to minimize time; they need a way to communicate securely in ways other than do it in person.
The problem we are trying to address is the following. 

{\em User $U_1$ with a mobile device $D_1$ wants to securely
interact with another user $U_2$ with a mobile device $D_2$ or any
central authority $C$, through an untrusted communication channel.}

When we say securely interact or communicate we mean that we have information secrecy;
 the information is revealed only to the intended user. 
We will first start with the assumptions and goals of the systems and then move
on to the threat model. 


\subsection{Assumptions}
Our protocol requires that the users have a smartphone. First, we assume that the users know how to use a smartphone. We also assume that the user can read and understand the instructions in English and that the user wants security and does not deliberately disclose private information. As our protocol requires frequent SMS sending and receiving; we assume that the user has enough credit in his account for sending text messages. With respect to our Secure Mobile Identities protocol the basic assumptions of the system are as follows.
\begin{itemize}
\item {\em The cellular service is trusted}. We assume that the cellular service on top of which
DSMI is built is trusted. When a mobile device authenticates itself with a cellular base station,
we assume that the IMSI number, Ki (key) is secure and nobody can steal the identity
of the device.
\item {\em SMS is always delivered}. We assume that the messages we send are delivered to the 
	person intended and it does not get lost once the device is on the network is authenticated. 
	For example, Alice and Bob are exchanging keys and
	Alice has authenticated Bob and sends a verification message to Bob which also includes 
	information for her authentication. This messages fails to get delivered. In this case Alice's
	records would have Bob as the authenticated user but in Bob's records Alice isn't authenticated.
\item {\em The cellular service provider is trusted}. If the cellular service
  provider is malicious then he could intercept the transaction
  between the users, perform a DoS attack and render the protocol
  useless. Vulnerabilities can be inserted to the SIM card using OTA
  (Over-the-air) updates which would compromise any message or phone
  call on the phone. Since the possibility of a rouge service provider
  is a rare occurrence, we assume the service provider is trusted. 
\item {\em SMS is secure}. This assumption is based on our assumption of the
	cellular service provider being trusted. If the provider is not trusted and if 
	there	is an intruder who is keeping a tap of messages being exchanged then the verification
	step in our protocol becomes null and void. We assume that the SMS can only be sent and
	received by the	user who owns the SIM. For example, a malicious user may start a secure communication
	with Alice using the phone number of Bob. Alice thinks that she is talking to Bob because
	the number she is exchanging messages with is the same as Bob's.
\item {\em The mobile phone is trusted}. We make this assumption because if
  the phone is not trusted then PIN, secret keys and other secure
  information related to the user would be insecure. Since most of the
  cryptographic protocols rely on the user's key being secure, it is
  natural to assume that the phone is trusted and that the user's
  credentials on the phone are secure. This also means we assume that
  there are no rootkit attacks on the phone.
\item {\em The mobile phone is devoid of malware}. We assume that the software and
	hardware of the phone is not prone to attacks from a third party which can intercept
	the user's phone. This also includes the phone apps that can allow attacks like
	these.
\item {\em Error checking and aborting}. In case of errors or suspicions, users will restart the
	application. 
\end{itemize}


\subsection{Goals}

Our main goal is to allow two users to exchange sensitive information securely 
through insecure channels. The Secure Mobile Identities protocol aims to achieve the following
goals:
\begin{itemize}
	\item {\em Security}. We aim to provide a secure system that would not leak sensitive data
		that has to be communicated to the intended user.
	\item {\em Privacy}. Contact information, data and keys of a user are only available to the
		members of the interaction and remain hidden from intruders or malware.
	\item {\em Authenticity}. The users involved in the communication are authentic which means that
		the interaction is carried on by the intended users and no one else.
	\item {\em Reliability}. We aim to provide that reliability that the information being passed on
		is going to the right user under all circumstances. 
	\item {\em Usability}. We emphasize usability along with all our security properties.
	\item {\em Platform Independence}. Our system is not platform independent thus enabling interactions
		among smartphones of different manufactures.
\end{itemize}

Given the assumptions and goals, the threat model of the system can be described
as follows.

\subsection{Threat Model}

We are building a secure and trusted application over insecure and untrusted communication channel. This causes 
a threat to our security. Possible attacks to Secure mobile identities include:
\begin{itemize}
	\item {\em Man-in-the-Middle (MitM) attack}. If two users are communicating with each other an attacker
		can intercept their messages by controlling the wireless communication.
	\item {\em Message forgery}. It is also known as message spoofing. An attacker can deceive the user as to whom
		the real sender is. The user can share all the sensitive information to the attacker in this way.
	\item {\em Malicious user}. A fake user who initiates a communication link to another user.
	\item {\em Malicious server}. The server may be controlled by a malicious administrator. A compromised server
		can be a threat to our security.
	\item {\em Malicious app}. As our protocol is intended for a smartphone it is very likely that the user
		has a malicious app installed on the smartphone which is used for communication using Secure mobile identities
		protocol. That application may be able to read the private keys and/or read the messages.
	\item {\em Fake or compromised base station}. It is possible that an attacker has set up a fake base station
		that can intercept all the messages going on through it.
	
\end{itemize}

\subsection{Security guarantees}

Despite being exposed to various attacks, our protocol offers security guarantees. Our protocol
has uses multiple channels for its operation. If an attacker attacks one of the channels, for example
the server is compromised, the verification has to go through the SMS channel. It is very difficult for
an attacker to attack all three channels: bluetooth, server and SMS.
For protocols that rely on a back-hand server, it is possible that the server is controlled by a malacious
administrator. Our protocol removes the message in a matter of a few minutes from the server from
the time it gets uploaded. It does not 100\% success but it is better than leaving the information on
the server for longer time.



==> Eurosys'16/Old Draft/threat_model.tex <==
\section{Problem Setting}

In this section, we define the problem we set out to solve, discuss our assumptions, goals and also perform a review of the adversary we defend against and present attacks.

%\begin{comment}
%\subsection{Motivation}
%\label{sec:motiv}
%
%The fundamental limitation of the GSM security is the absence of an authentication scheme between subscriber and the Mobile Network Operator (MNO). This can be exploited by setting up an adversarial base station with appropriate hardware and software. We discuss two realistic threats against GSM security. 
%
%\textbf{\textbf{Connecting to an Adversarial BTS}}
%\begin{comment}
%%Do we need all of this?
%
%
%
%As part of a cellular network, a Base Transceiver Station (BTS) has equipment for the encryption and decryption of communication, spectrum filtering equipment, antennas and transceivers (TRX) to name a few. There are several situations in which the Mobile Station (MS) starts to look for a new BTS to connect to.
%\begin{itemize}
%\itemsep-0.23em 
%\item When the MS registers to the BTS of the network provider, the BTS sends a list containing the frequencies of nearby BTS stations belonging to the same MNO. Based on this information, the MS selects the BTS with the best signal strength. If none are found, it scans through standard frequencies to find an active BTS. To force the selection of a fake BTS, the attacker can exploit knowledge of the MS periodically measuring its connection strength with the nearest BTS. To ensure forced selection, the \textit{fake signal} is sent on the BTS frequency with the strongest signal. 
%
%\item The MS may find a BTS with a better signal. In this case the fake BTS sends signals on the frequency channel used by one of the BTSs which are near the MS. This is called \textit{forced BTS selection}. 
%
%\item The frequency channel used by MS to connect with its original BTS is jammed which leads the MS to search for a new BTS.
%\end{itemize}
%
%\textbf{\textbf{Man in the Middle (MITM) attack}}
%
%
%With the availability of software defined radios like USRP \cite{usrp}, sysmoBTS \cite{sysmobts}, Fairwaves \cite{fairwaves} and Opencell \cite{opencell} the attacks on the unsecure GSM network have become a reality. This has further been facilitated by the availability of OpenBTS \cite{openbts} and OpenBSC \cite{openbsc} like open source projects that help provide the software infrastructure to run a BTS. Meyer et al \cite{germany} show a MITM attack on Universal Mobile Telecommunications Systems (UMTS) by exploiting the lack of integrity protection in GSM base stations. Kostrzewa \cite{thesis} demonstrates exploit the weakness of A5/2 \cite{comp128} cipher to demonstrate MITM attack. 
%
%Two kinds of MITM attack can be employed with an adversarial BTS, henceforth referred to as the \textit{fake BTS}. In the first phase of both, the MS is tricked to connect to the fake BTS. 
%\begin{itemize}
%\itemsep-0.23em 
%\item In the first case, once the MS decides to choose a fake BTS, it sends its International Mobile Subscriber Identity (IMSI) to the fake BTS. The fake BTS then sends a fake authentication request containing a forged randomly generated number, RAND. The MS calculates the Signed Response (SRES) by encrypting RAND with A3 algorithm using the Root Key, $K_i$. The fake BTS authenticates the MS regardless of the SRES value received and then uses A5/0 for ciphering. It can now read all of the outgoing traffic from the MS and then send it over IP to cover the ongoing attack. The incoming traffic will be saved by the MNO as voice mails and delayed text messages.
%
%\item The second kind of attack is complex and requires decrypting traffic. This attack has been demonstrated in \cite{germany} and requires an alternate phone to connect to, henceforth reffered to as a \textit{fake phone}. After the MS has been lured to connect to the fake BTS, the attacker forwards the IMSI received to the fake phone. The attacker initiates authentication of the fake phone with a real BTS. The RAND received by the fake phone for the IMSI is sent back via the fake BTS to the MS. The MS computes SRES and returns it to the fake phone via the fake BTS. The fake BTS orders the MS to start the A5/2 cipher encryption procedure. The attacker uses known ciphertext attack \cite{kca} to find the session key, $K_c$. When obtained, it is sent to the fake phone which now has both IMSI and $K_c$ and can finish authentication with the real MNO. The attacker sends back SRES. When the network requests encryption using A5/1, the response can be sent by the adversary since it already knows the $K_c$. 
%\end{itemize}
%\end{comment}

\subsection{Problem Definition}

The basic primitive that we seek to accomplish is to securely exchange information between participating individuals, say $U_1$ and $U_2$, using a partially trustworthy communication channel achieving information secrecy (only the intended entities receive the information) and device-verifiable association of data to another honest device (device knows the information that is associated with a specific honest device). We define secure communication along the lines of Semantic Security \cite{goldreich2004foundations} where knowledge of the ciphertext (and length) of some unknown message does not reveal any additional information on the message that can be feasibly extracted. We define partial trustworthiness of a channel as a probability metric that proportionally provides confidence that the user is communicating with the party he \textit{intended}. We also define honesty as a primitive where the participating parties follow the protocol diligently, without any intention to deceive others.

When the exchange involves more than two people, the group exchange should produce the exact same security properties that would result from the pairwise exchange between all group members. Given such a secure exchange that includes a public key bound to a user, all subsequent mechanisms for authentic and secret communication can be implemented using well known protocols.

\subsection{Goals} 

The main goal of the DSMI protocol is to establish secure communication between participating parties. To enable such a system, we outline four properties desired from the protocol:
\begin{itemize}
\itemsep-0.23em 
\item \textbf{Robustness.} We wish to show that a combination of user ID, device ID and periodic and aperiodic interactions from diverse geographic locations and timestamps creates a unique identity. This identity is hard to forge without substantial expenditure for the adversary. Expenditure in this context includes cost of following the user and/or colluding with other adversaries to obtain additional information. 
\item \textbf{Ergonomic.} We wish to show that the protocol is minimally invasive and requires nominal user intervention.
\item \textbf{Scalablity.} We wish to show that the protocol scales with the number of participating users with minimum latency.
\item \textbf{Portability.} We wish to support interactions between smartphones of several manufacturers, running different operating systems. This promotes heterogeneity in platforms. 
\end{itemize}

\subsection{Assumptions}
Our protocol needs to assume certain user behaviour for successful execution. We assume users can operate a smartphone and follow simple instructions. We also assume that users have a natural desire for security and do not deliberately
disclose private information. Our underlying assumptions are:

\begin{itemize}
\itemsep-0.23em 

%\begin{comment}
%\item \textbf{Users possess \textit{similar} devices}. Users have devices that support the same physical method for exchanging information (e.g., our implementation requires SMS support and programmable software).
%
%\end{comment}

\item \textbf{SMS is delivered with high probability}. The Network Layer in a Cellular Network is unexposed. This makes it harder to compromise and hence messages sent are delivered to the intended recipient with high probability. 

\item \textbf{The adversaries do not collude with each other}. Adversarial action being carried out at two different locations at different timestamps are independent events. That is, their joint probability equals the product of their individual probabilities : $P(\cap_{i=1}^{n} A_i)=\prod_{i=1}^{n} P(A_i)$, for independent events $A_i$, $i \in [1,n]$.

\item \textbf{A user does not deliberately disclose private information}. We assume that the probability of both Sybil attacks \cite{douceur2002sybil} and internal attacks are minimal. 

\item \textbf{The cellular service provider and mobile device is trusted}. Fraudulent cellular service providers could intercept interaction between users or perform a Denial of Service (DoS). However, the probability of a rogue service provider is low. Such providers could insert vulnerabilities into the SIM card or mobile applications using over-the-air (OTA) updates. We also assume that there are no rootkit attacks on the phone and it is devoid of malware.

\item \textbf{Diligent error checking and aborting}. In case of an error or suspicion, users will abort the protocol.

\end{itemize}

DSMI is not limited to only smartphone users. However, we focus on participants who use their smartphones frequently since smartphones are easy to use, are readily available, and are also easy to design applications for. Additionally, the ability to access multiple channels in smartphones helps reduce the load on the cellular network, which will be explained in \S 5.1.

\begin{comment}
\subsection{Initial Authentication Procedure} 

To better understand the protocol, we need to first understand the functioning of authentication in cellular networks. The following are some important steps that are required for the Mobile Station (MS) to connect to the cellular network through the Base Transceiver Station (BTS).

\begin{enumerate}
\item On verification of the unique International Mobile Subscriber Identity (IMSI), the authentication request of a MS is forwarded to the Authentication Center (AuC). The AuC looks for the Root Key, $K_i$ associated with a given IMSI and generates a 128 bit random value (RAND). 
\item Along with $K_i$, RAND is used as input for the A3 and A8 encryption algorithms \cite{comp128}. The outputs are the 32-bit Signed Response (SRES) and the 64-bit Session Key $K_c$ respectively. 
\item The MS calculates its own SRES using RAND, $K_i$ and the A3 encryption algorithm. It also calculates $K_c$ using the RAND received from Base Station Controller (BSC), and $K_i$. 
\item The MS sends back to the network its SRES.
\item The network compares its own SRES with the one obtained from the MS and authenticates the MS on matching. 
\item GSM ciphering is done with the help of the A5 encryption algorithm. There are four variants of A5 in GSM:
\begin{itemize}
\item{A5/0: No ciphering.}
\item{A5/1: Strong ciphering, used in North America and Europe.}
\item{A5/2: Weak ciphering, used in other parts of the world.}
\item{A5/3: Strongest ciphering with open design \cite{kasumi}.}

\end{itemize}
\end{enumerate}
\end{comment}

\subsection{Adversary Model}

We consider that a user can be in the presence of a Dolev-Yao style network adversary \cite{dolev} at a particular location, with probability $P$. This adversary wants to break the properties as described in the problem definition. An additional combinatorial optimization constraint on the adversary coerces it to assimilate maximum information whilst minimizing cost, similar to the one dimensional knapsack problem. Cost or \textit{Bootstrapping Cost} is associated with setting up equipment at each location and is large. Thus, we assume that the adversary will neither follow the user to more than $k$ locations, nor will follow any user continuously. With their devices, adversaries can overhear, intercept, and inject any wireless communication. We also consider DoS attacks by the adversary to be out of scope, as we assume that the diligent users re-start the protocol as needed. 

\subsection{Attacks}

Secure information exchange is a challenging problem. The attacks DSMI is resilient towards include:

\begin{itemize}
\itemsep-0.23em 
\item \textbf{Fake or compromised base station:} The adversary can create a fake BTS to monitor and alter any or all communication relayed through it. This is a form of a MITM attack, resulting in message spoofing and signal jamming \cite{stхhlberg2000radio}.


%\begin{comment}
%\item \textbf{Malicious server:} For protocols that rely on a back-end server, the server may be controlled by a malicious administrator or become compromised.
%
%\item \textbf{Information leakage after protocol abort:} The adversary may be able to cause the protocol to abort and trigger leakage of private information.
%\end{comment}

\item \textbf{Collision attack on low-entropy hash:} Low-entropy hash values are vulnerable to efficient attacks unless precautions are taken.
	
\end{itemize}




==> Eurosys'16/Old Draft/trusted_locations.tex <==
\section{Trusted location based key exchange}

\subsection{Trusted location data}

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1,c1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2,c2)S_2,c1 \\
 \textbf{3}.& \quad U_1 \rightarrow U_2: & & (c2)S_1 \\
\end{align*}

In this protocol, the location data ($L_1,L_2,t)$ is from a trusted
source. The GPS chip within the mobile devices $W_1,W_2$ are trusted
and the cell tower information obtained is also trusted. Hence the
protocol boils down to the three-way handshake protocol. 


\subsection{Trusted point of sale device}

\subsection*{Assumptions}
\begin{itemize}
\item Point of sale devices are trusted. 
\item Point of sale devices have the ability to sign a message and
  transmit the message securely to the device $W_1$ of the user $U_1$.
\end{itemize}

\subsubsection{Protocol}

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow G: & & P_1,L_1,t,U_1,D_1  \\
 \textbf{2}.& \quad G \rightarrow U_1: & & G_P, (P_1,L_1,t,U_1,D_1)G_S \\
 \textbf{3}.& \quad U_1 \rightarrow C: & & P_1, (G_P,(P_1,L_1,t,U_1,D_1)G_S)S_1 \\
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] $U_1$ sends the message $P_1,L_1,t,U_1,D_1$ to a
  point of sale device $G$. 

\item[\textbf{2.}] A point of sale device can be a NFC
  device or other device which is capable to signing a message. The
  point of sale device $G$ signs the message $(P_1,L_1,t,U_1,D_1)G_S$
  and along with $G_P$ (public key) sends it back to $U_1$.

\item[\textbf{3.}] Now $U_1$ signs the message it received from $G$,

  ($P_1$,$L_1$,$t$,$U_1$,$D_1$)$G_S$)$S_1$ and sends it to the central
  authority $C$ along with $P_1$. Since $G$ is trusted (has trusted
  credentials), $C$ is certain that the message is signed by $G$ and
  that $U_1$ was indeed present at the point of sale location. The
  point of sale device could also have a fingerprint reader (or any
  biometric device) to authenticate user's identity and the biometric
  data can also be part of the signed message from $G$ to $U_1$. 
\end{enumerate}



==> NSDI/dump/6-Security.tex <==
\section{Security Analysis}
\label{security}

In this section, we address the attacks and challenges discussed in \S \ref{probsettings}, specifically:



%\subsection{Addressing Threats}
%\begin{itemize}
\itemsep-0.23em 
{\bf Malicious Adversaries:} As discussed earlier, adversaries can create a fBTS. Once the honest device connects to it, the adversary negotiates to the lowest level of encryption supported by the device and relays inbound and outbound calls, as well as IP traffic sent on the data channel. In theory, these adversaries can be detected by the other BTS of the network provider, but there is no documented responses against such temporary rogue towers. This attack is heavily dependent on the probability $P$ of a user being in the vicinity of the fBTS. However, this attack is alleviated by moving outside the transmission zone of the fBTS. The probability that the user moves to $k$ locations and is in the vicinity of the fBTS in all of them is $P^k$, which is very small. Hence the probability of failure of the attack, or probability of protocol success is $1-P^k$. By ensuring mobility, the success of this attack decreases exponentially. If communication is carried out across multiple channels, the probability of protocol success across multiple channels is $\prod_{i=1}^{3} (1 - P^{k_i})$ ; $\sum_{i=1}^3 k_i \leq k$. This is a measure in the worst-case scenario as the event in which more than a single channel is compromised is very rare. Setting the predefined threshold large enough provides a degree of flexibility towards partially diligent users.  

{\bf Signal Jamming:} Another variant of the attack is where such an adversary jams communication of the device connected to the fBTS and attempts to join interactions in its place. However, the exchange of random parameters $a,b$ at the beginning of every epoch ensure that subsequent interactions in the epoch are consistent (as explained in \S4). On detecting an inconsistent interaction, a diligent participant aborts the protocol and restarts it at a different location. 

If an attacker spoofs the identity of a victim \textit{and} remains part of a consistent interaction by obtaining values $a,b$ at the beginning of an epoch, another improbable event, the other user will receive messages from two \textit{distinct} identities (as part of the PKI) once the victim is no longer in the vicinity of the fBTS. We wish to reiterate that as long as the users are mobile and diligent, these attacks fail. In the absence of mobility, there is a significant increase in probability of successful jamming and other failure events.



{\bf DoS:} As discussed in \S \ref{attacks}, adversarial DoS attacks are mitigated by moving out the range of the fBTS. Our honest MNO assumption invalidates any operator-based MitM and DoS attacks. Solutions such as MAC level disambigution of the message channel \cite{ghaderi2012connection} and content-based vertical handoff ensure that the cellular network is not overprovisioned due to scaling.

{\bf Low-Entropy Hash:} Modern smartphone processors run at clockspeeds upto 2 GHz, giving them fairly strong computational ability. By selecting an appropriately large key-length, we can ensure that the probability of a collision is significantly reduced. 

{\bf Key-pair generation:} The increasing processing capabilities of modern smartphones and the various entropy sources such as cameras and accelerometers \cite{voris2011accelerometers, marghescu2014cryptographic, yuzuguzel2015shakeme} available to it ensure that key-pairs can be frequently generated without substantial strain. The generated key-pair is stored safely as we assume that the user does not disclose any sensitive information.

%\end{itemize}


==> NSDI/dump/7-Additional.tex <==
\section{Discussion}
\label{discussion}

We now discuss the rationale behind our design.
\vspace{-2mm}
\subsection{Trusted Location Distrbution}
\label{tld}

309 retailers have an estimated 7623 stores in New York City \cite{survey}. With a size of 304.6 sq. miles, the average store density is 25 stores/sq. mile. The zip code 10003 (Greenwich Village) of size 0.58 sq. miles has 164 retail stores, resulting in value of 282 stores/sq.mile in this area. This is 11 times the city-wide average and is attributed to the high population density of Manhattan and it being a popular tourist destination. The recent proliferation of NFC based payment has resulted in a large number of stores adapting contact-less payment solutions. Based on analysis, close to 80\% of the chosen stores in New York have use such solutions and are hence are location verified \cite{mastercard}. 
%That is to say, 8 in 10 stores one would visit is a trusted location.

\vspace{-2mm}
\subsection{Smartphone Proliferation}
\label{proliferation}

Based on a Pew survey, 64 \% of all US adults now have smartphones. However, among the population of mobile phone owners (91 \% of US adults), the smartphone penetration number is now 61 \%. Apple iPhone sales alone exceeded 40 million in the US for the 2014 financial year. 19\% of Americans rely to some degree on a smartphone for accessing online services and information-either because they lack broadband at home, or because they have few options for online access other than their cell phone.
\vspace{-2mm}
\subsection{Economic Implications}
\label{economics}

Another Pew survey suggests cell owners between the ages of 18 and 24 exchange an average of 109.5 messages on a normal day which works out to more than 3,200 texts per month. The typical or median cell owner in this age group sends or receives 50 messages per day (or 1500 messages per month). However, over 100 service providers in the United States provide unlimited messaging as part of their monthly plans \cite{whistleout}. This greatly alleviates the cost associated with the large number of messages exchanged between users of SMI.
\vspace{-2mm}
\subsection{Human Mobility}
\label{mobility}

The average moderately active person take aound 7500 steps per day. Doing the math; the average person with the average stride walks 3.76 miles a day. To support this claim, New York was voted the most active state in the US, according to a recent study from Fitbit, where a resident takes an average of 10000 steps per day.
%\subsection{QoS In Cellular Networks}
%
%A variety of factors affect the time taken to successfully deliver a message. Delays are caused due to:
%\vspace{-2mm}
%\begin{itemize}[leftmargin=-.01in]
%\itemsep-0.23em
%\item Low quality cellular devices.
%\item Delay in allocation of adequate network infrastructure.
%\item Lack of fairness from service providers.
%\item Limited coverage and network capacity.
%\item Poor government monitoring on standards.
%\item Environmental materials and current location i.e. distance from the cellular towers.
%\end{itemize}
%\vspace{-2mm} 
%Any combination of the afforementioned reasons could result in a deviation from optimal delivery time of the messages required for the SMI protocol. For example, the difference in message delivery time between AT$\&$T in New York City and Etisalat at Abu Dhabi may arise due differences in city demographics, geographics and infrastructure. This could cause advancements or delays towards the time required to build sufficient reputation. 










==> Old Draft/Acknowledgements.tex <==
\section{Acknowledgments}
This material is based on the work partially supported by
 funding from the Center of 
Technology and Economic Development (CTED), NYU Abu Dhabi. We thank CTED and NYUAD for their support.

==> Old Draft/Applications.tex <==
\section{Applications}

There can be various applications that can be built on top of Secure Mobile
Identities protocol. DSMI promises security and reliability along with usability.
DSMI does not involve any user involvement and the simplicity of DSMI makes
it favorable to be adapted in existing as well as new applications.
We present here some of the ideas of the applications which we think can be built
on top of DSMI protocol seamlessly. 

\subsection{Secure Messaging Application}
We have implemented secure SMS for Android. Secure information; text or pictures or
documents; can be encrypted using shared public key using DSMI and the information
exchanged is authenticated by DSMI as well. Popular applications like Whatsapp\cite{whatsapp}, 
Viber\cite{viber}, 
and BBM\cite{bbm} etc can be extended to include another security layer(DSMI) without changing
their signature interface.

Photo sharing is popular these days (snapchat~\cite{snapchat}, instagram~\cite{instagram}), 
the users needs privacy for the pictures pictures they
share. Building an application that sends private pictures to a closed set of audience with
no intrusion is possible using DSMI.


\subsection{Secure Cash}
We can leverage DSMI to build an app that requires the most security. We can build a virtual
cash system on top of DSMI which can be used as the security layer. The bank is a trusted 
party whose secure cash app would allow its customers to perform secure digital transactions.
The secure cash is the implementation of the process of sending and receiving a bank transaction 
through an app, removing the requirements of a cash register. 
Electronic transactions can be done with or without the presence of a designated point of sale.
Alice wants to buy a dress, from a store which is registered with her bank and has a trusted 
location device, using her secure cash app. She opens the application and scans/takes a picture 
of the bar-code of the dress and sends it to her bank using the pre-installed trusted location device 
in the shop. Alice's phone performs the three-way handshake using the trusted location device at the
shop with the bank. The bank authenticates the location and evaluates the trust level of Alice and 
sends a receipt to the shop indicating that the transaction has been taken place.

Another important scenario using secure cash can be the cash receipt system and it can be useful in places
where banks/ATM/credit card transactions are not widely accessible. Alice who wants to transfer money to
Bob's account; uses the secure cash application to do so; signs a cheque and sends it to Bob after 
completing a secure key exchange handshake. Bob on receiving the cheque goes to the bank where it gets
scanned and receives the money.

\subsection{Safe and Secure Virtual Identity}
Documents like passport, SSN, driver's license, property documents etc are very sensitive and need to be
kept at a safe location at all times. Applications can be built on top of DSMI that can encrypt these files
and send them to the trusted intended party or user without physically sending the documents. Using DSMI 
would help the sending and the receiving party be sure that the document is actually received from the
actual owner and is received by the intended user.

\begin{comment}
\subsection{Secure SMS}

We have implemented secure SMS for Android as discussed in the Implementation section.
The two users exchange their keys using one of the paths: SMS, bluetooth or IP.
Alice and Bob wants to share some secret information with one another so they decided
to use the DSMI text message app. Alice enters the contact number of Bob and the app
performs the 3-way key exchange handshake in the background after Alice choose one of
the three methods she wants the key exchange to take place through. Then she types the
top secret information in plain text and hit send. The app encrypts the message in plain
text and sends it to Bob. The DSMI application decrypts the message and shows the message
to Bob in plain text. This can be done for instant messaging applications
as well. Existing applications for example WhatsApp \cite{whatsapp},
Viber \cite{viber} and Line \cite{line} can make use of DSMI to perform the same functionality and their signature
interface but they can add additional security without having to change their popular
application.

\subsection{Secure Photo exchange}

Sharing pictures online is the new trend. Every user who has a phone with a camera not
only takes a picture of every single moment of his/her life, they want to share these pictures within
their social circle. As photo sharing became popular, it became apparent that the user
needs privacy for those personal pictures as well. One such popular application: Snapchat \cite{snapchat} enables
its users to share their picture with their friends for a set amount of time and then the picture
is removed. While this allows a certain degree of security this isn't completely devoid of any kind
of intruder attacks. Instagram \cite{instagram} is also one of the leading photo sharing application these days. Both 
these applications can use DSMI protocol to make their system reliable and secure. Similarly, one can develop
an application that can encrypt the photos only the user wants them to encrypt-doing so we can reduce the overhead of
an application for encryption and decryption.

\subsection{Secure cash}

We can leverage DSMI to build an app that requires the most security. We can create 
a cash receipt system using DSMI. The system would require a bank account that would 
allow transactions. We can create an application for a user to sign the bank approvals
and authorize another user to cash those approvals. The application can make use of
DSMI as a security layer. The security layer is a much needed feature in this application.
Nobody wants an intruder to eavesdrop in transactions as critical and sensitive as this.
After completing a secure key exchange handshake, Alice who wants to authorize Bob
to get cash from a bank; digitally allows Bob to do so by signing a cheque using secure
cash. The bank is a trusted party whose secure cash app would allow its customers to perform
secure digitally transactions.

\subsection{Secure File exchange}

In the present era of technology, it seems redundant to have a physical copy of
all the important and sensitive documents. One needs to securely place them and in hour
of need take those documents out of the secure area and send them securely to the
trusted intended recipient. Documents like a user's passport, social security number,
property documents etc. Applications can be built on DSMI and can encrypt the files
and send them to the trusted intended party or user. Using DSMI would help the sending 
and the receiving party be sure that the document is actually received from the
actual owner and is received by the intended user.
\end{comment}

==> Old Draft/Conclusion.tex <==
\section{Conclusion}

People share information all the time using their cell phones. Phone carriers claim
that their system is protected and all the data sent and received by a user is
encrypted. However, this is not the case. A lot of times users fall a victim of
various attacks such as snooping, eavesdropping, jamming, stealing the identity etc.
To fill in this gap of security we designed Secure Mobile Identities, a protocol that
uses various locations and multiple paths to develop a notion of trust. The
user uses DSMI repeatedly through various locations and through different paths to
earn trust score. The trust score is directly proportional to the user's authentication.

We have implemented and evaluated DSMI on an android platform. It is an easy-to-use app
and is similar to that of a native SMS android app to enhance usability of DSMI.
DSMI can be extended to share pictures, documents and it can be used for bank transactions
as well. Using DSMI can help users communicate securely and with a confidence that no
other person in the middle and they are communicating to the person they intend to communicate with.


==> Old Draft/Evaluation.tex <==
\section{Evaluation}

To evaluate the usability of Secure Mobile Identities usability
we conducted trial runs and tests to gather stats. In this section
we will explain the procedure and the results and observations on
the basis of the tests conducted.

\subsection{Procedure}
We wanted to test how long it takes for a user to complete the key
exchange handshake as it involves exchanging multiple text messaging.
The results depends on the network used for sure. Our tests were
conducted in Abu Dhabi, UAE using Etisalat \cite{etisalat} as our 
telecommunications services provider. 
We used java's function for time calculation to get time in nanoseconds.
We recorded the current time in nanoseconds. We used two ways to get the time: the phone
is linked with a PC via bluetooth and both phones signals the PC to record the
time (to get time of one machine) and for more accuracy we used the phones
to record their times themselves (to account for any delays caused while
transmitting the messages via bluetooth).
Time 1a is the time required to start the transaction by phone A and when phone
B replies back with its own data. Time 1b is the time recorded from the moment
phone B sends back its own data until it receives the challenge reply by A.
Both these times: Time 1a and Time 2a are taken by the PC connected via
bluetooth to both phones.
Time 1b and 2b is the same time as Time 1a and 2a, the difference is the
way the time is recorded. 1b and 2b are recorded on phone A and phone B
themselves.
Time a is the time required by phone A to send data to phone B. It is calculated
by getting the time in nanoseconds when user using phone A clicks send; phone
A sends an alert to PC to record the current time via bluetooth. Phone B when
receives the message sends an alert to PC to record the current time.
\\Time b is the time recorded when phone B sends its own data to A and the time
A receives it. Time c is the time required when A sends the challenge reply to
phone B and B receives it.

\subsection{Observations and Results}

We used a PC for recording the time when the phone sends a signal using bluetooth. 
We also used phones themselves to record the time. Using another device, in our case
the PC, for recording time can cause delays and by using two different devices for
recording time can create the difference in time. Figure \ref{timeDif} shows the difference
in times. Time 1 is the time taken by phone A to send meta-data to phone B 
and phone B replies back with encrypted challenge reply and its own metadata to phone A.
Time 2 is the time taken by phone B to send the encrypted challenge reply and its 
own metadata to phone A and phone A replies with the challenge reply. This figure shows that
the difference between the two is not very significant and we can use the average number to 
add into the results for an approximate time calculation.


\begin{figure}[htb]
    \centering
		\subfigure[{\smallTime difference for time 1: time taken by phone A to send meta-data to phone B and gets back a response}]
		{
				\includegraphics[width=0.45\columnwidth]
				{C:/Users/fa45/Dropbox/secmobid/tex/analysis/DiffTime1.jpg}
    }
		\subfigure[{\small Time difference for time 2: time taken by phone B to send the encrypted challenge reply and its 
own metadata to phone A and gets back a response}]
		{
				\includegraphics[width=0.45\columnwidth]
				{C:/Users/fa45/Dropbox/secmobid/tex/analysis/DiffTime2.jpg}
        
		}
		\caption{The time difference recorded}
		\label{timeDif}
\end{figure}


\\We measure the total amount of time needed to complete the 3-way key exchange
handshake by all paths.
ToDo: include data and bluetooth as well
\\Figure \ref{ttime} shows the timing analysis. According to this figure, for the
SMS the maximum time taken in all the tests was approximately 120seconds and the
minimum time taken was approximately 70seconds. The average is approximately 95seconds.
This means on average a user has to wait for up to 95seconds to start the exchanging
the messages with the intended user.

\begin{figure}[htb]
    \center{\includegraphics[width=2in]
        {C:/Users/fa45/Dropbox/secmobid/tex/analysis/totalTimeTaken.jpg}}
    \caption{\label{ttime} Total time taken for 3-way key exchange}
\end{figure}

\\Figure \ref{timeabc} shows which part of the 3-way protocol takes the most time.
Time a is the time required by phone A to send data to phone B. Time b is the time recorded when phone B sends its own data to A and the time
A receives it. Time c is the time required when A sends the challenge reply to
phone B and B receives it. The figure clearly shows that time C requires the least
amount of time whereas time a requires the most.


\begin{figure}[htb]
    \center{\includegraphics[width=2in]
        {C:/Users/fa45/Dropbox/secmobid/tex/analysis/TIMEabc.jpg}}
    \caption{\label{timeabc} Time a, Time b and Time c}
\end{figure}















==> Old Draft/SMI.tex <==
\section{DSMI protocol overview}

The main idea of Secure Mobile Identities is to enable users to exchange keys for
a secure one-to-one session. We want to implement a highly secure protocol
over highly insecure channels. DSMI uses various paths for building trust amongst 
the users. The application uses the cell towers and the GPS coordinates to 
gather the location data. It also uses various forms of trusted location services.
DSMI is a repetitive, spatiotemporal protocol that uses time, location and paths to
develop digital trust. 

\subsection{Overall design} 

Secure Mobile Identities uses the solo SMS path/single path, the IP-SMS path 
and the Bluetooth-SMS path. So there are 3 ways in which
a user can communicate: via SMS, via Bluetooth and via IP.
All these paths receive the verification of the
key exchange handshake via SMS. Hence it is our assumption that the SMS will 
always be delivered to the user. The single path relies only on the SMS. 

\\The user opens the application and enter the number of the intended user. This is all
what a user has to do in order to initiate the key-exchange process. 
Secure Mobile Identities uses a 3-way key exchange handshake, like most of the 
network security protocols. In single path all these 3 messages are transmitted via
SMS. In multi-path; the data is exchanged using IP or Bluetooth but the verification
which is the challenge reply is always done via SMS. We have modified the 3-way handshake
for the multi-path.

\\For a 3-way handshake,(1) user A sends A's public key, A's location, time, A's phone number
and a challenge to the user B. User B on receiving this message sends back (2) B's public
key, B's location, time, B's phone number, challenge and the reply to A's challenge.
User A verifies the challenge reply sent by the user B and if correct sends (3) the final
challenge reply to B. 

\\For a muti-path modified 3-way handshake,(1) user A sends A's public key, A's location, time, A's phone number
and a challenge to the user B via Bluetooth or IP channel. User B on receiving this message
sends back (2) B's public key, B's location, time, B's phone number and B's challenge to A via 
Bluetooth or IP channel "and" User B then sends  the reply to A's challenge via SMS path.
User A verifies the challenge reply sent by the user B and if correct sends (3) the final
challenge reply to B via SMS. 


\\DSMI maintains a table of the digital trust; as mentioned in section \ref{score}; using the 
user's location data, the time of exchanging keys and the path used. Location
plays a very vital role in DSMI. Location of the user is captured by a number of
ways which includes using cell towers and the GPS coordinates. For more reliable 
and trust worthy location data, DSMI uses various forms of getting trusted and
certifying location along with a time stamp. The location data gathered via
trusted location provider is considered the most authentic and trustworthy location
data. 

\\Each user performs the key exchange multiple times and each time the location and time of
user is recorded along with the path used to exchange the keys. Doing so, DSMI determines the
pattern the user is using for the interaction. 
Once the 3-way handshake is completed, the
score is increased on the basis if the location information obtained. If the location data 
obtained is from a trusted/authentic location provider such as trusted location provider; as discussed in section 
\ref{location} and \ref{score}; the score is increased more. As DSMI is the repetitive key exchange protocol; the user
exchanges keys multiple times along with the location and time. This information is stored and
on the basis of this information; the score is calculated. The score is maintained by DSMI to develop different
levels of trust. If an attacker has hacked the user's information, it is a very less probability
that the attacker is at the same location as the user. The user builds more trust i.e. more score
by following some kind of a pattern. Therefore, if the same set of keys are exchanged
from a location that does not follow the pattern; the level of trust and hence the score is
decreased. DSMI has established a certain threshold which when is achieved by the user; the keys
are assumed to be genuine. The score is calculated on the basis of the location pattern, it is
also set on the basis of different paths used by the user. A user sharing the same set of keys
from a set pattern of location across different paths of DSMI is also a variable that is set for calculating
the trust score. The variety of paths used and the set pattern followed by the user helps achieving
a high trust score.


\subsection{Spatiotemporal single and multi paths}

The single path in DSMI relies only on the SMS. It is a one-way probabilistically trusted
path. The assumption is that the user's phone is connected to the network which is
trusted. If the network that the phone is connected to is trusted then we can also assume
that there are no main-in-the-middle attacks in that path and our final assumption is that
there is no loss in the SMS i.e. SMS will always be delivered to the intended user. In a 
nutshell it can be said that SMS is the most secure, one-way, trusted path. By saying so
we believe that SMS once sent-will be delivered but we are not making any assumptions
that the user who is sending the SMS is the intended user; the user who's sending the
SMS can be an attacker.
DSMI uses multiple channels to exchange keys in a secure manner. Having multiple
channels for authentication allows the DSMI protocol to have added security. The assumption is that the attacker can compromise one channel
only-the probability to compromise both paths is extremely low. DSMI uses two such paths:
IP-SMS channel and Bluetooth-SMS channel. SMS channel in both cases is used for verification
or for the challenge reply in the key exchange handshake as discussed in section \ref{location}
. It should also
be noted that it is assumed that the verification SMS will always reach the intended user.
Users using different channels across different times and locations increase the trust level.


\subsection{Trusted or untrusted location}\label{location}

In DSMI, location plays a pivot role. Location data is gathered in a number of ways. Location data
is the key variable in evaluating reputation score. The user can have trusted location and the
user can have untrusted location. Users performing the key exchange using trusted location scores
more than the users performing the key exchange using untrusted location. A trusted location is
a certifying location signed by a trusted 3rd party. We describe the different ways of gathering data
as follows: 

\begin{itemize}

\item {\em GPS coordinates and cell towers}. The most
common way is through cellular tower and GPS coordinates. This is an unreliable and untrustworthy 
way to acquire the location information as any attacker can modify the GPS coordinates easily. Cell
towers maintains the location and this location information can be easily fetched.  

\item {\em Trusted 3rd party service} As the location gathered by GPS coordinates and cell towers
is not secure as it can easily be modified; we propose a secure, certifying location service. A 3rd
party service such as Google wallet \cite{googlewallet} can be used to fetch a signed location 
contract along with the timestamp. This service is not limited to Google wallet; a 3rd party can
deploy their own location tracking system which can enable a user to quickly sync the phone via
bluetooth to get the certifying and signed location. The location, timestamp can be used by any user
using a global public key. 

\item {\em Trusted IP} Another way of gathering location information is through the user's IP address.
IP address of every device is unique and it is theoretically possible, to determine the 
physical location of IP addresses. This is called Geolocation. Geolocation systems attempt to map IP 
addresses to geographic locations using large computer databases. As it is possible that the attacker
can hide behind a proxy, thus we need a trusted 3rd party wifi hotspot which works in essentially the
same way as described above but instead of using coordinates gives away a certifying IP address.

\end{itemize}

\\DSMI requires the users to perform this key exchange handshake a number of times for score
generation as discussed below. Performing this exchange across different locations at different
time would help increase the level of trust for that user.
 
\subsection{Repetitive key exchange and Reputation score}\label{score}

DSMI maintains a table of user information data including user's phone number,
user's public key, all the various locations the user performed the handshake and
the date and time of the handshake. DSMI requires the users to 
perform this key exchange handshake a number of times for score
generation. On the basis of this table; DSMI evaluates the digital
trust score against each user. Retaining these scores creates various levels of trust.
Each time a user use the same key from different or same location across various timings
and via a variety of paths used, the score of the user is increased. Getting a variety of
location information helps DSMI determine a pattern. If the location information deviates from
the set pattern, the score is affected accordingle. Some factors like
trusted location add more score than the usual, insecure location gathering techniques.
The score is deducted if the data gathered and stored in the table shows anomaly. If
a user's score reach a certain threshold, the key of that user is considered genuine. 
To reach that level of trust requires repetitive key exchange across different locations,
time and path.



==> Old Draft/SMI_with_trusted_location.tex <==
\section{DSMI with trusted location}

In this section we will discuss the DSMI protocol in detail using trusted location data gathered
through 3rd party services. We first explain the details of trusted location data.

\subsection{Trusted location based key exchange}

The location data gathered through GPS and cell tower is not trusted as explained the above section.
We need a secure and trusted location gathering mechanism. By a trusted location we mean a location that
can not be changed by an attacker and is signed by a trusted 3rd party. The location data gathered through
these trusted points of location gathering devices is considered the most authentic and a user having a trusted
location gains more score points. There can be a number of ways to achieve this. We present a few of those
techniques in this paper.

\\A trusted 3rd party installs some of these certifying location gathering devices in a few places for a user to sync
their device and gets a certifying location along with a time stamp. The location data is actually the location
of that device and as the user is in close proximity of that device; the location of the user is the same as that
of the device. Syncing can be done via bluetooth or any other technology. This is something very trivial to do
as Google already has deployed its Google wallet points at various location. A user can sync up with the
Google wallet point and get a certifying location.

\\Another way of gathering location data is through IP. As the public IP address of every device is unique and IP
addresses are assigned in the form of a tier system based on the geographical location. It is possible to gather
the location information through IP. Mapping IP addresses to a geographical location is known as Geolocation and is
described in \cite{taylor2012bringing}  and \cite{kovacs2002geolocation}. The idea is to have a trusted 3rd party
hotspot deployed at various location so that a user can sync the mobile to get a certifying IP location. The IP
location can further be processed as discussed above to break it down to geographical location. 


\subsubsection{Trusted location data}

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1,c1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2,c2)S_2,c1 \\
 \textbf{3}.& \quad U_1 \rightarrow U_2: & & (c2)S_1 \\
\end{align*}

In this protocol, the location data ($L_1,L_2,t)$ is from a trusted
source. The GPS chip within the mobile devices $W_1,W_2$ are trusted
and the cell tower information obtained is also trusted. Hence the
protocol boils down to the three-way handshake protocol. 


\subsubsection{Trusted point of sale device}

\subsubsection*{Assumptions}
\begin{itemize}
\item Point of sale devices are trusted. 
\item Point of sale devices have the ability to sign a message and
  transmit the message securely to the device $W_1$ of the user $U_1$.
\end{itemize}

\subsubsection*{Protocol}

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow G: & & P_1,L_1,t,U_1,D_1  \\
 \textbf{2}.& \quad G \rightarrow U_1: & & G_P, (P_1,L_1,t,U_1,D_1)G_S \\
 \textbf{3}.& \quad U_1 \rightarrow C: & & P_1, (G_P,(P_1,L_1,t,U_1,D_1)G_S)S_1 \\
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] $U_1$ sends the message $P_1,L_1,t,U_1,D_1$ to a
  point of sale device $G$. 

\item[\textbf{2.}] A point of sale device can be a NFC
  device or other device which is capable to signing a message. The
  point of sale device $G$ signs the message $(P_1,L_1,t,U_1,D_1)G_S$
  and along with $G_P$ (public key) sends it back to $U_1$.

\item[\textbf{3.}] Now $U_1$ signs the message it received from $G$,

  ($P_1$,$L_1$,$t$,$U_1$,$D_1$)$G_S$)$S_1$ and sends it to the central
  authority $C$ along with $P_1$. Since $G$ is trusted (has trusted
  credentials), $C$ is certain that the message is signed by $G$ and
  that $U_1$ was indeed present at the point of sale location. The
  point of sale device could also have a fingerprint reader (or any
  biometric device) to authenticate user's identity and the biometric
  data can also be part of the signed message from $G$ to $U_1$. 
\end{enumerate}



\subsection{SINGLE PATH SPATIO-TEMPORAL REPETITIVE KEY EXCHANGE}

It is the same as the described in the previous section except for the
addition of trusted location. We will now describe the same protocol
with added security.

\subsection*{Preliminaries}
\begin{itemize}
\item  Every mobile device is allocated a unique identity $D_1$
(either a phone number or IMSI number)
\item User $U_1$ registers with provider a $X_1$ using a device $W_1$
  with a unique identity $D_1$ 
\item If $W_1$ is directly connected to an authorized base station of
  provider $X_1$, then anyone who sends a message to identity $D_1$ is
  routed to $W_1$ and is received by user $U_1$.
\item The 3rd party location gathering device $W_2$ is trusted and the location
	data $D_2$ is genuine. 
%\item The routing layer within the cellular network is trusted
\end{itemize}


The step by step protocol is described as follows.

\begin{align*}

	\textbf{1}.& \quad W_2 \rightarrow U_1: & & (L_1)S_G  \\
	\textbf{2}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1,c1)S_1  \\
	\textbf{3}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2,c2)S_2,c1 \\
	\textbf{4}.& \quad U_1 \rightarrow U_2: & & (c2)S_1 \\
	\textbf{5}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
								times} \\
 \textbf{6}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}

\begin{enumerate}

\item[\textbf{1.}] User $U_1$ syncs with a trusted location device $W_2$ which gives
	$U_1$ a certifying location $L_1$. $W_2$ sends the signed message $(L_1)S_G$ to $U_1$.

\item[\textbf{2.}] User $U_1$ generates a self certifying key $P_1$ and
  signs the message consisting of location data $L_1$, time $t$,
  username $U_1$, user identity $D_1$ and challenge nonce $c1$. Here
  $L_1$ is location data obtained using 3rd party in step 1. $U_1$ sends the signed
  message $(L_1,t,U_1,D_1,c1)S_1$ and $P_1$ to $U_2$.

\item[\textbf{3.}] User $U_2$ generates a self certifying key $P_2$ and
  decrypts the message using the key $P_1$ sent in the message. $U_2$
  then signs the message consisting his location data $L_2$, time $t$,
  username $U_2$, user identity $D_2$ and reverse challenge nonce $c2$. User
  $U_2$ sends key $P_2$, challenge nonce $c1$ and signed message
  $(L_2,t,U_2,D_2,c2)S_2$ to $U_1$.

\item[\textbf{4.}] User $U_1$ decrypts message and sends the signed
  reverse challenge nonce $c2$ back to $U_2$. This completes the
  three-way handshake protocol.

\item[\textbf{5.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. We have to repeat the protocol $n$ times because
  the location information is untrusted. The rationale here is, an
  attacker might try to spoof the identity of $U_2$ once or twice, but
  repeatedly ($n$ times) masquerading the identity of $U_2$ is
  hard. So by repeating the protocol $n$ times, preferably from
  different locations, increases the chances of the user being $U_2$. 

\item[\textbf{6.}] If after $n$ times $(D_2, P_2)$ corresponds to
  $(L_1,L_2,t)$ then with high probability $U_1$ has established a
  secure connection with $U_2$.
\end{enumerate}



\subsection{Multi-Path spatio-temporal repetitive key exchange}

In the previous section we looked at single path key exchange protocol, where
just one channel (SMS) was used to exchange keys between two users with trusted location.
In this section we discuss the multi-path key exchange protocol, where
multiple communication channels are used to exchange keys in a secure
manner using trusted location data. 

\subsubsection{IP and SMS}
The key exchange handshake is the same as described in the previous section, we present here
the key exchange handshake with trusted location data.

\begin{align*}
 \textbf{1}.& \quad W_2 \rightarrow U_1: & & (L_1)S_G  \\
 \textbf{2}.& \quad U_1 \rightarrow IP: & & P_1,t_1,IP_1  \\
           .& \quad U_2 \rightarrow IP: & & P_2,t_2,IP_2  \\
 \textbf{3}.& \quad U_1 \rightarrow U_2: & & (L_1,t,U_1,D_1,c1)S_2 \\
 \textbf{4}.& \quad U_2 \rightarrow U_1: & & (L_2,t,U_2,D_2,c2,c1)S_1,\\
 \textbf{5}.& \quad U_1 \rightarrow U_2: & & (c1,c2)S_1 \\
 \textbf{6}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
 times} \\
 \textbf{7}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] User $U_1$ syncs with a trusted location device $W_2$ which gives
	$U_1$ a certifying location $L_1$. $W_2$ sends the signed message $(L_1)S_G$ to $U_1$.

\item[\textbf{2.}] $U_1$ and $U_2$ exposure their public keys $P_1$
  and $P_2$ respectively though an IP channel. The keys get deleted
  after a certain time period ($t_1$ and $t_2$). $IP_1$ and $IP_2$ are
  IP addresses where $P_1$ and $P_2$ were stored respectively. 

\item[\textbf{3.}] $U_1$ signs the message $(L_1,t,U_1,D_1,c1)$ where
  the message consists of 
  location data $L_1$, time $t$, username $U_1$, user identity $D_1$
  and challenge nonce $c1$. with 
  the public key $S_2$ and sends it to $U_2$ using SMS. $L_1$ is the
  location data obtained in step 1.

\item[\textbf{4.}] $U_2$ decrypts the message and gets the challenge
  nonce $c_1$. $U_2$ signs the message $(L_2,t,U_2,D_2,c2,c1)$ and
  sends it back to $U_1$ using SMS. $L_2$ is the location data of the
  $U_2$ which might be one of, or a combination of i) Trusted location, 
	ii) cell tower information, and iii) GPS information, as
  mentioned on the previous step. 

\item[\textbf{5.}] $U_2$ sends the signed nonces $c1$ and $c2$ to
  $U_2$. This completes the three-way handshake protocol. 


\item[\textbf{6.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. We have to repeat the protocol $n$ times because
  the location information is untrusted. $U_2$ also follows the same
  approach and verifies whether $(D_1, P_1)$ corresponds to
  $(L_1,L_2)$. 

\item[\textbf{7.}] By repeating the protocol $n$ times, the reputation
  score (as described in the previous section) either increases or
  decreases. Once the reputation score crosses a certain threshold,
   then with high probability $U_1$ has established a
  secure connection with $U_2$.

\end{enumerate}


\subsubsection{Bluetooth and SMS}

Following is the detailed version of the Bluetooth protocol using trusted location:

\begin{align*}
 \textbf{1}.& \quad W_2 \rightarrow U_1: & & (L_1)S_G  \\
 \textbf{2}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1)S_1  \\
 \textbf{3}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2)S_2 \\
 \textbf{4}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
            times} \\
 \textbf{5}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}


\begin{enumerate}
\item[\textbf{1.}] User $U_1$ syncs with a trusted location device $W_2$ which gives
	$U_1$ a certifying location $L_1$. $W_2$ sends the signed message $(L_1)S_G$ to $U_1$.
	
\item[\textbf{2.}] $U_1$ sends the location information $L_1$ obtained above, time
  $t$, username $U_1$, user identity $D_1$ to $U_2$ using Bluetooth. 

\item[\textbf{3.}] $U_2$ sends the location information $L_2$, time
  $t$, username $U_2$, user identity $D_2$ to $U_1$ using Bluetooth. 

\item[\textbf{4.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. 

\item[\textbf{5.}] If after $n$ times $(D_2, P_2)$ corresponds to
  $(L_1,L_2,t)$ then with high probability $U_1$ has established a
  secure connection with $U_2$.

\end{enumerate}

==> Old Draft/SMI_with_untrusted_location.tex <==
\section{DSMI with untrusted location}

In this section we will discuss the DSMI protocol in detail using untrusted location data gathered
through GPS and cell tower.

\subsection{SINGLE PATH SPATIO-TEMPORAL REPETITIVE KEY EXCHANGE}\label{singlepath}

In this protocol, only SMS is used to exchange keys between the
users. It is a one-way probabilistically trusted
path under the assumption that the SMS that is sent to a user is
always delivered to that user and that the network is trusted such that
there are no man-in-the-middle attacks possible.
The location information is not trusted, hence the protocol has
a repetitive procedure. Initially keys are exchanged using a simple
3-way handshake protocol where each user generates a self certifying
key. Once the initial 3-way protocol is completed, a reputation score
is maintained by each user. This score is increased based on the
location information obtained from the cell 
towers and the GPS. The assumption here is
the attacker will not follow the user at all times. So if the
adversary was impersonating the user a few times, his location will be
very different from the actual user's location. As the keys are
repetitively exchanged at different intervals of time the location
information is updated. As the user location behavior follows a
specific pattern repeatedly, the reputation score is increased. Same
set of keys are exchanged at different intervals and from different 
locations, where the locations follow a pattern. If the same set of
keys are exchanged from a location that does not follow the
established pattern, then the reputation score is reduced. Else it is
increased. When the reputation score reached a certain threshold the
keys are assumed to be genuine. 

\subsection*{Preliminaries}
\begin{itemize}
\item  Every mobile device is allocated a unique identity $D_1$
(either a phone number or IMSI number)
\item User $U_1$ registers with provider a $X_1$ using a device $W_1$
  with a unique identity $D_1$ 
\item If $W_1$ is directly connected to an authorized base station of
  provider $X_1$, then anyone who sends a message to identity $D_1$ is
  routed to $W_1$ and is received by user $U_1$.
%\item The routing layer within the cellular network is trusted
\end{itemize}


The step by step protocol is described as follows.

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1,c1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2,c2)S_2,c1 \\
 \textbf{3}.& \quad U_1 \rightarrow U_2: & & (c2)S_1 \\
 \textbf{4}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
 times} \\
 \textbf{5}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] User $U_1$ generates a self certifying key $P_1$ and
  signs the message consisting of location data $L_1$, time $t$,
  username $U_1$, user identity $D_1$ and challenge nonce $c1$. Here
  $L_1$ is the location data which might be the location of the cell
  tower combined with the GPS coordinates. $U_1$ sends the signed
  message $(L_1,t,U_1,D_1,c1)S_1$ and $P_1$ to $U_2$.

\item[\textbf{2.}] User $U_2$ generates a self certifying key $P_2$ and
  decrypts the message using the key $P_1$ sent in the message. $U_2$
  then signs the message consisting his location data $L_2$, time $t$,
  username $U_2$, user identity $D_2$ and reverse challenge nonce $c2$. User
  $U_2$ sends key $P_2$, challenge nonce $c1$ and signed message
  $(L_2,t,U_2,D_2,c2)S_2$ to $U_1$.

\item[\textbf{3.}] User $U_1$ decrypts message and sends the signed
  reverse challenge nonce $c2$ back to $U_2$. This completes the
  three-way handshake protocol.

\item[\textbf{4.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. We have to repeat the protocol $n$ times because
  the location information is untrusted. The rationale here is, an
  attacker might try to spoof the identity of $U_2$ once or twice, but
  repeatedly ($n$ times) masquerading the identity of $U_2$ is
  hard. So by repeating the protocol $n$ times, preferably from
  different locations, increases the chances of the user being $U_2$. 

\item[\textbf{5.}] If after $n$ times $(D_2, P_2)$ corresponds to
  $(L_1,L_2,t)$ then with high probability $U_1$ has established a
  secure connection with $U_2$.
\end{enumerate}

\subsubsection{Security Analysis}

In Step 1, $U_1$ generates a self certifying key $P_1$, signs the
message which contains the location data $L_1$, time $t$,
  username $U_1$, user identity $D_1$ and challenge nonce $c1$, and
  sends the message and $P_1$ to the other user $U_2$. As we discussed
  in the previous Section, the cellular network is one-way
  probabilistically secure. An adversary can spoof the cellphone
  number of $U_1$ and hijack the message. But if $U_2$ is present in
  the cellular network $U_2$ would also receive the message, since the
  message is being routed to $U_2$'s number. The adversary could
  create a fake base station within $U_2$'s vicinity and hijack the
  message. In this case $U_2$ would never receive the message. The
  adversary could continue the entire protocol with $U_1$. But this is
  a highly unlikely event due to the following reasons. i) the
  adversary has to be in the vicinity of $U_2$ at the exact moment
  when the message is sent to by $U_1$ to $U_2$. ii) during the entire
  course of the protocol the $U_2$'s cellphone has be switched off, so
  that $U_2$ can't join the network. If $U_2$ joins the network during
  the course of the protocol, $U_2$ would get an encrypted message
  from $U_1$ with no key to decrypt. This would alert $U_2$ about the
  MITM attack and $U_2$ could send a message to $U_1$ to abort the
  protocol. $U_1$ would receive messages from two different locations
  and because of this $U_1$ would abort the protocol. Another scenario
  is $U_2$ would switch on the phone during the repetitive location
  exchange step. This would again give $U_1$ different or
  inconsistent location information and $U_1$ would abort the protocol. 

In Step 2, $U_2$ first checks if the message sent by $U_1$ is
consistent. If not, it aborts the protocol. If the message is
consistent, $U_2$ generates its self
certifying keys and signs the message containing its location data
$L_2$, time $t$, username $U_2$, user identity $D_2$ and reverse
challenge nonce $c2$.  An adversary could spoof $U_1$'s message. So
$U_2$ does not have any guarantee that the message was indeed sent by
$U_1$. Only in step 5 of the protocol when the reputation score goes
above a certain threshold, $U_2$ would have established a secure key
exchange with $U_1$.

In Step 3, $U_1$ checks if the message sent by $U_2$ is consistent. If
not, $U_1$ aborts the protocol. Else, $U_1$ will sign a reverse
challenge response $c_2$ and send it to $U_2$.

{\em Reputation score:} In Step 4, $U_1$ stores $(D_2, P_2)$ and its
corresponding location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. Similarly, $U_2$ stores the $(D_1, P_1)$ and its
  corresponding location information and time $(L_1, L_2)$. In this
  step, the keys are exchanged $n$ times. Each time if the location
  and time information are consistent then the reputation score is
  increased by 1. If the time to send or receive the message is
  greater than a certain time $T$, then the reputation score is reset
  to zero and Step 4 is started again. An adversary could spoof the
  location and time message by performing a MITM attack, but since the
  step is performed $n$ at different locations and time periods, the
  adversary would not be able to modify the message such that either
  $U_1$ or $U_2$ would always get consistent location and time
  information. Also, if the message is inconsistent $k$ times, then
  the protocol is aborted. When the reputation score
  passes $n$, then $U_1$ and $U_2$ have exchanged keys with high
  probability. 

\subsection{Multi-Path spatio-temporal repetitive key exchange}

In section \ref{singlepath} we looked at single path key exchange protocol, where
just one channel (SMS) was used to exchange keys between two users. In
the section we discuss the multi-path key exchange protocol, where
multiple communication channels are used to exchange keys in a secure
manner. We introduce two such paths: IP-SMS and Bluetooth-SMS; both of
which are discussed in detail below. The assumption is that the attacker can compromise a single path
and the probability of attacking another path is very low. Thus, having more
than one path adds to the security. 

\subsubsection{IP and SMS}
The first protocol in the multi-path key exchange is a protocol that
uses an IP path and SMS to exchange keys. The user initiates the key exchange
handshake using IP channel. User A sends its data (A's number, A's location,
A's challenge, current time, A's public key) to a centralized server. Once A's
data is uploaded on the server successfully, A send the nonce to B via SMS. User
B when receives the SMS, uploads its own data on the server and sends the reply 
to A's challenge via SMS. User A receives the response, verifies it, stores B's
information in its table and fetches B's information from the server. A then replies
back to B with the challenge response which B receives and stores it in its table
after verifying it. It should be noted that the messages on the server are removed
as soon as the user fetches the data from the server.


The step by step protocol is described as follows.

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow IP: & & P_1,t_1,IP_1  \\
           .& \quad U_2 \rightarrow IP: & & P_2,t_2,IP_2  \\
 \textbf{2}.& \quad U_1 \rightarrow U_2: & & (L_1,t,U_1,D_1,c1)S_2 \\
 \textbf{3}.& \quad U_2 \rightarrow U_1: & & (L_2,t,U_2,D_2,c2,c1)S_1,\\
 \textbf{4}.& \quad U_1 \rightarrow U_2: & & (c1,c2)S_1 \\
 \textbf{5}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
 times} \\
 \textbf{6}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] $U_1$ and $U_2$ exposure their public keys $P_1$
  and $P_2$ respectively though an IP channel. The keys get deleted
  after a certain time period ($t_1$ and $t_2$). $IP_1$ and $IP_2$ are
  IP addresses where $P_1$ and $P_2$ were stored respectively. 

\item[\textbf{2.}] $U_1$ signs the message $(L_1,t,U_1,D_1,c1)$ where
  the message consists of 
  location data $L_1$, time $t$, username $U_1$, user identity $D_1$
  and challenge nonce $c1$. with 
  the public key $S_2$ and sends it to $U_2$ using SMS. $L_1$ is the
  location data which might be a one of, or a combination three types of
  location information, i) IP-geographic location, ii) cell tower
  information, and iii) GPS information.

\item[\textbf{3.}] $U_2$ decrypts the message and gets the challenge
  nonce $c_1$. $U_2$ signs the message $(L_2,t,U_2,D_2,c2,c1)$ and
  sends it back to $U_1$ using SMS. $L_2$ is the location data of the
  $U_2$ which might be one of, or a combination of i) IP-geographic
  location, ii) cell tower information, and iii) GPS information, as
  mentioned on the previous step. 

\item[\textbf{4.}] $U_2$ sends the signed nonces $c1$ and $c2$ to
  $U_2$. This completes the three-way handshake protocol. 


\item[\textbf{5.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. We have to repeat the protocol $n$ times because
  the location information is untrusted. $U_2$ also follows the same
  approach and verifies whether $(D_1, P_1)$ corresponds to
  $(L_1,L_2)$. 

\item[\textbf{6.}] By repeating the protocol $n$ times, the reputation
  score (as described in the previous section) either increases or
  decreases. Once the reputation score crosses a certain threshold,
   then with high probability $U_1$ has established a
  secure connection with $U_2$.

\end{enumerate}


\paragraph{Security Analysis}

In Step 1, $U_1$ and $U_2$ use publicly recognized IP to send or store
their respective public keys. Since each IP address can be
geographically mapped, the location information of both $U_1$ and
$U_2$ can be determined. Since we are assuming that the IP is public,
the adversary cannot spoof the location information. This initial location
information of $U_1$ and $U_2$ plays a significant role in the later
steps when the reputation score is computed.

In Step 2, $U_1$ signs the message with $U_2$ key and sends it to
$U_2$ using SMS. Note that this is a different channel than Step 1. In
Step 1, the IP-channel was used to get the key and location
information. In Step 2, since the channel used is SMS, the encrypted
message has to be go through the cellular route. As discussed earlier,
the cellular channel is one-way probabilistically secure. Therefore if
in Step 1 the adversary spoofed the user, then in Step 2, when the
message is sent using the cellular network it reaches the genuine user
with high probability. Once the message is sent if there is no
response within a certain period of time or if the response from $U_2$
is negative, this means that there is a MITM attack and the protocol
is aborted. 

In Step 3, if the message sent by $U_1$ reaches $U_2$, then $U_2$
sends back the response with a signed message with its location data
$L_2$, time $t$, username $U_2$, user identity $D_2$ and reverse 
challenge nonce $c2$.  An adversary could spoof $U_1$'s message. So
$U_2$ does not have any guarantee that the message was indeed sent by
$U_1$. Only in step 5 of the protocol when the reputation score goes
above a certain threshold, $U_2$ would have established a secure key
exchange with $U_1$.

In Step 4, $U_1$ checks if the message sent by $U_2$ is consistent. If
not, $U_1$ aborts the protocol. Else, $U_1$ will sign a reverse
challenge response $c_2$ and send it to $U_2$.

In Step 5 and 6, the protocol is repeated $n$ times to check for
consistency in the (key,location) pair. $U_1$ stores $(D_2, P_2)$ and its
corresponding location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. Similarly, $U_2$ stores the $(D_1, P_1)$ and its
  corresponding location information and time $(L_1, L_2)$. The
  reputation score is computed in the same manner as described in the
  single path key exchange protocol. The difference in the multi-path
  protocol is that initial exchange of keys using a different channel
  or path. The number of rounds of key and location information
  exchanges might be reduced, if Step 1 to Step 4 are consistent. This
  means the keys that were exchanged in Step 1 are being used in
  subsequent steps (in the cellular network) so there is a high
  probability that the users are genuine. 

\subsubsection{Bluetooth and SMS}
In this protocol, the users are in close proximity and Bluetooth is
used to exchange keys between them. Once the keys and the messages are
exchanged the users can communicate securely using SMS or other channels.
Bluetooth is an unreliable way of communication as described in \cite{bluetooth1}
and \cite{bluetooth2}. For added security, when user A opts Bluetooth as a mean
of key exchange the system asks for a password which both users: A and B; should
decide before starting the key exchange. Once they both enter the same password-
the key exchange process starts. User A sends its data (A's number, A's location,
A's challenge, current time, A's public key) to B via bluetooth. User
B when receives the SMS, sends its own data to A via Bluetooth and sends the reply 
to A's challenge via SMS. User A receives the SMS response, verifies it, stores B's
information in its table and when it receives B's data; replies
back to B with the challenge response via SMS which B receives and stores it in its table
after verifying it. 


\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2)S_2 \\
 \textbf{3}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
 times} \\
 \textbf{4}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}


\begin{enumerate}
\item[\textbf{1.}] $U_1$ sends the location information $L_1$, time
  $t$, username $U_1$, user identity $D_1$ to $U_2$ using Bluetooth. 

\item[\textbf{2.}] $U_2$ sends the location information $L_2$, time
  $t$, username $U_2$, user identity $D_2$ to $U_1$ using Bluetooth. 

\item[\textbf{4.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. 

\item[\textbf{5.}] If after $n$ times $(D_2, P_2)$ corresponds to
  $(L_1,L_2,t)$ then with high probability $U_1$ has established a
  secure connection with $U_2$.

\end{enumerate}

\paragraph{Security Analysis}

In Step 1 and 2, $U_1$ and $U_2$ exchange keys using Bluetooth which
means they are in close proximity to each other. But there is a
possibility that the $U_1$ has not met $U_2$ before and does not have
any information on $U_2$'s identity and vice-versa. Hence just the key
exchange using Bluetooth is not sufficient. The repetitive key
exchange protocol is necessary to ensure that the users are talking to
each other instead of the adversary. In Step 3 and 4, reputation score
is computed just as in earlier protocols. In the first step the
messages were exchanged using Bluetooth and in the subsequent steps
the messages were exchanged using SMS. If the messages are consistent
from Step 1 to Step 4 and the repetitive key exchange is performed as
described in the earlier protocols, then there is no MITM attack and
the users can communicate with each in a secure manner. 




==> Old Draft/SMIprotocol.tex <==
\section{The Secure Mobile Identities Protocol Details}

In this section we will discuss the DSMI protocol in detail using untrusted and trusted
location data gathered through GPS and cell tower and 3rd party services.

\subsection{Single Path Spatio-Temporal Repetitive Key Exchange}\label{singlepath}

In this protocol, only SMS is used to exchange keys between the
users. It is a one-way probabilistically trusted
path under the assumption that the SMS that is sent to a user is
always delivered to that user and that the network is trusted such that
there are no man-in-the-middle attacks possible.
The location information is not trusted, hence the protocol has
a repetitive procedure. Initially keys are exchanged using a simple
3-way handshake protocol where each user generates a self certifying
key. Once the initial 3-way protocol is completed, a reputation score
is maintained by each user. This score is increased based on the
location information obtained from the cell 
towers and the GPS. The assumption here is
the attacker will not follow the user at all times. So if the
adversary was impersonating the user a few times, his location will be
very different from the actual user's location. As the keys are
repetitively exchanged at different intervals of time the location
information is updated. As the user location behavior follows a
specific pattern repeatedly, the reputation score is increased. Same
set of keys are exchanged at different intervals and from different 
locations, where the locations follow a pattern. If the same set of
keys are exchanged from a location that does not follow the
established pattern, then the reputation score is reduced. Else it is
increased. When the reputation score reached a certain threshold the
keys are assumed to be genuine. 

\subsection*{Preliminaries}
\begin{itemize}
\item  Every mobile device is allocated a unique identity $D_1$
(either a phone number or IMSI number)
\item User $U_1$ registers with provider a $X_1$ using a device $W_1$
  with a unique identity $D_1$ 
\item If $W_1$ is directly connected to an authorized base station of
  provider $X_1$, then anyone who sends a message to identity $D_1$ is
  routed to $W_1$ and is received by user $U_1$.
%\item The routing layer within the cellular network is trusted
\end{itemize}


The step by step protocol is described as follows.

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1,c1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2,c2)S_2,c1 \\
 \textbf{3}.& \quad U_1 \rightarrow U_2: & & (c2)S_1 \\
 \textbf{4}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
 times} \\
 \textbf{5}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] User $U_1$ generates a self certifying key $P_1$ and
  signs the message consisting of location data $L_1$, time $t$,
  username $U_1$, user identity $D_1$ and challenge nonce $c1$. Here
  $L_1$ is the location data which might be the location of the cell
  tower combined with the GPS coordinates. $U_1$ sends the signed
  message $(L_1,t,U_1,D_1,c1)S_1$ and $P_1$ to $U_2$.

\item[\textbf{2.}] User $U_2$ generates a self certifying key $P_2$ and
  decrypts the message using the key $P_1$ sent in the message. $U_2$
  then signs the message consisting his location data $L_2$, time $t$,
  username $U_2$, user identity $D_2$ and reverse challenge nonce $c2$. User
  $U_2$ sends key $P_2$, challenge nonce $c1$ and signed message
  $(L_2,t,U_2,D_2,c2)S_2$ to $U_1$.

\item[\textbf{3.}] User $U_1$ decrypts message and sends the signed
  reverse challenge nonce $c2$ back to $U_2$. This completes the
  three-way handshake protocol.

\item[\textbf{4.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. We have to repeat the protocol $n$ times because
  the location information is untrusted. The rationale here is, an
  attacker might try to spoof the identity of $U_2$ once or twice, but
  repeatedly ($n$ times) masquerading the identity of $U_2$ is
  hard. So by repeating the protocol $n$ times, preferably from
  different locations, increases the chances of the user being $U_2$. 

\item[\textbf{5.}] If after $n$ times $(D_2, P_2)$ corresponds to
  $(L_1,L_2,t)$ then with high probability $U_1$ has established a
  secure connection with $U_2$.
\end{enumerate}

\subsubsection{Security Analysis}

In Step 1, $U_1$ generates a self certifying key $P_1$, signs the
message which contains the location data $L_1$, time $t$,
  username $U_1$, user identity $D_1$ and challenge nonce $c1$, and
  sends the message and $P_1$ to the other user $U_2$. As we discussed
  in the previous Section, the cellular network is one-way
  probabilistically secure. An adversary can spoof the cellphone
  number of $U_1$ and hijack the message. But if $U_2$ is present in
  the cellular network $U_2$ would also receive the message, since the
  message is being routed to $U_2$'s number. The adversary could
  create a fake base station within $U_2$'s vicinity and hijack the
  message. In this case $U_2$ would never receive the message. The
  adversary could continue the entire protocol with $U_1$. But this is
  a highly unlikely event due to the following reasons. i) the
  adversary has to be in the vicinity of $U_2$ at the exact moment
  when the message is sent to by $U_1$ to $U_2$. ii) during the entire
  course of the protocol the $U_2$'s cellphone has be switched off, so
  that $U_2$ can't join the network. If $U_2$ joins the network during
  the course of the protocol, $U_2$ would get an encrypted message
  from $U_1$ with no key to decrypt. This would alert $U_2$ about the
  MITM attack and $U_2$ could send a message to $U_1$ to abort the
  protocol. $U_1$ would receive messages from two different locations
  and because of this $U_1$ would abort the protocol. Another scenario
  is $U_2$ would switch on the phone during the repetitive location
  exchange step. This would again give $U_1$ different or
  inconsistent location information and $U_1$ would abort the protocol. 

In Step 2, $U_2$ first checks if the message sent by $U_1$ is
consistent. If not, it aborts the protocol. If the message is
consistent, $U_2$ generates its self
certifying keys and signs the message containing its location data
$L_2$, time $t$, username $U_2$, user identity $D_2$ and reverse
challenge nonce $c2$.  An adversary could spoof $U_1$'s message. So
$U_2$ does not have any guarantee that the message was indeed sent by
$U_1$. Only in step 5 of the protocol when the reputation score goes
above a certain threshold, $U_2$ would have established a secure key
exchange with $U_1$.

In Step 3, $U_1$ checks if the message sent by $U_2$ is consistent. If
not, $U_1$ aborts the protocol. Else, $U_1$ will sign a reverse
challenge response $c_2$ and send it to $U_2$.

{\em Reputation score:} In Step 4, $U_1$ stores $(D_2, P_2)$ and its
corresponding location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. Similarly, $U_2$ stores the $(D_1, P_1)$ and its
  corresponding location information and time $(L_1, L_2)$. In this
  step, the keys are exchanged $n$ times. Each time if the location
  and time information are consistent then the reputation score is
  increased by 1. If the time to send or receive the message is
  greater than a certain time $T$, then the reputation score is reset
  to zero and Step 4 is started again. An adversary could spoof the
  location and time message by performing a MITM attack, but since the
  step is performed $n$ at different locations and time periods, the
  adversary would not be able to modify the message such that either
  $U_1$ or $U_2$ would always get consistent location and time
  information. Also, if the message is inconsistent $k$ times, then
  the protocol is aborted. When the reputation score
  passes $n$, then $U_1$ and $U_2$ have exchanged keys with high
  probability. 

\subsection{Multi-Path spatio-temporal repetitive key exchange}\label{multi-path}

In section \ref{singlepath} we looked at single path key exchange protocol, where
just one channel (SMS) was used to exchange keys between two users. In
the section we discuss the multi-path key exchange protocol, where
multiple communication channels are used to exchange keys in a secure
manner. We introduce two such paths: IP-SMS and Bluetooth-SMS; both of
which are discussed in detail below. The assumption is that the attacker can compromise a single path
and the probability of attacking another path is very low. Thus, having more
than one path adds to the security. 

\subsubsection{IP and SMS}
The first protocol in the multi-path key exchange is a protocol that
uses an IP path and SMS to exchange keys. The user initiates the key exchange
handshake using IP channel. User A sends its data (A's number, A's location,
A's challenge, current time, A's public key) to a centralized server. Once A's
data is uploaded on the server successfully, A send the nonce to B via SMS. User
B when receives the SMS, uploads its own data on the server and sends the reply 
to A's challenge via SMS. User A receives the response, verifies it, stores B's
information in its table and fetches B's information from the server. A then replies
back to B with the challenge response which B receives and stores it in its table
after verifying it. It should be noted that the messages on the server are removed
as soon as the user fetches the data from the server.


The step by step protocol is described as follows.

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow IP: & & P_1,t_1,IP_1  \\
           .& \quad U_2 \rightarrow IP: & & P_2,t_2,IP_2  \\
 \textbf{2}.& \quad U_1 \rightarrow U_2: & & (L_1,t,U_1,D_1,c1)S_2 \\
 \textbf{3}.& \quad U_2 \rightarrow U_1: & & (L_2,t,U_2,D_2,c2,c1)S_1,\\
 \textbf{4}.& \quad U_1 \rightarrow U_2: & & (c1,c2)S_1 \\
 \textbf{5}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
 times} \\
 \textbf{6}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] $U_1$ and $U_2$ exposure their public keys $P_1$
  and $P_2$ respectively though an IP channel. The keys get deleted
  after a certain time period ($t_1$ and $t_2$). $IP_1$ and $IP_2$ are
  IP addresses where $P_1$ and $P_2$ were stored respectively. 

\item[\textbf{2.}] $U_1$ signs the message $(L_1,t,U_1,D_1,c1)$ where
  the message consists of 
  location data $L_1$, time $t$, username $U_1$, user identity $D_1$
  and challenge nonce $c1$. with 
  the public key $S_2$ and sends it to $U_2$ using SMS. $L_1$ is the
  location data which might be a one of, or a combination three types of
  location information, i) IP-geographic location, ii) cell tower
  information, and iii) GPS information.

\item[\textbf{3.}] $U_2$ decrypts the message and gets the challenge
  nonce $c_1$. $U_2$ signs the message $(L_2,t,U_2,D_2,c2,c1)$ and
  sends it back to $U_1$ using SMS. $L_2$ is the location data of the
  $U_2$ which might be one of, or a combination of i) IP-geographic
  location, ii) cell tower information, and iii) GPS information, as
  mentioned on the previous step. 

\item[\textbf{4.}] $U_2$ sends the signed nonces $c1$ and $c2$ to
  $U_2$. This completes the three-way handshake protocol. 


\item[\textbf{5.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. We have to repeat the protocol $n$ times because
  the location information is untrusted. $U_2$ also follows the same
  approach and verifies whether $(D_1, P_1)$ corresponds to
  $(L_1,L_2)$. 

\item[\textbf{6.}] By repeating the protocol $n$ times, the reputation
  score (as described in the previous section) either increases or
  decreases. Once the reputation score crosses a certain threshold,
   then with high probability $U_1$ has established a
  secure connection with $U_2$.

\end{enumerate}


\paragraph{Security Analysis}

In Step 1, $U_1$ and $U_2$ use publicly recognized IP to send or store
their respective public keys. Since each IP address can be
geographically mapped, the location information of both $U_1$ and
$U_2$ can be determined. Since we are assuming that the IP is public,
the adversary cannot spoof the location information. This initial location
information of $U_1$ and $U_2$ plays a significant role in the later
steps when the reputation score is computed.

In Step 2, $U_1$ signs the message with $U_2$ key and sends it to
$U_2$ using SMS. Note that this is a different channel than Step 1. In
Step 1, the IP-channel was used to get the key and location
information. In Step 2, since the channel used is SMS, the encrypted
message has to be go through the cellular route. As discussed earlier,
the cellular channel is one-way probabilistically secure. Therefore if
in Step 1 the adversary spoofed the user, then in Step 2, when the
message is sent using the cellular network it reaches the genuine user
with high probability. Once the message is sent if there is no
response within a certain period of time or if the response from $U_2$
is negative, this means that there is a MITM attack and the protocol
is aborted. 

In Step 3, if the message sent by $U_1$ reaches $U_2$, then $U_2$
sends back the response with a signed message with its location data
$L_2$, time $t$, username $U_2$, user identity $D_2$ and reverse 
challenge nonce $c2$.  An adversary could spoof $U_1$'s message. So
$U_2$ does not have any guarantee that the message was indeed sent by
$U_1$. Only in step 5 of the protocol when the reputation score goes
above a certain threshold, $U_2$ would have established a secure key
exchange with $U_1$.

In Step 4, $U_1$ checks if the message sent by $U_2$ is consistent. If
not, $U_1$ aborts the protocol. Else, $U_1$ will sign a reverse
challenge response $c_2$ and send it to $U_2$.

In Step 5 and 6, the protocol is repeated $n$ times to check for
consistency in the (key,location) pair. $U_1$ stores $(D_2, P_2)$ and its
corresponding location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. Similarly, $U_2$ stores the $(D_1, P_1)$ and its
  corresponding location information and time $(L_1, L_2)$. The
  reputation score is computed in the same manner as described in the
  single path key exchange protocol. The difference in the multi-path
  protocol is that initial exchange of keys using a different channel
  or path. The number of rounds of key and location information
  exchanges might be reduced, if Step 1 to Step 4 are consistent. This
  means the keys that were exchanged in Step 1 are being used in
  subsequent steps (in the cellular network) so there is a high
  probability that the users are genuine. 

\subsubsection{Bluetooth and SMS}
In this protocol, the users are in close proximity and Bluetooth is
used to exchange keys between them. Once the keys and the messages are
exchanged the users can communicate securely using SMS or other channels.
Bluetooth is an unreliable way of communication as described in \cite{bluetooth1}
and \cite{bluetooth2}. For added security, when user A opts Bluetooth as a mean
of key exchange the system asks for a password which both users: A and B; should
decide before starting the key exchange. Once they both enter the same password-
the key exchange process starts. User A sends its data (A's number, A's location,
A's challenge, current time, A's public key) to B via bluetooth. User
B when receives the SMS, sends its own data to A via Bluetooth and sends the reply 
to A's challenge via SMS. User A receives the SMS response, verifies it, stores B's
information in its table and when it receives B's data; replies
back to B with the challenge response via SMS which B receives and stores it in its table
after verifying it. 


\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2)S_2 \\
 \textbf{3}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
 times} \\
 \textbf{4}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}


\begin{enumerate}
\item[\textbf{1.}] $U_1$ sends the location information $L_1$, time
  $t$, username $U_1$, user identity $D_1$ to $U_2$ using Bluetooth. 

\item[\textbf{2.}] $U_2$ sends the location information $L_2$, time
  $t$, username $U_2$, user identity $D_2$ to $U_1$ using Bluetooth. 

\item[\textbf{4.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. 

\item[\textbf{5.}] If after $n$ times $(D_2, P_2)$ corresponds to
  $(L_1,L_2,t)$ then with high probability $U_1$ has established a
  secure connection with $U_2$.

\end{enumerate}

\paragraph{Security Analysis}

In Step 1 and 2, $U_1$ and $U_2$ exchange keys using Bluetooth which
means they are in close proximity to each other. But there is a
possibility that the $U_1$ has not met $U_2$ before and does not have
any information on $U_2$'s identity and vice-versa. Hence just the key
exchange using Bluetooth is not sufficient. The repetitive key
exchange protocol is necessary to ensure that the users are talking to
each other instead of the adversary. In Step 3 and 4, reputation score
is computed just as in earlier protocols. In the first step the
messages were exchanged using Bluetooth and in the subsequent steps
the messages were exchanged using SMS. If the messages are consistent
from Step 1 to Step 4 and the repetitive key exchange is performed as
described in the earlier protocols, then there is no MITM attack and
the users can communicate with each in a secure manner. 

\subsection{Trusted location based key exchange}

The location data gathered through GPS and cell tower is not trusted and can easily be manipulated.
We need a secure and trusted location gathering mechanism. By a trusted location we mean a location that
can not be changed by an attacker and is signed by a trusted 3rd party. The location data gathered through
these trusted points of location gathering devices is considered the most authentic and a user having a trusted
location gains more score points. There can be a number of ways to achieve this. We present a few of those
techniques in this paper. Instead of gathering location through GPS, this is an added security step that 
can be included in the DSMI protocol as explained in section \ref{singlepath} and \ref{multi-path}.

\subsubsection{Third-party trusted location devices}

A trusted 3rd party installs some of these certifying location gathering devices in a few places for a user to sync
their device and gets a certifying location along with a time stamp. The location data is actually the location
of that device and as the user is in close proximity of that device; the location of the user is the same as that
of the device. Syncing can be done via bluetooth or any other technology. This is something very trivial to do
as Google already has deployed its Google wallet points at various location. A user can sync up with the
Google wallet point and get a certifying location. 

\subsubsection{Geolocation}

Another way of gathering location data is through IP. As the public IP address of every device is unique and IP
addresses are assigned in the form of a tier system based on the geographical location. It is possible to gather
the location information through IP. Mapping IP addresses to a geographical location is known as Geolocation and is
described in \cite{taylor2012bringing}  and \cite{kovacs2002geolocation}. The idea is to have a trusted 3rd party
hotspot deployed at various location so that a user can sync the mobile to get a certifying IP location. The IP
location can further be processed as discussed above to break it down to geographical location. 


\subsubsection{Trusted location data}
\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1,c1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2,c2)S_2,c1 \\
 \textbf{3}.& \quad U_1 \rightarrow U_2: & & (c2)S_1 \\
\end{align*}
In this protocol, the location data ($L_1,L_2,t)$ is from a trusted
source. The GPS chip within the mobile devices $W_1,W_2$ are trusted
and the cell tower information obtained is also trusted. Hence the
protocol boils down to the three-way handshake protocol. 


\subsubsection{Trusted point of sale device}

\subsubsection*{Assumptions}
\begin{itemize}
\item Point of sale devices are trusted. 
\item Point of sale devices have the ability to sign a message and
  transmit the message securely to the device $W_1$ of the user $U_1$.
\end{itemize}

\subsubsection*{Protocol}

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow G: & & P_1,L_1,t,U_1,D_1  \\
 \textbf{2}.& \quad G \rightarrow U_1: & & G_P, (P_1,L_1,t,U_1,D_1)G_S \\
 \textbf{3}.& \quad U_1 \rightarrow C: & & P_1, (G_P,(P_1,L_1,t,U_1,D_1)G_S)S_1 \\
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] $U_1$ sends the message $P_1,L_1,t,U_1,D_1$ to a
  point of sale device $G$. 

\item[\textbf{2.}] A point of sale device can be a NFC
  device or other device which is capable to signing a message. The
  point of sale device $G$ signs the message $(P_1,L_1,t,U_1,D_1)G_S$
  and along with $G_P$ (public key) sends it back to $U_1$.

\item[\textbf{3.}] Now $U_1$ signs the message it received from $G$,

  ($P_1$,$L_1$,$t$,$U_1$,$D_1$)$G_S$)$S_1$ and sends it to the central
  authority $C$ along with $P_1$. Since $G$ is trusted (has trusted
  credentials), $C$ is certain that the message is signed by $G$ and
  that $U_1$ was indeed present at the point of sale location. The
  point of sale device could also have a fingerprint reader (or any
  biometric device) to authenticate user's identity and the biometric
  data can also be part of the signed message from $G$ to $U_1$. 
\end{enumerate}



==> Old Draft/abstract-new.tex <==
\begin{abstract}

%motivation%
The proliferation of cell phones has brought out issues in security
as they are becoming more and more vulnerable as targets 
for attack \cite{cyberThreats} like man-in-the-middle (MITM) attacks and 
phishing attacks where an attacker may trick the user by masquerading 
as a trustworthy entity. 
%related work 2-3%
Methods like SSL/TLS-a third party service,
apps which use one-time PIN and passwords, protocols that require the users to be there
physically are some of the examples of the efforts made to solve this issue.
%DSMI 3-4%
In this paper we propose the design
and implementation of Secure Mobile Identities (DSMI), a protocol that promises a 
secure and reliable communication by exchanging and authenticating keys.
The key idea of DSMI is to provide a spatio-temporal, multi-path, repetitive 
challenge-response key exchange protocol to enable two mobile entities to 
builds up reputation across multiple levels of trust.
%Applications 1-2%
Many new and existing applications can be built on top of DSMI which require sensitive data handling
such as apps that involve money transactions or apps that involve sensitive data transaction. 
%evaluation results%
In this paper we show the protocol 
implementation and evaluation across variety of channels. 



\begin{comment}
%motivation%
The proliferation of cell phones has brought out issues in security
which is causing a major problem worldwide. 
Mobile phones are becoming more and more vulnerable as targets 
for attack \cite{cyberThreats}. Some major security threats that a 
common user is facing are man-in-the-middle (MITM) attacks and 
phishing attacks where an attacker may trick the user by masquerading 
as a trustworthy entity. 

%related work 2-3%
Methods like SSL/TLS-a third party service,
apps which use one-time PIN and passwords, protocols that require the users to be there
physically are some of the examples of the efforts made to solve this issue.

%DSMI 3-4%

In this paper we propose the design
and implementation of Secure Mobile Identities (DSMI), a protocol that promises a 
secure and reliable communication by exchanging and authenticating keys.
The key idea of DSMI is to provide a spatio-temporal, multi-path, repetitive 
challenge-response key exchange protocol to enable two mobile entities to 
builds up reputation across multiple levels of trust. DSMI tags keys with 
location and time and populates the table for 
the same traditional (identity, key) pair.

%Applications 1-2%
\\Many new applications can be built on top of DSMI which require sensitive data handling
such as apps that involve money transactions or apps that involve sensitive data transaction. 

%evaluation results%
\\In this paper we show the protocol 
implementation and evaluation across variety of channels. 
\end{comment}
\end{abstract}

==> Old Draft/abstract.tex <==
\begin{abstract}
Mobile devices are increasingly becoming vulnerable to a variety of
network-level security threats including different types of
man-in-the-middle (MITM) attacks such as message interceptions and
modifications, eavesdropping on calls and text messages, message
spoofing and phishing attacks. In this paper, we propose the design
and implementation of Secure Mobile Identities (DSMI), a secure
key-exchange protocol that enables a mobile user to establish a secure
and trustworthy communication channel with other mobile users in the
face of external adversaries.  The design of DSMI places initial
bootstrap trust on the cellular providers and builds upon the basic
assumption that cellular networks offer a unique ``partially
trustworthy one-way'' channel to connected mobile devices; unlike
Internet routes which can be hijacked, the cellular network routing
layer is closed thereby forcing the MITM attacker to attack only the
last-hop wireless channel between the tower and the device. Building
on this assumption, DSMI provides a spatio-temporal, multi-path,
repetitive challenge-response key exchange protocol to enable two
mobile entities to tag every key exchange with a (location, time,
path) triplet and leverage diversity across paths to build a trust
reputation for every key. The security of DSMI can be further enhanced
with the use of external trusted entities providing non-forgeable
trusted location signatures (e.g. trusted GPS, trusted cell towers,
physical synchronization points). In this paper, we demonstrate the
effectiveness of our protocol using a prototype implementation and
demonstrate ease of use across a variety of real-world channels. We
also show how the DSMI abstraction can enable new forms of secure
mobile applications including secure cash transfer, secure physical
identities and secure file exchange.

\end{abstract}



==> Old Draft/abstract_mod.tex <==
\begin{abstract}
The proliferation of cellphones has brought out issues in security
which is causing major problems worldwide. 
Recent reports suggests that due to vulnerabilities in the network, 
security loopholes exist which puts the users at risk to
attackers\cite{cyberThreats}. Man-in-the-middle (MITM)
attacks such as snooping, eavesdropping on phone calls and text
messages, to jamming the channel to block access to secure session
,phishing attacks where an attacker may trick
the user by masquerading as a trustworthy entity, have been
increasing. In this paper we present the design and implementation of
Secure Mobile Identities (DSMI), a key exchange protocol that helps the
users to communicate in a secure manner. 
The key idea of DSMI is to provide a spatio-temporal, multi-path, repetitive 
challenge-response key exchange protocol to enable two mobile entities
to develop trust in order to communicate securely. Assuming the
cellular network is a trusted one way probabilistic path, we use self
certifying keys, location of the devices and communication
channels in different ways to increase the trust in the mobile
identity of each person. 
We develop a real world implementation and evaluate the protocol
across a variety of communication channels. 

\end{abstract}


==> Old Draft/appANDeval.tex <==
\section{Applications and Evaluation}

There can be various applications that can be built on top of Secure Mobile
Identities protocol. DSMI promises security and reliability along with usability.
DSMI does not involve any user involvement and the simplicity of DSMI makes
it favorable to be adapted in existing as well as new applications.
To evaluate the usability of Secure Mobile Identities usability
we conducted trial runs and tests to gather stats.

\subsection{Applications}

We present here some of the ideas of the applications which we think can be built
on top of DSMI protocol seamlessly. 

\subsubsection{Secure Cash}
We can leverage DSMI to build an app that requires the most security. We can build a virtual
cash system on top of DSMI which can be used as the security layer. The bank is a trusted 
party whose secure cash app would allow its customers to perform secure digital transactions.
The secure cash is the implementation of the process of sending and receiving a bank transaction 
through an app, removing the requirements of a cash register. 
Electronic transactions can be done with or without the presence of a designated point of sale.
Alice wants to buy a dress, from a store which is registered with her bank and has a trusted 
location device, using her secure cash app. She opens the application and scans/takes a picture 
of the bar-code of the dress and sends it to her bank using the pre-installed trusted location device 
in the shop. Alice's phone performs the three-way handshake using the trusted location device at the
shop with the bank. The bank authenticates the location and evaluates the trust level of Alice and 
sends a receipt to the shop indicating that the transaction has been taken place.

Another important scenario using secure cash can be the cash receipt system and it can be useful in places
where banks/ATM/credit card transactions are not widely accessible. Alice who wants to transfer money to
Bob's account; uses the secure cash application to do so; signs a cheque and sends it to Bob after 
completing a secure key exchange handshake. Bob on receiving the cheque goes to the bank where it gets
scanned and receives the money.

\subsubsection{Safe and Secure Virtual Identity}
Documents like passport, SSN, driver's license, property documents etc are very sensitive and need to be
kept at a safe location at all times. Applications can be built on top of DSMI that can encrypt these files
and send them to the trusted intended party or user without physically sending the documents. Using DSMI 
would help the sending and the receiving party be sure that the document is actually received from the
actual owner and is received by the intended user.


\subsection{Evaluation}

We wanted to test how long it takes for a user to complete the key
exchange handshake as it involves exchanging multiple text messaging.
The results depends on the network used for sure. Our tests were
conducted in Abu Dhabi, UAE using Etisalat \cite{etisalat} as our 
telecommunications services provider. 
We used java's function for time calculation to get time in nanoseconds.
We recorded the current time in nanoseconds. We used two ways to get the time: the phone
is linked with a PC via bluetooth and both phones signals the PC to record the
time (to get time of one machine) and for more accuracy we used the phones
to record their times themselves (to account for any delays caused while
transmitting the messages via bluetooth).
Time 1a is the time required to start the transaction by phone A and when phone
B replies back with its own data. Time 1b is the time recorded from the moment
phone B sends back its own data until it receives the challenge reply by A.
Both these times: Time 1a and Time 2a are taken by the PC connected via
bluetooth to both phones.
Time 1b and 2b is the same time as Time 1a and 2a, the difference is the
way the time is recorded. 1b and 2b are recorded on phone A and phone B
themselves.
Time a is the time required by phone A to send data to phone B. It is calculated
by getting the time in nanoseconds when user using phone A clicks send; phone
A sends an alert to PC to record the current time via bluetooth. Phone B when
receives the message sends an alert to PC to record the current time.
\\Time b is the time recorded when phone B sends its own data to A and the time
A receives it. Time c is the time required when A sends the challenge reply to
phone B and B receives it.

\subsubsection{Observations and Results}

We used a PC for recording the time when the phone sends a signal using bluetooth. 
We also used phones themselves to record the time. Using another device, in our case
the PC, for recording time can cause delays and by using two different devices for
recording time can create the difference in time. Figure \ref{timeDif} shows the difference
in times. Time 1 is the time taken by phone A to send meta-data to phone B 
and phone B replies back with encrypted challenge reply and its own metadata to phone A.
Time 2 is the time taken by phone B to send the encrypted challenge reply and its 
own metadata to phone A and phone A replies with the challenge reply. This figure shows that
the difference between the two is not very significant and we can use the average number to 
add into the results for an approximate time calculation.


\begin{figure}[htb]
    \centering
		\subfigure[{\smallTime difference for time 1: time taken by phone A to send meta-data to phone B and gets back a response}]
		{
				\includegraphics[width=0.45\columnwidth]
				{C:/Users/fa45/Dropbox/secmobid/tex/analysis/DiffTime1.jpg}
    }
		\subfigure[{\small Time difference for time 2: time taken by phone B to send the encrypted challenge reply and its 
own metadata to phone A and gets back a response}]
		{
				\includegraphics[width=0.45\columnwidth]
				{C:/Users/fa45/Dropbox/secmobid/tex/analysis/DiffTime2.jpg}
        
		}
		\caption{The time difference recorded}
		\label{timeDif}
\end{figure}


We measure the total amount of time needed to complete the 3-way key exchange
handshake by all paths.
Figure \ref{ttime} shows the timing analysis. According to this figure, for the
SMS the maximum time taken in all the tests was approximately 120seconds and the
minimum time taken was approximately 70seconds. The average is approximately 95seconds.
This means on average a user has to wait for up to 95seconds to start the exchanging
the messages with the intended user.

\begin{comment}

\begin{figure}[htb]
    \center{\includegraphics[width=2in]
        {C:/Users/fa45/Dropbox/secmobid/tex/analysis/totalTimeTaken.jpg}}
    \caption{\label{ttime} Total time taken for 3-way key exchange}
\end{figure}


\begin{figure}[htb]
    \center{\includegraphics[width=2in]
        {C:/Users/fa45/Dropbox/secmobid/tex/analysis/TIMEabc.jpg}}
    \caption{\label{timeabc} Time a-SMS path, Time b-data/SMS path and Time c-bluetooth/SMS path}
\end{figure}


\begin{figure}[htb]
    \centering
		\subfigure[{\small Total time taken for 3-way key exchange}]
		{
				\includegraphics[width=0.45\columnwidth]
				{C:/Users/fa45/Dropbox/secmobid/tex/analysis/totalTimeTaken.jpg}
    }\label{ttime}
		\subfigure[{\small Time a-SMS path, Time b-data/SMS path and Time c-bluetooth/SMS path}]
		{
				\includegraphics[width=0.45\columnwidth]
				{C:/Users/fa45/Dropbox/secmobid/tex/analysis/TIMEabc.jpg}
        
		}\label{timeabc}
\end{figure}
\end{comment}

Figure \ref{timeabc} shows time taken by all path. Time taken by data/SMS path is the most and depends on the
upload and download speed as well the time taken by the cellular service provider for receiving
and sending an SMS.


\begin{figure}[ht]
	\begin{minipage}[b]{0.45\linewidth}
		\centering
			\includegraphics[width=\textwidth]{C:/Users/fa45/Dropbox/secmobid/tex/analysis/totalTimeTaken.jpg}
			\caption{{\small Total time taken for 3-way key exchange}}
			\label{ttime}
	\end{minipage}
	\hspace{0.5cm}
	\begin{minipage}[b]{0.45\linewidth}
		\centering
			\includegraphics[width=\textwidth]{C:/Users/fa45/Dropbox/secmobid/tex/analysis/TIMEabc.jpg}
			\caption{{\small Time a-SMS path, Time b-data/SMS path and Time c-bluetooth/SMS path}}
			\label{timeabc}
	\end{minipage}
\end{figure}





==> Old Draft/flow.tex <==
1, Introduction

No good solution for mobile security
Too much trust on the cellular base station
Attacks are for real

Secure Mobile Identities problem
Key Contributions
Key Ideas

Implementation and Eval results



2. Threat Model and Security Overview

Assumptions
Phone is trusted
The Real Cellular Network is not an adversary

Threat
Fake base stations
Man in the Middle Attackers
Channel eavesdropping and jammers


3. Related Work


4. One-way Probabilistic Secure Cellular Channels

Cellular Voice and SMS channel
Under what assumptions does it give the One-way probabilistic secure channel
abstraction.



5. Single Path Spatiotemporal Repetitive Key Exchange Protocol

3-way handshake over SMS channel alone

How to measure reputations after repetitive exchange?

Security guarantees of the protocol under the probabilistic security guarantee?

Detecting an attacker? - adding a repetitive checking protocol (did you actually exchange keys with me?)



6. Multi-Path Spatiotemporal Repetitive Key Exchange

The IP path (Scenario 1b)

The Bluetooth path (Scenario 3 - physical handshake)

Reputation computation

Security guarantees




7. Trusted Locations

Trusted Cell towers 

Trusted GPS 

Google Wallet Model

The Trusted IP model?

Security guarantees in the face of non-forgeable locations




8. Trusted Fingerprints

User fingerprint based exchange?

Device Fingerprint based exchange?


9. Implementation


10. Evaluation



11. Conclusions


==> Old Draft/implementation.tex <==
\section{Implementation}

Android was selected as our target operating system primarily because of the availability and cost of the android phones. We used the android 
SDK for Eclipse as our development environment which we downloaded from the official android website. For implementation we used two Samsung 
Galaxy Young (GT-S5360) phones having Android version 2.3.6 installed on them. For implementing the Bluetooth part we downloaded the BlueCove
 Java library from the BlueCove website.
\\Android crypto library was used for RSA encryption. The RSA keys used are 2048-bit long; we chose this key size for security purposes. 
A 2048-bit long RSA key can encrypt 215-bytes of data; which is roughly the size of data we want to encrypt. We generate a random, 128-bytes 
long nonce in our implementation for maximum security purposes. The phone stores the RSA keys generated for itself in the 
Android's shared preferences for the app. Shared Preferences in Android are stored as a file within the application's 
data directory with file permissions set that allow only that application to access it. For the rest of data that we 
want to store goes into a SQLite database for storing public keys of other phones and messages. Metadata used in all the 
interactions is the phone number location and the current time of the phone that is generating the metadata. The time includes 
the seconds, hours, date, month and year. 
\\All the messages, we receive and through whatever channel we are sending it through, have a specific header that helps the application 
in determining what to do with it. In our application we have a SMS receiver class that checks whether the SMS is supposed to be 
processed by our application; our protocol SMS; or is it just a regular SMS. If it is the SMS that our application needs to process then we do not let the SMS go to the Android phone's default application for receiving SMS; thus making sure that the SMS used for our application remains private. If it 
is a regular SMS then the application discards it and sends to the Android phone's default SMS application. SMS in our 
application are used for the following purposes: sending metadata, location and key; sending challenges and sending signed challenge replies.
Bluetooth channel works in pretty much the same way as the SMS channel but it has an added security feature 
of providing a password before starting key-exchange. The signed verification is not sent through the Bluetooth channel instead it is 
sent through SMS.
\\The signed verification in our data path is also sent through SMS. The phones connect to our server 
to send and receive messages. One phone uploads the message with a randomly generated, 128-byte long nonce on the server and 
sends the nonce to the other phone via SMS.


\begin{comment}
\\ Figure \ref{sms} shows how SMS are being exchanged between two phones A and B. A generates metadata and nonce and stores them in 
its database for verification later. It then sends them and its public key to B via SMS. B when receives the text message 
containing this information stores the public key of A in its database. It signs the metadata and nonce of A using its 
private key and generates its own metadata and nonce and sends it to A including its public key. 

\begin{figure}[htb]
    \center{\includegraphics[width=3in]
        {C:/Users/fa45/Dropbox/secmobid/tex/SMS.jpg}}
    \caption{\label{sms} SMS exchange between two phones: A and B}
\end{figure}
			
			
When A receives this reply, it fetches the metadata and nonce it generated before sending the message to B from the database, 
decrypts the challenge using B's public key and compares the two. If they are equal it stores B's public key, B's location and 
the path it used to send i.e. SMS in its database. It then signs the metadata and nonce sent by B using its private key and then 
sends this to B. B fetches: the public key of A to decrypt the challenge, the metadata and nonce it generated before sending them 
to A and compares the two. If the two are the same it stores them in its database. 

\begin{figure}[htb]
    \center{\includegraphics[width=3in]
        {C:/Users/fa45/Dropbox/secmobid/tex/Bluetooth.jpg}}
    \caption{\label{bluetooth} Message exchange between two phones: A and B; using Bluetooth (in blue) and SMS (in orange)}
\end{figure}

\\ Figure \ref{bluetooth} shows the exchange of messages using an alternate path: Bluetooth. When A wants to send a message to B using Bluetooth 
it enters a password which should also be known to B. If both passwords match then the following happens. A generates and stores metadata
 and nonce and sends it via Bluetooth to B. B receives it, generates and stores its own metadata and nonce and save it along with the public
 key of A. B sends metadata and nonce it generated to A via Bluetooth and it signs metadata and nonce of A and sends it using SMS channel.
 A gets the metadata and nonce and the message containing and verifies it. If the match it sends an SMS to B containing signed metadata 
and nonce of B.

\begin{figure}[htb]
    \center{\includegraphics[width=3in]
        {C:/Users/fa45/Dropbox/secmobid/tex/Data.jpg}}
    \caption{\label{data} Message exchange between two phones: A and B; using data}
\end{figure}
	

\\ Figure \ref{data} shows how we are sending messages from A to B. The basic protocol is the same. A generates and stores the metadata and the 
nonce. It creates another nonce and stores the message with a reference to the new nonce and sends an SMS to B to fetch the message using 
the new nonce. B fetches the messages from the server and the server deletes the message. Then B signs the metadata and nonce sent by A 
and sends it using SMS. Then B generates its own metadata and nonce and sends it to A in the same way.
The metadata includes the location of the phone. In order to get a certifying location the phone connects to one of 
the certifying Bluetooth device and gets a certifying location in return. The phone and the certifying Bluetooth device 
know a key. The certifying Bluetooth device sends its own public key, location and time to live signed with the known key to the device.
\end{comment}


==> Old Draft/intro-new.tex <==
\section{Introduction}

Security loopholes exists due to vulnerabilities in the network which puts 
the users at risk to attackers~\cite{securityVul}\cite{securityVul2}. A recent advancement 
in attacks on Global System for Mobile Communications (GSM) security has shown that
anybody with some skill can use the techniques and hardware 
to eavesdrop or record GSM cell phone calls~\cite{PerezAttack}.
Security issues range from man-in-the-middle (MITM)
attacks such as snooping, eavesdropping on phone calls and text
messages, to jamming the channel to block access to secure session
thereby causing disruption in the service. 
While SSL/TLS~\cite{oppliger2008ssl} is used in secure web transactions, most of the
transactions in the mobile world is through apps. Researchers have
noted that SSL is not always enabled in apps and there is no easy way to
check whether the traffic between the mobile app and the server is
encrypted~\cite{SSL/TLSVul}. Due to these issues it is
hard to conduct reliable secure transactions between users.

There have been efforts to enhance the security of mobile
devices. Apps such as Lookout Security \cite{lookoutSecurity} and others use PINs and
passwords to conduct transactions. But their security models and
processes do not depend on the identity of the person involved in the
transaction. If the password or PIN is stolen then the so called
secure wallet is exposed to the attackers. There have been efforts by
few companies to provide one-time PIN authentication which gives the
user the ability to input a one-time PIN before opening the
application or conducting a transaction~\cite{haller1995s};
and two-factor authentication~\cite{financial2007two}\cite{lakshmiraghavan2013two},
which allows users to authenticate using the debit cards and the pin. 
But since the PIN is a one
time solution and there is no guarantee that the PIN reached the user
or not, the security of this model can be compromised. 

%The design of DSMI places initial
%bootstrap trust on the cellular providers and builds upon the basic
%assumption that cellular networks offer a unique ``partially
%trustworthy one-way'' channel to connected mobile devices; unlike
%Internet routes which can be hijacked, the cellular network routing
%layer is closed thereby forcing the MITM attacker to attack only the
%last-hop wireless channel between the tower and the device.

In this paper we introduce a new protocol; Secure Mobile Identities (DSMI); 
to provide reliable identities
of the user thereby enabling secure transactions. DSMI guarantees that the user is
communicating only with the intended users.
DSMI is built over the trusted security layer provided by the cellular network. We assume that it is a
`partial trustworthy' channel as a user gets authenticated by the cell tower and once the user
is on the network, he/she will always get messages sent to them.
In our solution, we generate a secure mobile identity of a user and share it
to other users via different paths. Third party solutions like 
SSL/TLS~\cite{oppliger2008ssl}, used in secure web transactions requires all
web services to go through the certification authority to validate the credentials.
The identity assigned to each device and its
authentication is done using a decentralized approach in our protocol.

DSMI uses multiple paths for exchanging keys and
verification. The idea behind this is that if a certain path is compromised, 
the verification is always done via SMS based on our trust assumption. The probability of both channels being 
compromised is very low. DSMI maintains a list of users with their keys along
with their location and time. It creates different levels of trust depending
on how reliable the location information is and from how many different paths
the user has tried to contact the intended user. Using multiple paths has been
proposed to be a better authentication scheme
\cite{bauckman2013multi}\cite{abdurrahman2013new}\cite{dispensa2007multi}\cite{weber2010multi}.

DSMI is a repetitive spatio-temporal key exchange method. The users exchange
their keys across various location at different times. By repetitively exchanging keys
over different locations-the users develop trust or a strong identity. DSMI maintains a {\textit{trust score}}
against each user. The higher the score is the stronger the identity is.
Since location can be tapered in a variety of ways~\cite{GPSTemper}\cite{bland2008gps} and that would weaken our protocol; DSMI
introduces other methods for secure location. One idea is using a trusted location sync interface like
Google wallet~\cite{googleWallet} or using geolocation~\cite{katz2006towards}. By syncing with the Google wallet device, the mobile can get a certifying location of 
the wallet or the user can map his/her IP addresses to the geographical location and that would earn more trust score for the user.

Many applications can be developed on top of DSMI and many existing applications can extend DSMI
using it as the security layer. Applications
as data sensitive as mobile banking can be built leveraging DSMI. It can particularly be useful in
places where access to banks is not easy. Other applications
involving private photo exchange and file exchange can be built using DSMI.

We implemented the android version of DSMI. It is a very user friendly in a way
that only requires the user to enter the number of the intended user, rest of
the work is done in the background without any user involvement, which
makes this application very trivial to use. Secure
Mobile Identities is not platform specific which makes it even more diverse and scalable.


\begin{comment}
DSMI does not require third party solutions and it is built on minimum trust assumptions.
SSL/TLS~\cite{oppliger2008ssl}, used in secure web transactions requires all
web services to go through the certification authority to validate the credentials.
The identity assigned to each device and its
authentication is done using a decentralized approach in our protocol.
DSMI is built over the trusted layer provided by the cellular network. We assume that it is an
almost reliable delivery path in a way that the text messages are always delivered to the
intended recipient and the cellular network is trusted.


Users regularly face a problem of mobile security which is why they suffer of 
crisis of confidence. Recent reports suggests that due to vulnerabilities in the network, 
security loopholes exist which puts the users at risk to
attackers~\cite{securityVul}\cite{securityVul2}. The users doubt whether the message is actually sent by
the claimed person or if their conversation is being eavesdropped. A recent advancement 
in attacks on Global System for Mobile Communications (GSM) security has shown that it 
is now trivial to intercept or record GSM cell phone calls. Anybody with some skill can 
use the techniques and hardware described by Chris Paget~\cite{PerezAttack} to eavesdrop or 
record GSM cell phone calls.
\end{comment}

==> Old Draft/intro.tex <==
\section{Introduction}

Users regularly face a problem of mobile security which is why they suffer of 
crisis of confidence. Recent reports suggests that due to vulnerabilities in the network, 
security loopholes exist which puts the users at risk to
attackers. The users doubt whether the message is actually sent by
the claimed person or if their conversation is being eavesdropped. A recent advancement 
in attacks on Global System for Mobile Communications (GSM) security has shown that it 
is now trivial to intercept or record GSM cell phone calls. Anybody with some skill can 
use the techniques and hardware described by Chris Paget \cite{PerezAttack} to eavesdrop or 
record GSM cell phone calls.

\\Security issues range from man-in-the-middle (MITM)
attacks such as snooping, eavesdropping on phone calls and text
messages, to jamming the channel to block access to secure session
thereby causing disruption in the service. 
While SSL/TLS is used in secure web transactions, most of the
transactions in the mobile world is through apps. Researchers have
noted that SSL is not always enabled in apps and there is no easy way to
check whether the traffic between your mobile app and the server is
encrypted. Due to these issues it is
hard to conduct reliable secure transactions between users. Since the
communication channel is insecure, there is no good solution which a
service (or service provider) could use in which the identity of the
user is guaranteed. This mobile 
security issue is a major problem and because of this there hasn't
been any reliable way to conduct secure transactions where the mobile
device and user's identity is guaranteed to be genuine. 


\\In this paper we introduce new protocols to provide reliable identity
of the user thereby enabling secure transactions. We provide protocols
that enable two or more parties to transaction in a secure manner,
where with high probability each party is guaranteed that it is
communicating with other genuine parties. A number of applications can be built on
top of these protocols that enable secure transfer of messages, secure
transfer of funds. mobile payments etc.  

There have been efforts to increase the security of mobile
devices. Apps such as Lookout Security \cite{lookoutSecurity} and others use PINs and
passwords to conduct transactions. But their security models and
processes does not depend on the identity of the person involved in the
transaction. If the password or PIN is stolen then the so called
secure wallet is exposed to the attackers. There have been efforts by
few companies to provide two-factor authentication, which gives the
user the ability to input a one-time PIN before opening the
application or conducting a transaction. But since the PIN is a one
time solution and there is no guarantee that the PIN reached the user
or not, the security of this model can be compromised. 

\\In our solution we use self certifying keys which are exchanged by the
users in addition to their location and identity information in a
specific manner providing a much stronger security guarantee than the
earlier efforts in the area. DSMI uses multiple paths for exchanging keys and
verification. The idea behind this is that if a certain path is compromised, 
the verification is always done via SMS. The probability of both channels being 
compromised is very low. DSMI maintains a list of users with their keys along
with their location and time. It creates different levels of trust depending
on how reliable the location information is and from how many different paths
the user has tried to contact the intended user.

\\We implemented the android version of DSMI. It is a very user friendly in a way
that only requires the user to enter the number of the intended user, rest of
the work is done in the background without any user involvement, which
makes this application very trivial to use. Closely related work includes
SafeSlinger \cite{safeslinger} which requires the users to be present; physically
or virtually; with each other at the same time as the keys are being exchanged. Secure
Mobile Identity is not platform specific which makes it even more diverse and scalable.

\\The organization of this paper is as follows: In section 2 we will describe the problem
definition and threat model. In section 3 we discuss some of the closely related work and
how DSMI is different that them. We give the overall general setup in section 4. ...






==> Old Draft/location.tex <==
\section{Identifying location}

In this section, we try to answer the following question: can we
correctly identify the physical location of a cellphone? Either using
the location information from the cell towers or GPS information
present on the phone, nearby Wifi signals etc. 

Nowadays, Android and other mobile operating systems use various
techniques for pin pointing the location of the cellphone. 


\section{Techniques}


==> Old Draft/protocol.tex <==
\section{Protocol}

\begin{itemize}
\item GSM security is broken. Therefore, we need end-to-end security
mechanism to make sure that mobile banking and other security
applications implemented on top of GSM are always secure.
\item We plan to develop a protocol that satisfies certain security
  guarantees.
\item The central question is: how do you establish a secure
  communication channel between two mobile devices?
\end{itemize}

\subsection{Outline}
The device is associated with a username, a cellphone number, a set of
keys, a GPS location, cellular base station connection information,
set of self-certifying signatures and challenge-response signatures.
Let,  U - username, N - Mobile number, L - Location, P - Self
certifying key, c - challenge-response signature. 
Let $U_A,N_A,L_A,P_A, c_A$ be the properties of mobile device A and $U_B,
N_B, L_B, P_B, c_B$ are the properties of mobile device B.

The outline of the 3-way handshake protocol is as follows. 

\begin{align*}
 \textbf{1}.& \quad  D_A\rightarrow D_B: & & sign(M_A) \\
           .& \quad : & & \text{where}, M_A = (U_A, N_A, L_A, P_A, c_A)\\
 \textbf{2}.& \quad D_B \rightarrow D_A: & & sign(M_B), sign(c_A) \\
	   .& \quad : & & \text{where}, M_B = (U_B, N_B, L_B, P_B,
           c_B)\\
\textbf{3}.& \quad D_A \rightarrow D_B: & & sign(c_B)
\end{align*}

\textbf{1.} Device $D_A$ encrypts or signs message $M_A$ which
consists of $U_A, N_B, L_B, P_B, c_A$, using its key and sends it to
device $D_B$. 

\textbf{2.} Device $D_B$ signs $M_B$ which consists of $U_B, N_B, L_B,
P_B, c_B$, signs $c_A$ and sends it to $D_A$.

\textbf{3.} Device $D_A$ signs $c_B$ and sends it to $D_B$.

Repeat the 3-way handshake protocol across different $L_i$ (locations), at
different points in time. If $P_A$, $P_B$ are consistent after
repetitions, then both $D_A$ and $D_B$ have higher confidence that
they are talking to each other. This type of asynchronous method of
device pairing would help in thwarting some of the security flaws in
the underlying GSM channel.


\cite{Lin09spate}

==> Old Draft/protocols.tex <==
\section{Single path spatio-temporal key exchange}

In this protocol, only SMS is used to exchange keys between the
users. The location information is not trusted, hence the protocol has
a repetitive procedure. Initially keys are exchanged using a simple
3-way handshake protocol where each user generates a self certifying
key. Once the initial 3-way protocol is completed, a reputation score
is maintained by each user. This score is increased based on the
location information obtained from the cell 
towers and the GPS. The assumption here is
the attacker will not follow the user at all times. So if the
adversary was impersonating the user a few times, his location will be
very different from the actual user's location. As the keys are
repetitively exchanged at different intervals of time the location
information is updated. As the user location behavior follows a
specific pattern repeatedly, the reputation score is increased. Same
set of keys are exchanged at different intervals and from different 
locations, where the locations follow a pattern. If the same set of
keys are exchanged from a location that does not follow the
established pattern, then the reputation score is reduced. Else it is
increased. When the reputation score reached a certain threshold the
keys are assumed to be genuine. 

\subsection*{Preliminaries}
\begin{itemize}
\item  Every mobile device is allocated a unique identity $D_1$
(either a phone number or IMSI number)
\item User $U_1$ registers with provider a $X_1$ using a device $W_1$
  with a unique identity $D_1$ 
\item If $W_1$ is directly connected to an authorized base station of
  provider $X_1$, then anyone who sends a message to identity $D_1$ is
  routed to $W_1$ and is received by user $U_1$.
%\item The routing layer within the cellular network is trusted
\end{itemize}




The step by step protocol is described as follows.

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1,c1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2,c2)S_2,c1 \\
 \textbf{3}.& \quad U_1 \rightarrow U_2: & & (c2)S_1 \\
 \textbf{4}.& \quad U_1: & & (D_2, P_2) ~\text{verify with} (L_1,L_2,t) ~\text{n
 times} \\
 \textbf{5}.& \quad U_1: & & (U_2, D_2, P_2) ~\text{usable if verified n times}
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] User $U_1$ generates a self certifying key $P_1$ and
  signs the message consisting of location data $L_1$, time $t$,
  username $U_1$, user identity $D_1$ and challenge nonce $c1$. Here
  $L_1$ is the location data which might be the location of the cell
  tower combined with the GPS coordinates. $U_1$ sends the signed
  message $(L_1,t,U_1,D_1,c1)S_1$ and $P_1$ to $U_2$.

\item[\textbf{2.}] User $U_2$ generates a self certifying key $P_2$ and
  decrypts the message using the key $P_1$ sent in the message. $U_2$
  then signs the message consisting his location data $L_2$, time $t$,
  username $U_2$, user identity $D_2$ and reverse challenge nonce $c2$. User
  $U_2$ sends key $P_2$, challenge nonce $c1$ and signed message
  $(L_2,t,U_2,D_2,c2)S_2$ to $U_1$.

\item[\textbf{3.}] User $U_1$ decrypts message and sends the signed
  reverse challenge nonce $c2$ back to $U_2$. This completes the
  three-way handshake protocol.

\item[\textbf{4.}] $U_1$ stores $(D_2, P_2)$ and its corresponding
  location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. We have to repeat the protocol $n$ times because
  the location information is untrusted. The rationale here is, an
  attacker might try to spoof the identity of $U_2$ once or twice, but
  repeatedly ($n$ times) masquerading the identity of $U_2$ is
  hard. So by repeating the protocol $n$ times, preferably from
  different locations, increases the chances of the user being $U_2$. 

\item[\textbf{5.}] If after $n$ times $(D_2, P_2)$ corresponds to
  $(L_1,L_2,t)$ then with high probability $U_1$ has established a
  secure connection with $U_2$.
\end{enumerate}


\subsubsection{Security Analysis}

In Step 1, $U_1$ generates a self certifying key $P_1$, signs the
message which contains the location data $L_1$, time $t$,
  username $U_1$, user identity $D_1$ and challenge nonce $c1$, and
  sends the message and $P_1$ to the other user $U_2$. As we discussed
  in the previous Section, the cellular network is one-way
  probabilistically secure. An adversary can spoof the cellphone
  number of $U_1$ and hijack the message. But if $U_2$ is present in
  the cellular network $U_2$ would also receive the message, since the
  message is being routed to $U_2$'s number. The adversary could
  create a fake base station within $U_2$'s vicinity and hijack the
  message. In this case $U_2$ would never receive the message. The
  adversary could continue the entire protocol with $U_1$. But this is
  a highly unlikely event due to the following reasons. i) the
  adversary has to be in the vicinity of $U_2$ at the exact moment
  when the message is sent to by $U_1$ to $U_2$. ii) during the entire
  course of the protocol the $U_2$'s cellphone has be switched off, so
  that $U_2$ can't join the network. If $U_2$ joins the network during
  the course of the protocol, $U_2$ would get an encrypted message
  from $U_1$ with no key to decrypt. This would alert $U_2$ about the
  MITM attack and $U_2$ could send a message to $U_1$ to abort the
  protocol. $U_1$ would receive messages from two different locations
  and because of this $U_1$ would abort the protocol. Another scenario
  is $U_2$ would switch on the phone during the repetitive location
  exchange step. This would again give $U_1$ different or
  inconsistent location information and $U_1$ would abort the protocol. 

In Step 2, $U_2$ first checks if the message sent by $U_1$ is
consistent. If not, it aborts the protocol. If the message is
consistent, $U_2$ generates its self
certifying keys and signs the message containing its location data
$L_2$, time $t$, username $U_2$, user identity $D_2$ and reverse
challenge nonce $c2$.  An adversary could spoof $U_1$'s message. So
$U_2$ does not have any guarantee that the message was indeed sent by
$U_1$. Only in step 5 of the protocol when the reputation score goes
above a certain threshold, $U_2$ would have established a secure key
exchange with $U_1$.

In Step 3, $U_1$ checks if the message sent by $U_2$ is consistent. If
not, $U_1$ aborts the protocol. Else, $U_1$ will sign a reverse
challenge response $c_2$ and send it to $U_2$.

{\em Reputation score:} In Step 4, $U_1$ stores $(D_2, P_2)$ and its
corresponding location information and time $(L_1,L_2,t)$. $U_1$ verifies the
  whether ($D_2, P_2)$ corresponds to $(L_1,L_2,t)$ by repeating the
  protocol $n$ times. Similarly, $U_2$ stores the $(D_1, P_1)$ and its
  corresponding location information and time $(L_1, L_2)$. In this
  step, the keys are exchanged $n$ times. Each time if the location
  and time information are consistent then the reputation score is
  increased by 1. If the time to send or receive the message is
  greater than a certain time $T$, then the reputation score is reset
  to zero and Step 4 is started again. An adversary could spoof the
  location and time message by performing a MITM attack, but since the
  step is performed $n$ at different locations and time periods, the
  adversary would not be able to modify the message such that either
  $U_1$ or $U_2$ would always get consistent location and time
  information. Also, if the message is inconsistent $k$ times, then
  the protocol is aborted. When the reputation score
  passes $n$, then $U_1$ and $U_2$ have exchanged keys with high
  probability. 


\subsection{Two: Trusted location data}

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1,c1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2,c2)S_2,c1 \\
 \textbf{3}.& \quad U_1 \rightarrow U_2: & & (c2)S_1 \\
\end{align*}

In this protocol, the location data ($L_1,L_2,t)$ is from a trusted
source. The GPS chip within the mobile devices $W_1,W_2$ are trusted
and the cell tower information obtained is also trusted. Hence the
protocol boils down to the three-way handshake protocol. 


\subsection{Three: Trusted point of sale device}

\subsection*{Assumptions}
\begin{itemize}
\item Point of sale devices are trusted. 
\item Point of sale devices have the ability to sign a message and
  transmit the message securely to the device $W_1$ of the user $U_1$.
\end{itemize}

\subsubsection{Protocol}

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow G: & & P_1,L_1,t,U_1,D_1  \\
 \textbf{2}.& \quad G \rightarrow U_1: & & G_P, (P_1,L_1,t,U_1,D_1)G_S \\
 \textbf{3}.& \quad U_1 \rightarrow C: & & P_1, (G_P,(P_1,L_1,t,U_1,D_1)G_S)S_1 \\
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] $U_1$ sends the message $P_1,L_1,t,U_1,D_1$ to a
  point of sale device $G$. 

\item[\textbf{2.}] A point of sale device can be a NFC
  device or other device which is capable to signing a message. The
  point of sale device $G$ signs the message $(P_1,L_1,t,U_1,D_1)G_S$
  and along with $G_P$ (public key) sends it back to $U_1$.

\item[\textbf{3.}] Now $U_1$ signs the message it received from $G$,

  ($P_1$,$L_1$,$t$,$U_1$,$D_1$)$G_S$)$S_1$ and sends it to the central
  authority $C$ along with $P_1$. Since $G$ is trusted (has trusted
  credentials), $C$ is certain that the message is signed by $G$ and
  that $U_1$ was indeed present at the point of sale location. The
  point of sale device could also have a fingerprint reader (or any
  biometric device) to authenticate user's identity and the biometric
  data can also be part of the signed message from $G$ to $U_1$. 
\end{enumerate}



==> Old Draft/relatedWork.tex <==
\section{Related work}

% physical encounter,
% Short Authentic Strings (SAS)
% count no of participants

Closely related work by Farb, Lin, Kim, McCune and Perrig \cite{safeslinger}, provides a system, 
named SafeSlinger, that leverages physical encounter to establish digital trust that is exchange 
keys with one another. Our system on the other hand does not require any kind of physical encounter 
with the person the user wants to exchange information to. However, SafeSlinger does allow establishing
digital trust by having a common acquaintance to facilitate a mutual introduction. 
In addition to this SafeSlinger \cite{safeslinger} asks the users to compare a 3-word phrase(encoded 24-bit hash value)
for verification and to minimize attacks. Groupthink \cite{groupthink} like SafeSlinger \cite{safeslinger} requires 
users to count the number of participants and requires users to verify Short Authentic Strings (SAS)
Secure mobile identities, like Safeslinger \cite{safeslinger}, does all the cryptographic steps in the background; but in DSMI, 
the user only enters the number of the user similar to what they do while sending a traditional SMS or MMS. Secure mobile identities
protocol requires physical proximity only in case of bluetooth exchange of messages and/or trusted location.

%multi-path

Secure location sharing system(SLS) by Adams and Lee \cite{sls}, uses similar approach as DSMI in a way
that they use multi-path approach for exchanging keys. Unlike Secure mobile identities, SLS requires the users have previously communicated
via some other channel and that channel will be used for verification. For further verification(someone other than the intended user
is using the channel) the user generates a secret question which has to be answered correctly by the intended user.

%server + visual encounter

DSMILE \cite{DSMILE} establishes trust between individuals who shared an encounter and they must provide a proof of that encounter.
The user broadcasts the encounter key to other devices within its communication range and then uploads a cryptographically secure hash
of they key along with a message encrypted by the encounter key to a server. The intended users claim the encounter by looking up
the hash of the key at the server.
Meetup \cite{meetup} similar to DSMILE \cite{DSMILE}, requires a visual authentication scheme which is a digital certificate signed by a 
trusted authority but they have to be at the encounter site. DSMI does not require a server and a visual authentication.

% public authentication

PGP Key signing parties \cite{keySigningParty} use people to verify that the public key is authentic. The larger the number of verification,
the more authentic the key is which is similar to our scoring mechanism except that DSMI uses location and path for scoring while PGP Key signing 
parties uses manual user authentication.

% a hub to pass info

GAnGS \cite{GANGS} exchanges group members' public keys such that each group member obtains the authentic public key of every member. 
It involves three phases: collection, distribution and identification. GAnGS need an untrusted projector or a phone as a hub to pass
information. This is too cumbersome to use because of so many operations to perform by a user.
SPATE \cite{SPATE} relies on visual channels and physical interactions. Like GAnGS \cite{GANGS}, SPATE requires a number of steps, 
visual hash function verification, leader selection, giving away personal information to bystanders. 

There is a proliferation of WiFi gadgets and sensors that do not have to protect against MITM attacks as the key exchange messages are 
not authenticated in any wayas it require devices to support an out-of-band communication channel. \cite{gollakota2011secure} presents 
tamper-evident pairing (TEP), a protocol that provides simple, secure WiFi pairing and protects against MITM attacks without an out-of-band
channel. DSMI is only built for phones or for devices capable of sending an SMS.


==> Old Draft/threat.tex <==
\section{Problem definition and threat model}

In this section we give the problem definition and threat model of the system and also
present an overview of the security properties. 

\subsection{Problem definition}

The current
state of security in the mobile ecosystem is either broken or have
severe vulnerabilities. We want to have a very secure and reliable communicating channel. 
We want to be absolutely certain that we are communicating only with the desired person and not to an intruder and that the conversation is not being intercepted by an imposter. This security and reliability is absolutely vital when 
two users or a user and the system wants to reveal their secret and/or sensitive information such as 
PIN codes or credit card numbers etc; without which data like this can fall in wrong hands and can be misused. In this age of technology; where people are always looking for ways to minimize time; they need a way to communicate securely in ways other than do it in person.
The problem we are trying to address is the following. 

{\em User $U_1$ with a mobile device $D_1$ wants to securely
interact with another user $U_2$ with a mobile device $D_2$ or any
central authority $C$, through an untrusted communication channel.}

When we say securely interact or communicate we mean that we have information secrecy;
 the information is revealed only to the intended user. 
We will first start with the assumptions and goals of the systems and then move
on to the threat model. 


\subsection{Assumptions}
Our protocol requires that the users have a smartphone. First, we assume that the users know how to use a smartphone. We also assume that the user can read and understand the instructions in English and that the user wants security and does not deliberately disclose private information. As our protocol requires frequent SMS sending and receiving; we assume that the user has enough credit in his account for sending text messages. With respect to our Secure Mobile Identities protocol the basic assumptions of the system are as follows.
\begin{itemize}
\item {\em The cellular service is trusted}. We assume that the cellular service on top of which
DSMI is built is trusted. When a mobile device authenticates itself with a cellular base station,
we assume that the IMSI number, Ki (key) is secure and nobody can steal the identity
of the device.
\item {\em SMS is always delivered}. We assume that the messages we send are delivered to the 
	person intended and it does not get lost once the device is on the network is authenticated. 
	For example, Alice and Bob are exchanging keys and
	Alice has authenticated Bob and sends a verification message to Bob which also includes 
	information for her authentication. This messages fails to get delivered. In this case Alice's
	records would have Bob as the authenticated user but in Bob's records Alice isn't authenticated.
\item {\em The cellular service provider is trusted}. If the cellular service
  provider is malicious then he could intercept the transaction
  between the users, perform a DoS attack and render the protocol
  useless. Vulnerabilities can be inserted to the SIM card using OTA
  (Over-the-air) updates which would compromise any message or phone
  call on the phone. Since the possibility of a rouge service provider
  is a rare occurrence, we assume the service provider is trusted. 
\item {\em SMS is secure}. This assumption is based on our assumption of the
	cellular service provider being trusted. If the provider is not trusted and if 
	there	is an intruder who is keeping a tap of messages being exchanged then the verification
	step in our protocol becomes null and void. We assume that the SMS can only be sent and
	received by the	user who owns the SIM. For example, a malicious user may start a secure communication
	with Alice using the phone number of Bob. Alice thinks that she is talking to Bob because
	the number she is exchanging messages with is the same as Bob's.
\item {\em The mobile phone is trusted}. We make this assumption because if
  the phone is not trusted then PIN, secret keys and other secure
  information related to the user would be insecure. Since most of the
  cryptographic protocols rely on the user's key being secure, it is
  natural to assume that the phone is trusted and that the user's
  credentials on the phone are secure. This also means we assume that
  there are no rootkit attacks on the phone.
\item {\em The mobile phone is devoid of malware}. We assume that the software and
	hardware of the phone is not prone to attacks from a third party which can intercept
	the user's phone. This also includes the phone apps that can allow attacks like
	these.
\item {\em Error checking and aborting}. In case of errors or suspicions, users will restart the
	application. 
\end{itemize}


\subsection{Goals}

Our main goal is to allow two users to exchange sensitive information securely 
through insecure channels. The Secure Mobile Identities protocol aims to achieve the following
goals:
\begin{itemize}
	\item {\em Security}. We aim to provide a secure system that would not leak sensitive data
		that has to be communicated to the intended user.
	\item {\em Privacy}. Contact information, data and keys of a user are only available to the
		members of the interaction and remain hidden from intruders or malware.
	\item {\em Authenticity}. The users involved in the communication are authentic which means that
		the interaction is carried on by the intended users and no one else.
	\item {\em Reliability}. We aim to provide that reliability that the information being passed on
		is going to the right user under all circumstances. 
	\item {\em Usability}. We emphasize usability along with all our security properties.
	\item {\em Platform Independence}. Our system is not platform independent thus enabling interactions
		among smartphones of different manufactures.
\end{itemize}

Given the assumptions and goals, the threat model of the system can be described
as follows.

\subsection{Threat Model}

We are building a secure and trusted application over insecure and untrusted communication channel. This causes 
a threat to our security. Possible attacks to Secure mobile identities include:
\begin{itemize}
	\item {\em Man-in-the-Middle (MitM) attack}. If two users are communicating with each other an attacker
		can intercept their messages by controlling the wireless communication.
	\item {\em Message forgery}. It is also known as message spoofing. An attacker can deceive the user as to whom
		the real sender is. The user can share all the sensitive information to the attacker in this way.
	\item {\em Malicious user}. A fake user who initiates a communication link to another user.
	\item {\em Malicious server}. The server may be controlled by a malicious administrator. A compromised server
		can be a threat to our security.
	\item {\em Malicious app}. As our protocol is intended for a smartphone it is very likely that the user
		has a malicious app installed on the smartphone which is used for communication using Secure mobile identities
		protocol. That application may be able to read the private keys and/or read the messages.
	\item {\em Fake or compromised base station}. It is possible that an attacker has set up a fake base station
		that can intercept all the messages going on through it.
	
\end{itemize}

\subsection{Security guarantees}

Despite being exposed to various attacks, our protocol offers security guarantees. Our protocol
has uses multiple channels for its operation. If an attacker attacks one of the channels, for example
the server is compromised, the verification has to go through the SMS channel. It is very difficult for
an attacker to attack all three channels: bluetooth, server and SMS.
For protocols that rely on a back-hand server, it is possible that the server is controlled by a malacious
administrator. Our protocol removes the message in a matter of a few minutes from the server from
the time it gets uploaded. It does not 100\% success but it is better than leaving the information on
the server for longer time.



==> Old Draft/threat_model.tex <==
\section{Problem Setting}

In this section, we define the problem we set out to solve, discuss our assumptions, goals and also perform a review of the adversary we defend against and present attacks.

%\begin{comment}
%\subsection{Motivation}
%\label{sec:motiv}
%
%The fundamental limitation of the GSM security is the absence of an authentication scheme between subscriber and the Mobile Network Operator (MNO). This can be exploited by setting up an adversarial base station with appropriate hardware and software. We discuss two realistic threats against GSM security. 
%
%\textbf{\textbf{Connecting to an Adversarial BTS}}
%\begin{comment}
%%Do we need all of this?
%
%
%
%As part of a cellular network, a Base Transceiver Station (BTS) has equipment for the encryption and decryption of communication, spectrum filtering equipment, antennas and transceivers (TRX) to name a few. There are several situations in which the Mobile Station (MS) starts to look for a new BTS to connect to.
%\begin{itemize}
%\itemsep-0.23em 
%\item When the MS registers to the BTS of the network provider, the BTS sends a list containing the frequencies of nearby BTS stations belonging to the same MNO. Based on this information, the MS selects the BTS with the best signal strength. If none are found, it scans through standard frequencies to find an active BTS. To force the selection of a fake BTS, the attacker can exploit knowledge of the MS periodically measuring its connection strength with the nearest BTS. To ensure forced selection, the \textit{fake signal} is sent on the BTS frequency with the strongest signal. 
%
%\item The MS may find a BTS with a better signal. In this case the fake BTS sends signals on the frequency channel used by one of the BTSs which are near the MS. This is called \textit{forced BTS selection}. 
%
%\item The frequency channel used by MS to connect with its original BTS is jammed which leads the MS to search for a new BTS.
%\end{itemize}
%
%\textbf{\textbf{Man in the Middle (MITM) attack}}
%
%
%With the availability of software defined radios like USRP \cite{usrp}, sysmoBTS \cite{sysmobts}, Fairwaves \cite{fairwaves} and Opencell \cite{opencell} the attacks on the unsecure GSM network have become a reality. This has further been facilitated by the availability of OpenBTS \cite{openbts} and OpenBSC \cite{openbsc} like open source projects that help provide the software infrastructure to run a BTS. Meyer et al \cite{germany} show a MITM attack on Universal Mobile Telecommunications Systems (UMTS) by exploiting the lack of integrity protection in GSM base stations. Kostrzewa \cite{thesis} demonstrates exploit the weakness of A5/2 \cite{comp128} cipher to demonstrate MITM attack. 
%
%Two kinds of MITM attack can be employed with an adversarial BTS, henceforth referred to as the \textit{fake BTS}. In the first phase of both, the MS is tricked to connect to the fake BTS. 
%\begin{itemize}
%\itemsep-0.23em 
%\item In the first case, once the MS decides to choose a fake BTS, it sends its International Mobile Subscriber Identity (IMSI) to the fake BTS. The fake BTS then sends a fake authentication request containing a forged randomly generated number, RAND. The MS calculates the Signed Response (SRES) by encrypting RAND with A3 algorithm using the Root Key, $K_i$. The fake BTS authenticates the MS regardless of the SRES value received and then uses A5/0 for ciphering. It can now read all of the outgoing traffic from the MS and then send it over IP to cover the ongoing attack. The incoming traffic will be saved by the MNO as voice mails and delayed text messages.
%
%\item The second kind of attack is complex and requires decrypting traffic. This attack has been demonstrated in \cite{germany} and requires an alternate phone to connect to, henceforth reffered to as a \textit{fake phone}. After the MS has been lured to connect to the fake BTS, the attacker forwards the IMSI received to the fake phone. The attacker initiates authentication of the fake phone with a real BTS. The RAND received by the fake phone for the IMSI is sent back via the fake BTS to the MS. The MS computes SRES and returns it to the fake phone via the fake BTS. The fake BTS orders the MS to start the A5/2 cipher encryption procedure. The attacker uses known ciphertext attack \cite{kca} to find the session key, $K_c$. When obtained, it is sent to the fake phone which now has both IMSI and $K_c$ and can finish authentication with the real MNO. The attacker sends back SRES. When the network requests encryption using A5/1, the response can be sent by the adversary since it already knows the $K_c$. 
%\end{itemize}
%\end{comment}

\subsection{Problem Definition}

The basic primitive that we seek to accomplish is to securely exchange information between participating individuals, say $U_1$ and $U_2$, using a partially trustworthy communication channel achieving information secrecy (only the intended entities receive the information) and device-verifiable association of data to another honest device (device knows the information that is associated with a specific honest device). We define secure communication along the lines of Semantic Security \cite{goldreich2004foundations} where knowledge of the ciphertext (and length) of some unknown message does not reveal any additional information on the message that can be feasibly extracted. We define partial trustworthiness of a channel as a probability metric that proportionally provides confidence that the user is communicating with the party he \textit{intended}. We also define honesty as a primitive where the participating parties follow the protocol diligently, without any intention to deceive others.

When the exchange involves more than two people, the group exchange should produce the exact same security properties that would result from the pairwise exchange between all group members. Given such a secure exchange that includes a public key bound to a user, all subsequent mechanisms for authentic and secret communication can be implemented using well known protocols.

\subsection{Goals} 

The main goal of the DSMI protocol is to establish secure communication between participating parties. To enable such a system, we outline four properties desired from the protocol:
\begin{itemize}
\itemsep-0.23em 
\item \textbf{Robustness.} We wish to show that a combination of user ID, device ID and periodic and aperiodic interactions from diverse geographic locations and timestamps creates a unique identity. This identity is hard to forge without substantial expenditure for the adversary. Expenditure in this context includes cost of following the user and/or colluding with other adversaries to obtain additional information. 
\item \textbf{Ergonomic.} We wish to show that the protocol is minimally invasive and requires nominal user intervention.
\item \textbf{Scalablity.} We wish to show that the protocol scales with the number of participating users with minimum latency.
\item \textbf{Portability.} We wish to support interactions between smartphones of several manufacturers, running different operating systems. This promotes heterogeneity in platforms. 
\end{itemize}

\subsection{Assumptions}
Our protocol needs to assume certain user behaviour for successful execution. We assume users can operate a smartphone and follow simple instructions. We also assume that users have a natural desire for security and do not deliberately
disclose private information. Our underlying assumptions are:

\begin{itemize}
\itemsep-0.23em 

%\begin{comment}
%\item \textbf{Users possess \textit{similar} devices}. Users have devices that support the same physical method for exchanging information (e.g., our implementation requires SMS support and programmable software).
%
%\end{comment}

\item \textbf{SMS is delivered with high probability}. The Network Layer in a Cellular Network is unexposed. This makes it harder to compromise and hence messages sent are delivered to the intended recipient with high probability. 

\item \textbf{The adversaries do not collude with each other}. Adversarial action being carried out at two different locations at different timestamps are independent events. That is, their joint probability equals the product of their individual probabilities : $P(\cap_{i=1}^{n} A_i)=\prod_{i=1}^{n} P(A_i)$, for independent events $A_i$, $i \in [1,n]$.

\item \textbf{A user does not deliberately disclose private information}. We assume that the probability of both Sybil attacks \cite{douceur2002sybil} and internal attacks are minimal. 

\item \textbf{The cellular service provider and mobile device is trusted}. Fraudulent cellular service providers could intercept interaction between users or perform a Denial of Service (DoS). However, the probability of a rogue service provider is low. Such providers could insert vulnerabilities into the SIM card or mobile applications using over-the-air (OTA) updates. We also assume that there are no rootkit attacks on the phone and it is devoid of malware.

\item \textbf{Diligent error checking and aborting}. In case of an error or suspicion, users will abort the protocol.

\end{itemize}

DSMI is not limited to only smartphone users. However, we focus on participants who use their smartphones frequently since smartphones are easy to use, are readily available, and are also easy to design applications for. Additionally, the ability to access multiple channels in smartphones helps reduce the load on the cellular network, which will be explained in \S 5.1.

\begin{comment}
\subsection{Initial Authentication Procedure} 

To better understand the protocol, we need to first understand the functioning of authentication in cellular networks. The following are some important steps that are required for the Mobile Station (MS) to connect to the cellular network through the Base Transceiver Station (BTS).

\begin{enumerate}
\item On verification of the unique International Mobile Subscriber Identity (IMSI), the authentication request of a MS is forwarded to the Authentication Center (AuC). The AuC looks for the Root Key, $K_i$ associated with a given IMSI and generates a 128 bit random value (RAND). 
\item Along with $K_i$, RAND is used as input for the A3 and A8 encryption algorithms \cite{comp128}. The outputs are the 32-bit Signed Response (SRES) and the 64-bit Session Key $K_c$ respectively. 
\item The MS calculates its own SRES using RAND, $K_i$ and the A3 encryption algorithm. It also calculates $K_c$ using the RAND received from Base Station Controller (BSC), and $K_i$. 
\item The MS sends back to the network its SRES.
\item The network compares its own SRES with the one obtained from the MS and authenticates the MS on matching. 
\item GSM ciphering is done with the help of the A5 encryption algorithm. There are four variants of A5 in GSM:
\begin{itemize}
\item{A5/0: No ciphering.}
\item{A5/1: Strong ciphering, used in North America and Europe.}
\item{A5/2: Weak ciphering, used in other parts of the world.}
\item{A5/3: Strongest ciphering with open design \cite{kasumi}.}

\end{itemize}
\end{enumerate}
\end{comment}

\subsection{Adversary Model}

We consider that a user can be in the presence of a Dolev-Yao style network adversary \cite{dolev} at a particular location, with probability $P$. This adversary wants to break the properties as described in the problem definition. An additional combinatorial optimization constraint on the adversary coerces it to assimilate maximum information whilst minimizing cost, similar to the one dimensional knapsack problem. Cost or \textit{Bootstrapping Cost} is associated with setting up equipment at each location and is large. Thus, we assume that the adversary will neither follow the user to more than $k$ locations, nor will follow any user continuously. With their devices, adversaries can overhear, intercept, and inject any wireless communication. We also consider DoS attacks by the adversary to be out of scope, as we assume that the diligent users re-start the protocol as needed. 

\subsection{Attacks}

Secure information exchange is a challenging problem. The attacks DSMI is resilient towards include:

\begin{itemize}
\itemsep-0.23em 
\item \textbf{Fake or compromised base station:} The adversary can create a fake BTS to monitor and alter any or all communication relayed through it. This is a form of a MITM attack, resulting in message spoofing and signal jamming \cite{stхhlberg2000radio}.


%\begin{comment}
%\item \textbf{Malicious server:} For protocols that rely on a back-end server, the server may be controlled by a malicious administrator or become compromised.
%
%\item \textbf{Information leakage after protocol abort:} The adversary may be able to cause the protocol to abort and trigger leakage of private information.
%\end{comment}

\item \textbf{Collision attack on low-entropy hash:} Low-entropy hash values are vulnerable to efficient attacks unless precautions are taken.
	
\end{itemize}




==> Old Draft/trusted_locations.tex <==
\section{Trusted location based key exchange}

\subsection{Trusted location data}

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow U_2: & & P_1,(L_1,t,U_1,D_1,c1)S_1  \\
 \textbf{2}.& \quad U_2 \rightarrow U_1: & & P_2,(L_2,t,U_2,D_2,c2)S_2,c1 \\
 \textbf{3}.& \quad U_1 \rightarrow U_2: & & (c2)S_1 \\
\end{align*}

In this protocol, the location data ($L_1,L_2,t)$ is from a trusted
source. The GPS chip within the mobile devices $W_1,W_2$ are trusted
and the cell tower information obtained is also trusted. Hence the
protocol boils down to the three-way handshake protocol. 


\subsection{Trusted point of sale device}

\subsection*{Assumptions}
\begin{itemize}
\item Point of sale devices are trusted. 
\item Point of sale devices have the ability to sign a message and
  transmit the message securely to the device $W_1$ of the user $U_1$.
\end{itemize}

\subsubsection{Protocol}

\begin{align*}
 \textbf{1}.& \quad U_1 \rightarrow G: & & P_1,L_1,t,U_1,D_1  \\
 \textbf{2}.& \quad G \rightarrow U_1: & & G_P, (P_1,L_1,t,U_1,D_1)G_S \\
 \textbf{3}.& \quad U_1 \rightarrow C: & & P_1, (G_P,(P_1,L_1,t,U_1,D_1)G_S)S_1 \\
\end{align*}

\begin{enumerate}
\item[\textbf{1.}] $U_1$ sends the message $P_1,L_1,t,U_1,D_1$ to a
  point of sale device $G$. 

\item[\textbf{2.}] A point of sale device can be a NFC
  device or other device which is capable to signing a message. The
  point of sale device $G$ signs the message $(P_1,L_1,t,U_1,D_1)G_S$
  and along with $G_P$ (public key) sends it back to $U_1$.

\item[\textbf{3.}] Now $U_1$ signs the message it received from $G$,

  ($P_1$,$L_1$,$t$,$U_1$,$D_1$)$G_S$)$S_1$ and sends it to the central
  authority $C$ along with $P_1$. Since $G$ is trusted (has trusted
  credentials), $C$ is certain that the message is signed by $G$ and
  that $U_1$ was indeed present at the point of sale location. The
  point of sale device could also have a fingerprint reader (or any
  biometric device) to authenticate user's identity and the biometric
  data can also be part of the signed message from $G$ to $U_1$. 
\end{enumerate}


